Operational Calibration: Debugging Confidence Errors for DNNs in the Field

Trained DNN models are increasingly adopted as integral parts of software systems, but they often perform deficiently in the field. A particularly damaging problem is that DNN models often give false predictions with high confidence, due to the unavoidable slight divergences between operation data and training data. To minimize the loss caused by inaccurate confidence, operational calibration, i.e., calibrating the confidence function of a DNN classifier against its operation domain, becomes a necessary debugging step in the engineering of the whole system. Operational calibration is difficult considering the limited budget of labeling operation data and the weak interpretability of DNN models. We propose a Bayesian approach to operational calibration that gradually corrects the confidence given by the model under calibration with a small number of labeled operation data deliberately selected from a larger set of unlabeled operation data. The approach is made effective and efficient by leveraging the locality of the learned representation of the DNN model and modeling the calibration as Gaussian Process Regression. Comprehensive experiments with various practical datasets and DNN models show that it significantly outperformed alternative methods, and in some difficult tasks it eliminated about 71% to 97% high-confidence (>0.9) errors with only about 10\% of the minimal amount of labeled operation data needed for practical learning techniques to barely work.

==> OptConfPaper/conclusions.tex <==
% !TEX root = main.tex
\section{conclusion}
\label{sec:conclusion}

Software quality assurance for systems incorporating DNN models 
is urgently needed. 
This paper focuses on the problem of operational calibration that 
detects and fixes the errors in the confidence given by a DNN model 
for its predictions in a given operation domain.
A Bayesian approach to operational calibration 
is given. It solves the problem with Gaussian Process Regression, 
which leverages the locality of the operation data, 
and also of their prediction correctness, in the representation space. 
\replaced{Experiments with representative datasets and DNN models
confirmed that the approach can significantly reduce the risk of 
high-confidence false prediction with a small number of  labeled data,
and thus efficiently improve the models' quality of service in operational settings.
}{The approach achieved impressive efficacy and efficiency 
in experiments with representative datasets and DNN models.} 


While with empirical evidence, we consider conducting more theoretical analysis on aspects
%Theoretical analysis on aspects 
such as the data efficiency and 
the convergence of our algorithm as future work. %is left for future work. 
In addition, we plan to investigate operational calibration methods 
for real-world decisions with more complicated cost models. 



==> OptConfPaper/confidence.tex <==
% !TEX root = main.tex

\section{Operational calibration Problem}
\label{sec:problem}

Now we focus on the problem of operational calibration. % as a specific quality assurance task for engineering DNN-based systems in the field. 
We first briefly introduce DNN classifiers and their prediction confidence to pave the way for 
the formal definition of the problem. 

\subsection{DNN classifier and prediction confidence}
\label{subsec:dnnconfidence}

A deep neural network classifier contains multiple hidden layers between its input and output layers. 
A popular understanding~\cite{Goodfellow-et-al-2016} of the role of these hidden layers is that 
they progressively extract abstract features (e.g., a wheel, human skin, etc.) 
from a high-dimensional low-level input (e.g., the pixels of an image). 
These features provide a relatively low-dimensional high-level \emph{representation} $\bm{z}$ for the input $\bm{x}$, which makes the classification much easier, e.g., the image is more likely to be a car if wheels are present. 

What a DNN classifier tries to learn from the training data is a posterior probability distribution, 
denoted as $p(y \mid \bm{x})$~\cite{bishop2006prml}.
For a \textit{K}-classification problem, the distribution can be written as 
$p_i(\bm{x}) = p(y = i \mid \bm{x})$, where $i=1,2,\dots,K$. 
For each input $\bm{x}$ whose representation is $\bm{z}$, 
the output layer first computes the non-normalized prediction  
$\bm{h} =\bm{W}^{\top} \bm{z} + \bm{b}$, 
whose element $h_i$  is often called the \emph{logit} for the $i$-th class. 
The classifier then normalizes $\bm{h}$ with a softmax function to approximate the posterior probabilities
\begin{equation}
\hat{p}_i(\bm{x}) = \text{softmax}(\bm{h})_i=\frac{e^{h_i} }{\sum_{j=1}^{K} e^{h_j}}, \quad i=1, \ldots, K.
\end{equation}
%where $h_i$ is the logit value for the $i$th class.   
%(aslo called logit layer). 
%logit layer precede the softmax (output) layer. 
%and then classify inputs according to the features with a softmax function implemented in the output layer.
%%Therefore, we also refer the output layer as softmax layer.
%The purpose of training a DNN model with a data set 
%
%For a DNN model, it actually learned a posterior probability distribution~\cite{bishop2006prml} from training data, 
%denoted as $p(y \mid \bm{x})$.
%Particularly, for the given input $\bm{x}$, DNN will provided \textit{K} posterior probability values $p_i = p(y = i \mid \bm{x}), i=1,2,\dots,K$ 
%
Finally, to classify $\bm{x}$, one just chooses the 
%he classification result for this input is 
the category corresponding to the maximum posterior probability, 
i.e.,  
 \begin{equation}
 \hat{y}(\bm{x}) = \mathop{\arg\max}_i \hat{p}_i(\bm{x}).
 \end{equation}


Obviously, this prediction is intrinsically uncertain.  
%$\hat{y}(\bm{x}) = \arg\max_i p(y = i \mid \bm{x})$, 
The \emph{confidence} for this prediction, which quantifies the  
likelihood of correctness, can be naturally measured as 
the estimated posterior class probability 
% $$\hat{c}(\bm{x}) = \max_i \hat{p_i}(\bm{x}).$$ 
 \begin{equation}
 \hat{c}(\bm{x}) = \hat{p_i}(\bm{x}),  \quad i=\hat{y}(\bm{x}).
 \end{equation}
%
Confidence takes an important role in decision-making. 
For example, if the loss due to an incorrect prediction % $u_1$
is four times of the gain of a correct prediction, % $u_2$, 
one should not invest on predictions with confidence less than 0.8. 
%Inaccurate confidence could cause significant loss. 
%For example, an over-confident benign prediction for a pathology image 
%could mislead a doctor into overlooking a malignant tumor, 
%while an under-confident benign prediction could result in unnecessary confirmatory testings. 

Modern DNN classifiers are often inaccurate in confidence~\cite{szegedy2016rethinking}, 
because they overfit to the surrogate loss used in training~\cite{guo2017calibration, tewari2007consistency}. 
Simply put, they are over optimized toward the accuracy of classification, 
but not the accuracy of estimation for posterior probabilities. 
To avoid the potential loss caused by inaccurate confidence, 
\emph{confidence calibration} can be employed in the learning process~~\cite{flach2016calibration,guo2017calibration,tewari2007consistency}. 
\added{Early calibration methods such as isotonic regression~\cite{zadrozny2002transforming}, 
histogram binning~\cite{zadrozny2002transforming}, and Platt scaling~\cite{Platt1999probabilisticoutputs} simply 
train a regression model taking the uncalibrated confidence as input with the validation dataset.
More flexible methods, e.g., Temperature Scaling~\cite{hinton2015distilling}, 
find} a function $R$
to correct the logit $\bm{h}$ such that 
 \begin{equation}
 \hat{c}(\bm{x}) = \hat{p_i}(\bm{x})=\text{softmax}(R(\bm{h}))_i,  \quad i=\hat{y}(\bm{x})
 \label{equ:logitcali}
 \end{equation}
matches the real posterior probability $p_i(\bm{x})$. 
%   
Notice that, in this setting the inaccuracy of confidence is viewed as a kind of 
systematic error or bias, not associated with particular inputs or domains.
That is, \added{the calibration does not distinguish between different inputs with the same uncalibrated confidence.} \deleted{$R$ does not take $\bm{x}$ or $\bm{z}$ as input}. 




%which means 
%
%The fundamental goal of confidence calibration 
%is to make the confidence for a given input 
%equal to the true posterior probability of predictions.
%One often assume that confidence error 
%is caused by some systematic error of $\bm{h}$.
%For details, for each input, 
%there produces some consistent shifts between $\bm{h}$ 
%and the logit $\bm{h}'$ corresponding to true posterior probability.
%Thus, what we need to do is to learn a function
%that maps original logit $\bm{h}$ to the true logit $\bm{h}'$.

%There exist different kinds of calibration methods, such as isotonic regression~\cite{zadrozny2002transforming}, 
%histogram binning~\cite{zadrozny2002transforming}, and Platt scaling~\cite{Platt1999probabilisticoutputs}. 
%\added{These methods all attempt to train a regression model whose input is confidence. 
%For example, 
%The isotonic regression attempt to find a one-dimensional monotonic calibration function such that minimizing the Brier score.
%and the Platt scaling define the calibration function as}
%\begin{equation}
%\added{R(c) = \frac{1}{1+e^{-(a \cdot c + b)}},}
%\end{equation}
%\added{where $c$ is the input of confidence value, and $a, b$ are parameter computed by minimizing the cross entropy on the validation dataset. }
%However, according to a recent study~\cite{guo2017calibration}, 
%the most effective choice is often a simple method called Temperature Scaling~\cite{hinton2015distilling}.
%The idea is to define the calibration function as
% \begin{equation}
% R(\bm{h}) = \frac{\bm{h}}{T}, 
% \end{equation}
%where $T$ is a scalar parameter computed by minimizing the 
%negative log likelihood~\cite{hastie2009elements}
%on the validation dataset. 
%\added{Moreover, Platt scaling can also be improved through taking logit as input~\cite{guo2017calibration}, i.e., define the calibration function as}
% \begin{equation}
% \added{R(\bm{h}) = \bm{W}^{\mathsf{T}}\bm{h}+\bm{b}, }
% \end{equation}
% \added{where $\bm{W}$ is a matrix parameter and $\bm{b}$ is a vector parameter. 
% Both of these two parameters are computed by minimizing the cross entropy. }
 
%\begin{equation}
%\text{NLL}=- \sum_{i=1}^{n} \log \hat{c}(\bm{x}_i).
%\end{equation} 

%\emph{Expected Calibration Error}:
%\begin{equation}
%\mathrm{ECE}=\sum_{m=1}^{M} \frac{\left|D_{m}\right|}{n}\left|\operatorname{acc}\left(D_{m}\right)-\operatorname{conf}\left(D_{m}\right)\right|,
%\end{equation}
%where $D_m$ is the set of inputs whose confidence falls into 
%the interval $I_{m}=\left(\frac{m-1}{M}, \frac{m}{M}\right]$, 
%and the $acc(D_m)$ and $conf(D_m)$ are the expected accuracy and confidence in $D_m$, respectively.

%
%The experimental results show that the most fruitful method for calibration are \emph{temperature scaling} (TS):
%\begin{equation}
%\hat{q}(\bm{x}) = \max_{i} \frac{e^{(h_i/T)}}{\sum_{j=1}^{K} e^{(h_j/T)}}, \quad i=1, \ldots, K.
%\end{equation}
%where the temperature $T$ is chosen by minimizing the ECE.



%We first define the problem, and then present our method based on Gaussian Process. 

\subsection{Operational confidence calibration}



Given a domain where a previously trained DNN model is deployed, 
operational calibration 
identifies and fixes the model's errors in the confidence of predictions on individual inputs
in the domain.  
%against a set of operation data collected from 
%for a given domain in which the model actually operates.
%
%Viewing confidence as part of model output, operational calibration is not only testing, 
%but also a kind of debugging.  
%
Operational calibration is conservative in that it does not change the predictions made by the model, 
but tries to give accurate estimations on the likelihood of the predictions being correct. 
With this information, a DNN model will be useful even though its prediction accuracy 
is severely affected by the domain shift. 
One may take only its predictions on inputs with high confidence, 
but switch to other models or other backup measures if unconfident.  
 
 

%\subsection{Operational calibration}



%What operational calibration addresses is more an engineering problem than a machine learning problem.
%The essential task of machine learning is to induce from training data, 
%and it emphasizes the generalizability of the trained model, 
%although unfortunately the scope of generalization cannot be explicitly specified. 
%In dealing with domain shift, machine learning techniques such as transfer learning or domain adaptation 
%tend to \emph{generalize} the scope of the model to include the new operation context. 
%As a consequence these techniques heavily relies on the data from the original domain, 
%besides the new data from the operation context. 

%Contrastingly, operational calibration tries to make the most of a DNN model in a given operation context. 
%The model may be trained by a third party and provided \emph{as is}. 
%In operational calibration  
%the generalization to any domain other than the current one is not necessary.
%This more focused duty relieves us of the dependence to the original data. 
%The decoupling of DNN models from their training data and process is crucial to 
%promote the reuse of these models and to reduce privacy and proprietary risks~\cite{zhou2016learnware}. 
%Operational calibration also prioritize the saving of efforts in labeling data collected in operation context.   
%
%Besides these methodological considerations, 
%as to be shown later in Section~\ref{sec:evaluation},
%practically it would be imprudent and ineffective 
%to fine-tune or adapt a DNN model to fit an operational context 
%without access to the original training data, 
%unless we could afford a large number of labeled operation data.
%The trap here is that 
%%the performance of the model could be worsen because it 
%the model is very likely to be overfitting to the limited labeled operation data, 
%but not the entire operation domain without the balance from the original training data. 


 
%
%technique or fine-tuning  
%
%However, when applying DNN into application, 
%the specific operation context bring two tremendous difficulties. 
%First, the domain shift
%between original context and operation context 
%leads to some non-systematic error. 
%Therefore, the TS and other similar methods, which only rely on the logit, 
%is not effective in calibrating the operational confidence.
%Second, the information of original context, which includes original dataset and detailed training process of DNN, may be unavailable, 
%and operation dataset is not large enough. 
%Thus the transfer learning technique even fine-tuning could not effectively increasing the accuracy of model.
%%In this situation, it is reckless to modify the model directly based on operation data.

%Fortunately, the ability in extracting features is still useful. 
%In other words, the representation $\bm{z}$ in last hidden layer is still reliable.
%In this situation, instead of learning the parameters of function which map $\bm{z}$ to the true logit, we choose a bayesian method to estimate the operation confidence.

To quantify the accuracy of the confidence of a DNN model on a dataset 
%$D = \{(\bm{x}_i, \mathbb{I}(\bm{x}_i)), i=1,\dots,N\}$, 
$D = \{(\bm{x}_i, y_i), i=1,\dots,N\}$, 
one can use the  
%Generally, the confidence of a machine learning model can be viewed as a prediction operation datafor 
%the likelihood of the model giving correct prediction on a given input. 
%It can be measured by 
Brier score (BS)~\cite{brier1950verification}, which is actually the mean squared error of the estimation:
\begin{equation}
BS(D) = \frac{1}{N}\sum_{i=1}^N (\mathbb{I}(\bm{x}_i) - \hat{c}(\bm{x}_i))^2, 
\end{equation}
where $\mathbb{I}(\bm{x})$ 
is the indicator function for whether the labeled input $\bm{x}$ 
is misclassified or not, i.e., 
$\mathbb{I}(\bm{x}) = 1$ if $\hat{y}(\bm{x})=y(\bm{x})$, and $0$ otherwise.  
%is indicator function for whether the classification result is correct.



Now we formally define the problem of operation calibration:
\begin{problem} 	
%Given $\mathfrak{M}$ a previously trained DNN classifier, 
%%with its original confidence estimation $\hat{c}(\cdot)$
%$S$ a set of $N$ unlabeled examples collected from an operational domain, 
%and a budget $n \ll N$ for labeling the examples in $S$, 
%the task of operation calibration is try to find a confidence estimation function 
%$\hat{c}(\cdot)$ for $\mathfrak{M}$ 
%to minimize $BS(S)$ the Brier score in the cost-insensitive case, 
%or $\ell(S)$ for given $\lambda$ the loss due to confidence error in the cost-sensitive case.  
Given $\mathfrak{M}$ a previously trained DNN classifier, 
%with its original confidence estimation $\hat{c}(\cdot)$
$S$ a set of $N$ unlabeled examples collected from an operation domain, 
and a budget $n \ll N$ for labeling the examples in $S$, 
the task of operational calibration is to find a confidence estimation function 
$\hat{c}(\cdot)$ for $\mathfrak{M}$ with minimal Brier score $BS(S)$.
%to minimize  the .
%in the cost-insensitive case, 
%or $\ell(S)$ for given $\lambda$ the loss due to confidence error in the cost-sensitive case.  
\end{problem}

Notice that operational calibration is different from the confidence calibration discussed in 
Section~\ref{subsec:dnnconfidence}.
The latter is domain-independent and usually included as a step in the training process of a DNN model (one of machine learning's focuses), 
but the former is needed when the model is deployed as a software component by a third party in a specific operation domain (what software engineering cares about). 
Technically, operational calibration cannot take the confidence error as a systematic error of the learning process, 
%as the latter does, 
because the error is caused by the domain shift 
from the training data to the operation data, and it may \added{assign different confidence values to inputs with the same uncalibrated confidence value.} \deleted{depend on specific inputs from the operation domain.}


==> OptConfPaper/dnnqa.tex <==
% !TEX root = main.tex

\section{Quality assurance for DNN models used as software artifacts}
\label{sec:operqa}

%Deep learning is intrinsically inductive~\cite{Goodfellow-et-al-2016}.
%However, conventional software engineering is mostly deductive, as evidenced by 
%its fundamental principle of specification-implementation consistency. 
%Adopting DNN models as integral parts of software systems poses 
%new challenges for quality assurance. 
%We first discuss the quality assurance problem for DNN models used in 
%given operation domains from a software engineering perspective, 
%and then briefly introduce DNN and its prediction confidence
%to provide the background for the work on operational calibration.  

%Different from human written programs, a DNN model is intrinsically uncertain about its predictions, 
%which is quantified by the corresponding confidence values. 
%Confidence takes an important role in practical decisions. 
%In this section we briefly introduce DNN and prediction confidence, 
%formally define the problem of confidence calibration for DNN in operation context, 
%and discuss its connection and difference with the calibration step usually included in the model training process.  

%\subsection{Operational quality assurance}

Well trained DNN models can provide marvelous capabilities, 
but unfortunately their failures in applications are also very common~\cite{Riley2019nature}.
When using a trained model as an integral part of a high-stakes software system, 
it is crucial to know quantitatively \emph{how well} the model will work \added{and to adapt it to the application conditions}.
The quality assurance combining the viewpoints from software engineering and machine learning is needed, but largely missing. 
\added{In what follows, we first discuss the non-conventional requirements for such quality assurance, 
and then give an application scenario to highlight the software engineering concerns. 
}




Deep learning is intrinsically inductive~\cite{Goodfellow-et-al-2016, zhou2019abductive}.
However, conventional software engineering is mostly deductive, 
as evidenced by its fundamental principle of specification-implementation consistency. 
%The principle of software quality assurance is founded on the specifications for software artifacts 
%and the deductive reasonings based on them. 
A specification defines the assumptions and guarantees of a software artifact.
The artifact is expected to meet its guarantees whenever its assumptions are satisfied.
Thus explicit specifications make software artifacts more or less domain independent.
However, statistical machine learning does not provide such kind of specifications. 
Essentially it tries to induce a model from its training data, 
which is intended to be general 
so that the model can give predictions on previously unseen inputs. 
Unfortunately the scope of generalization is unspecified. 
%Most transfer learning and domain adaptation techniques tries to 
%Thus the problem of domain shift is regarded as the lack of generalization 
As a result, a major problem comes from the divergence between the domain 
where the model was originally trained 
and the domain where it actually operates. 

So the first requirement for the quality assurance of a DNN model is to be \emph{operational}, i.e., to 
focus on the concrete domain where the model actually operates. 
Logically speaking, the quality of a trained DNN model will be pointless without considering its operation domain.
In practice, the performance of a model may drop significantly with domain shift~\cite{li2019boosting}.
%
On the other hand, focusing on the operation domain also relieves the DNN model 
from depending on its original training data. 
Apart from practical concerns such as protecting the privacy and property of the training data, 
decoupling a model from its training data and process will also be helpful for (re)using it 
as a commercial off-the-shelf (COTS) software product~\cite{zhou2016learnware}. 
This viewpoint from software engineering is in contrasting to machine learning techniques dealing with domain shift such as 
transfer learning or domain adaptation that heavily rely 
on the original training data and hyperparameters~\cite{pan2009survey,shu2018a,transferlearning.xyz}. 
They need original training data because they try to \emph{generalize} 
the scope of the model to include the new operation domain. 



The second requirement is to embrace the uncertainty that is intrinsic in DNN models. 
A defect, or a ``bug'', of a software artifact is a case that it does not deliver its promise. 
Different from conventional software artifacts, 
a DNN model never promises to be certainly correct on any given input, 
and thus individual incorrect predictions \emph{per se} should not be regarded as bugs, 
but to some extent features~\cite{ilyas2019adversarial}.   
Nevertheless, the model \emph{statistically} quantifies the uncertainty of their predictions. 
Collectively, it is measured with metrics such as accuracy or precision. 
Individually, it is stated by the confidence value about the prediction on each given input.  
These qualifications of uncertainty, as well as the predictions a model made, 
should be subject to quality assurance. 
For example, given a DNN model and its operation domain, 
operational testing~\cite{li2019boosting} examines 
to what degree the model's overall accuracy is degraded by the domain shift.
Furthermore, operational calibration, which is the topic of the current paper, 
identifies and fixes the misspecified confidence values on individual inputs.  
%Viewing confidence as part of model output, operational calibration is not only testing, 
%but also a kind of debugging.  

Finally, operational quality assurance should prioritize the saving of human efforts, 
which include the cost of collecting, and especially labeling, the data in the operation domain.  
The labeling of operation data often involves physical interactions, such as surgical biopsies  
and destructive testings, and thus can be expensive and time-consuming. 
%
Note that, as exemplified by the EU GDPR~\cite{eu-269-2014}, there are 
increasing concerns about the privacy and property rights in the data used to train DNN models. 
So when adopting a DNN model trained by a third party, 
one should not assume the availability of its original training data~\cite{zhou2016learnware, Shokri2015CCS, konevcny2016federated}. 
Without the access to the original training data, 
re-training or fine-tuning a DNN model to an operation domain can be unaffordable 
because it typically requires a large amount of labeled examples to work. 
Quality assurance activities often have to work under a much tighter budget for labeling data. 



\begin{figure}[htbp]
\begin{center}
\includegraphics[width=.95\columnwidth]{figures/OpQA}
\caption{Operational quality assurance}
\label{fig:opqa}
\end{center}
\end{figure}

Figure~\ref{fig:opqa} depicts the overall idea for operational quality assurance, 
which generalizes the process of operational testing proposed in~\cite{li2019boosting}. 
A DNN model, which is trained by a third party with the data from the origin domain, 
is to be deployed in an operation domain. It needs to be evaluated, and possibly adapted, 
with the data from the current operation domain. To reduce the effort of labeling, 
data selection can be incorporated in the procedure with the guidance of the information generated by  
the DNN model and the quality assurance activity.
Only the DNN models that pass the assessments and are possibly equipped 
with the adaptations will be put into operation. 





\added{
\medskip
For example, consider a scenario that a hospital decides to equip its radiology 
department with automated medical image analysis enabled by Deep Learning~\cite{obermeyer2016predicting}. 
While the system may involve many functionalities such as clinical workflow management, 
computer-aided diagnosis, and computer-assisted reporting, the key component is a DNN model or an ensemble of DNN models 
acting as a radiologist to classify images~\cite{MCM20DLRadiology}. 
It is too expensive and technically demanding for the hospital to collect enough high quality data and 
train the model in-house. 
So the hospital purchases the model from a third-party provider, and uses it as a COTS software component. 
However, the training conditions of the model are likely to be different from the operation conditions,
and the model performance reported by the provider is unreliable due to potential issues 
such as data mismatch, selection bias, and non-stationary environments~\cite{WMD18DLbiomedicine,Zech18VarGenDLRadiograph}. 
%In such a scenario re-training the model for the operation domain is usually infeasible, 
%due to the unavailability of the original training data and the limited availability of the labeled operation data~\cite{kemker2018measuring, kirkpatrick2017overcoming}.
To assure the system's quality of service, the model must be tested and calibrated against the current operation domain. 
The hospital first assesses the real accuracy of the model through operational testing~\cite{li2019boosting}, 
and decides to adopt it or not accordingly. 
Once the model is adopted and deployed, operational calibration steps in to adapt the model to the current operation domain, 
by fixing the errors in the confidence values and avoiding high-confidence false predictions. }

\added{
As a software quality assurance task, operational calibration tries to achieve best efficacy 
with a limited budget. The cost here, however, is mainly spent on the labeling of 
operation data. For sophisticated DNN models used for medical imaging classification such as Inception-V3, ResNet-50 and DenseNet-121~\cite{liu2017detecting, Zech18VarGenDLRadiograph}, 
even thousands of labeled data 	could be too less 
for model retraining or fine-tuning to work properly (c.f. Figure~\ref{fig:fine-tune1}). 
Nevertheless, as will be shown later, a deliberately designed calibration method 
can identify and fix most of the erroneous high confidence values associated to false predictions 
with only tens to small hundreds of labeled data (c.f. Figure~\ref{fig:efficiency-curve}).  
A model well calibrated for its operation domain, 
although still suffering from some loss in prediction accuracy, 
becomes more reliable in that broken promises are far less likely.   
%
%We give an example to explain the problem of operational confidence calibration more clearly.
%The hospital developed a medical image detection system to assist doctors in checking up patients. 
%The DNN model deployed in the system is well-trained based on original training data. 
%However, the performance (e.g., accuracy of prediction) drops significantly when using this system as the application on operation domain.
%Many factors may cause this problem, such as 
%mislabeling the training data, 
%damage to the image acquisition camera,
%and the emergence of new kinds of diseases.
%Actually, differences between origin domain and operation domain are almost inevitable~\cite{pooch2019can}. 
%In this situation, it is impossible to re-train a new model towards operation domain since labeling cost is too expensive and the size of operation data is too limited to support effective training~\cite{kemker2018measuring, kirkpatrick2017overcoming}.
%Thus, one may instead try to ``fix'' the current model to make full use of this system, 
%and the most practicable method is to calibrate the confidence on operation domain such that minimizing the loss caused by the low accuracy of DNN model.
}

  


==> OptConfPaper/evaluation.tex <==
% !TEX root = main.tex
\section{Empirical evaluation}
\label{sec:evaluation}

We conducted a series of experiments to answer the following questions:
\begin{enumerate}
\item Is our approach to operational calibration generally effective in different tasks?
\item How effective it is, compared with alternative approaches?
\item How efficient it is, in the sense of saving labeling efforts? 
\end{enumerate}


We implemented our approach on top of the PyTorch 1.1.0 DL framework.
The code, together with the experimental data, are available at \url{https://github.com/Lizn-zn/Op-QA}. 
The experiments were conducted on a GPU server 
with two Intel Xeon Gold 5118 CPU @ 2.30GHz,
400GB RAM, and 10 GeForce RTX 2080 Ti GPUs.
The server ran Ubuntu 16.04 with GNU/Linux kernel 4.4.0. 

The execution time of our operational calibration 
depends on the size of the dataset used, and the architecture of the DNN model.  
For the tasks listed below, the execution time varied from about 3.5s to 50s, 
which we regard as totally acceptable. 

%\subsection{Evaluation setup}
\subsection{Experimental tasks}
To evaluate the general efficacy of our approach, 
we designed six tasks that were different in the application domains 
(image recognition and natural language processing), 
operation dataset size (from hundreds to thousands),
classification difficulty (from 2 to 1000 classes),
and model complexity (from $\sim$$10^3$ to $\sim$$10^7$ parameters).
To make our simulation of domain shifts realistic, 
in four tasks we adopted third-party operation datasets often used in the transfer learning research,
and the other two tasks we used mutations that are also frequented made in the machine learning community.  
Figure~\ref{fig:orig-and-opt} demonstrates some example images from the origin and operation domains 
\added{for tasks 3 and 5}.
%{\color{blue} Actually, a few factors may induce differences between origin domain and operation domain, such as the time of data collection (Task 2), the style of image background (Task 3), and the resolution of images (Task 6).
%}
%
%Considering different possible operation domains, 
%we choose various datasets to evaluate our approach. 
%In addition, DNN models with very different structures were used in these experiments.  
Table~\ref{tab:ExpDesign} lists the settings of the six tasks. %information of experimental design in details. 


%\begin{table}[htb]
%\caption{Dataset and model settings}
%\centering
%\setlength{\tabcolsep}{.38em}
%\begin{threeparttable}
%\begin{tabular}{|p{1.7cm}<{\centering}|c|p{1.1cm}<{\centering}|c|p{1.1cm}<{\centering}|}
%\hline
%\multirow{2}*{\textbf{Model}} & \multicolumn{2}{c|}{\textbf{Original}}  & \multicolumn{2}{c|}{\textbf{Operational}} \\
%\cline{2-5}
%& \textbf{Dataset} & \textbf{Acc. (\%)} & \textbf{Dataset} & \textbf{Acc. (\%)} 
%\\
%\hhline{|=====|}
%LeNet-5 & MNIST & 96.9 & USPS & 68.0 \\
%\hline %\hhline{|======|}
%RNN & Polarity v1.0 & 99.0 & Polarity v2.0 & 83.4 \\
%\hline
%VGG-19 & CIFAR-10 & 93.1 & Rotation & 71.1 \\
%\hline
%ResNet-50 & ImageCLEF-c & 99.2 & ImageCLEF-p & 73.2 \\
%\hline
%Inception-v3 & ImageNet & 77.5 & Down-sampling & 48.9 \\
%\hline
%\end{tabular}
%\end{threeparttable}
%\label{tab:ExpDesign}
%\end{table}

\begin{table}[htb]
\caption{Dataset and model settings of tasks}
\centering
\setlength{\tabcolsep}{.25em}
\begin{threeparttable}
\begin{tabular}{|c|c|c|c|c|p{0.4cm}<{\centering}|}
\hline
\multirow{2}*{\textbf{Task}} & \multirow{2}*{\textbf{Model}} & \multicolumn{3}{c|}{\textbf{Origin Domain} $\rightarrow$ \textbf{Operation Domain}} \\
\cline{3-5}
& & \textbf{Dataset} & \textbf{Acc. (\%)} & \textbf{Size$^*$} \\
\hhline{|=====|}
\multirow{2}*{1} & \multirow{2}*{LeNet-5} & Digit recognition & \multirow{2}*{96.9 $\rightarrow$ 68.0} & \multirow{2}*{900} \\
& & (MNIST $\rightarrow$ USPS) &  & \\
\hline %\hhline{|======|}
\multirow{2}*{2} & \multirow{2}*{RNN} & Polarity & \multirow{2}*{99.0 $\rightarrow$ 83.4} & \multirow{2}*{1,000} \\
& & (v1.0 $\rightarrow$ v2.0) & & \\
\hline
\multirow{2}*{3} & \multirow{2}*{ResNet-18} & Image classification & \multirow{2}*{93.2 $\rightarrow$ 47.1} & \multirow{2}*{5,000} \\
& & CIFAR-10 $\rightarrow$ STL-10 &  & \\
\hline
\multirow{2}*{4} & \multirow{2}*{VGG-19} & CIFAR-100 & \multirow{2}*{72.0 $\rightarrow$ 63.6} & \multirow{2}*{5,000} \\
& & (orig. $\rightarrow$ crop) &  & \\
\hline
\multirow{2}*{5} & \multirow{2}*{ResNet-50} & ImageCLEF & \multirow{2}*{99.2 $\rightarrow$ 73.2} & \multirow{2}*{480} \\
& & (c $\rightarrow$ p) &  & \\
\hline
\multirow{2}*{6} & \multirow{2}*{Inception-v3} & ImageNet & \multirow{2}*{77.5 $\rightarrow$ 45.3} & \multirow{2}*{5,000} \\
& & (orig. $\rightarrow$ down-sample) &  & \\
\hline
\end{tabular}
 \begin{tablenotes}
        \footnotesize
        \item[*] It refers to the maximum number of operation data available for labeling.
      \end{tablenotes}
\end{threeparttable}
\label{tab:ExpDesign}
\end{table}

% In our experiments, we set the number of clusters as 30, 
In Task 1 we applied a LeNet-5 model originally trained 
with the images from the \textbf{MNIST} dataset~\cite{lecun1998gradient} 
to classify images from the \textbf{USPS} dataset~\cite{friedman2001elements}. 
Both of them are popular handwritten digit recognition datasets consisting of 
single-channel images  of size 16$\times$16$\times$1, \added{but the latter is more difficult to read}.
%We will introduce each dataset in the following.
%\textbf{MNIST/USPS} are two ~\cite{lecun1998gradient, friedman2001elements}.
%Each image is single-channel of size 16$\times$16$\times$1.
%
%We randomly selected samples from MNIST and USPS 
%to constructed training and operation domains, respectively. 
The size of the training dataset was 2,000, and the size of the operation dataset was 1,800.
We reserved 900 of the 1,800 operation data for testing, and used the other 900 for operational calibration. 
%For the operation dataset, we divide it into two sets with the same size.
%We use the first set to do the tasks of input selection, input labeling, and building the gaussian process.
%The second set is held out as the test set for operation domain.


Task 2 was focused on natural language processing. 
\textbf{Polarity} is a dataset for sentiment-analysis~\cite{Pang2002sentiment}. 
It consists of sentences labeled with corresponding sentiment polarity (i.e., positive or negative). 
We chose Polarity-v1.0, which contained 1,400 movie reviews collected in 2002, as the training set.
The Polarity-v2.0, which contained 2,000 movie reviews collected in 2004, was used as the data from 
the operation domain. We also reserved half of the operation data for testing. 
%Similarly, for the operation dataset, 
%we divide it into two sets with the same size for calibration and testing.

In Task 3 we used two classic image classification datasets \textbf{CIFAR-10}~\cite{krizhevsky2009learning}
 and \textbf{STL-10}~\cite{coates2011analysis}.
The former consists of 60,000 32$\times$32$\times$3 images in 10 classes, 
and each class contains 6,000 images.
The latter has only 1,3000 images, 
but the size of each image is 96$\times$96$\times$3.
We used the whole CIFAR-10 dataset to train the model. 
The operation domain was represented by 8,000 images collected from STL-10, 
in which 5,000 were used for calibration, and the other 3,000 were reserved for testing.


Tasks 4 used the dataset \textbf{CIFAR-100}, which was more difficult than 
CIFAR-10 and contained 100 classes with 600 images in each.
We trained the model with the whole training dataset of 50,000 images.
To construct the operation domain, we randomly cropped the remaining 10,000 images. % as the operation dataset.
One half of these cropped images were used for calibration and the other half for testing.
%The examples of original domain and operation domain are shown in Figure~\ref{fig:orig-and-opt}.

Task 5 used the image classification dataset from the \textbf{ImageCLEF} 2014 challenge~\cite{Mller2010ImageCLEF}. 
It is organized with 12 common classes derived from three different domains: 
ImageNet ILSVRC 2012 (i), Caltech-256 (c), and Pascal VOC 2012 (p).
We chose the dataset (c) as the origin domain and dataset (p) as the operation domain.
Due to the extremely small size of the dataset, we divided the dataset (p) 
for calibration and testing by the ratio 4:1.
%The examples of original domain and operation domain are shown in Figure~\ref{fig:orig-and-opt}.
 
Finally, Task 6 dealt with an extremely difficult situation. 
\textbf{ImageNet} is a large-scale image classification dataset 
containing more than 1.2 million 224$\times$224$\times$3 images across 1,000 categories~\cite{Deng09imagenet}.
The pre-trained model Inception-v3 was adopted for evaluation.
The operation domain was constructed by down-sampling 10,000 images from the original test dataset.
Again, half of the images were reserved for testing.
%The examples of original domain and operation domain are shown in Figure~\ref{fig:orig-and-opt}.

\begin{figure}[htbp]
\begin{center}
\subfloat[CIFAR-10 (origin domain)]{
\includegraphics[width=.42\columnwidth]{figures/show/cifar10/orig1.png}}
%\includegraphics[width=.4\columnwidth]{figures/show/cifar10/orig2.png}}
\hspace{2em}
\subfloat[STL-10 (operation domain)]{
\includegraphics[width=.42\columnwidth]{figures/show/cifar10/opt1.png}}
%\includegraphics[width=.4\columnwidth]{figures/show/cifar10/opt2.png}} \\

\subfloat[ImageCLEF-(c) (origin domain)]{
\includegraphics[width=.21\columnwidth]{figures/show/imageclef/orig1.png}
\includegraphics[width=.21\columnwidth]{figures/show/imageclef/orig2.png}}
\hspace{2em}
\subfloat[ImageCLEF-(p) {\tiny (operation domain)}]{
\includegraphics[width=.21\columnwidth]{figures/show/imageclef/opt1.png}
\includegraphics[width=.21\columnwidth]{figures/show/imageclef/opt2.png}} \\
%\subfloat[ImageNet-origin]{
%\includegraphics[width=.4\columnwidth]{figures/show/imagenet/orig1.png}
%\includegraphics[width=.4\columnwidth]{figures/show/imagenet/orig2.png}}
%\hspace{2em}
%\subfloat[ImageNet-operation]{
%\includegraphics[width=.4\columnwidth]{figures/show/imagenet/opt1.png}
%\includegraphics[width=.4\columnwidth]{figures/show/imagenet/opt2.png}} 
\caption{Examples of origin and operation domains. 
\added{\rm{In task~3 a ResNet-18 model was trained with low-resolution images (a), but applied to high-resolution images (b). In task~5 a ResNet-50 model was applied to images (d) with backgrounds and styles different from training images (c). }}
%\rm{The left column is the images collected from CIFAR-10 and ImageCLEF-c, which are used as the original data. 
%The right column is the images collected from STL-10 and ImageCLEF-p, which are used as the operation data.}
}
\label{fig:orig-and-opt}
\end{center}
\end{figure}


\subsection{Efficacy of operational calibration}

Table~\ref{tab:brier-score} gives the Brier scores of the confidence before (col. Orig.) and after (col. GPR) operational calibration. 
In these experiments all operation data listed in Table~\ref{tab:ExpDesign} (not including the reserved test data) were labeled and used in the calibration.
The result unambiguously confirmed the general efficacy of our approach. 
%and its superiority over alternative approaches. 
In the following we elaborate on its relationship with the fine-tuning technique often employed in practice.  
%and how it was compared with other approaches.   

\begin{table*}[htb]
\caption{Brier scores of different calibration methods}
\centering
% \setlength{\tabcolsep}{.38em}
\begin{threeparttable}
\begin{tabular}{|p{0.6cm}<{\centering}|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}*{\textbf{Task}} & \multirow{2}*{\textbf{Model}} & \multirow{2}*{\textbf{Orig.}} & \multicolumn{3}{c|}{\textbf{Operational calibration}} & \multicolumn{4}{c|}{\textbf{Conventional calibration}} & \multirow{2}*{\textbf{SAR}}  \\
\cline{4-10} 
  & & & \textbf{GPR} & \textbf{RFR} & \textbf{SVR} & \textbf{TS} & \added{\textbf{PS-conf.}} & \added{\textbf{PS-logit}} & \added{\textbf{IR}} &   \\
\hhline{|===========|}
1  & LeNet-5 & 0.207 & \textbf{0.114} & 0.126 & 0.163 & 0.183 & \added{0.316}  & \added{0.182} & \added{0.320} & 0.320 \\
\hline
2  & RNN & 0.203 & \textbf{0.102} & 0.107 & 0.202 & 0.185 & \added{0.641} & \added{0.125} & \added{0.655} & 0.175 \\
\hline %\hhline{|======|}
3  & ResNet-18 & 0.474 & \textbf{0.101} & 0.121 & 0.115 & 0.387 & \added{0.471} & \added{0.254} & \added{0.529} & 0.308 \\
\hline
4  & VGG-19 & 0.216 & \textbf{0.158} & 0.162 & 0.170 & 0.217 & \added{0.359}  & \added{0.253} & \added{0.364}  & 0.529 \\
\hline
5  & ResNet-50 & 0.226 & \textbf{0.179} & 0.204 & 0.245 & 0.556 & \added{0.789}  & \added{0.319} & \added{0.925}  & 0.364 \\
\hline
6  & Inception-v3 & 0.192 & \textbf{0.161} & 0.167 & 0.217 & 0.191 & \added{0.546} & \added{0.427} &  \added{0.334} & - \\
\hline
\end{tabular}
 \begin{tablenotes}
        \footnotesize
        \item 	Orig.--Before calibration. 
        		GPR--Gaussian Process-based approach.
				RFR--Random Forest Regression in the representation space.
				SVR--Support Vector Regression in the representation space.
				TS--Temperature Scaling~\cite{guo2017calibration}.
				\added{PS--Platt Scaling~\cite{Platt1999probabilisticoutputs}.
				IR--Isotonic Regression Scaling~\cite{zadrozny2002transforming}.
				Conf./Logit indicates that the calibration took confidence value/logit as input. }
				SAR--Regression with Surprise values~\cite{kim2019guiding}.
				We failed to evaluate SAR on task 6 because it took too long to run on the huge dataset.
  \end{tablenotes}
\end{threeparttable}
\label{tab:brier-score}
\end{table*}


\subsubsection{Calibration when fine-tuning is ineffective}

A machine learning engineer might first consider to apply 
fine-tuning tricks to deal with the problem of domain shift. 
However, for non-trivial tasks, such as our tasks 4, 5, and 6,
it can be very difficult, if possible, to fine-tune the DNN model 
with small operation datasets. 
Figure~\ref{fig:fine-tune1} shows the vain effort in fine-tuning 
the models with all the operation data (excluding test data). 
We tried all tricks including data augmentation, weight decay, and regularization 
to avoid over-fitting but failed to improve the test accuracy.  

\begin{figure*}[htbp]
\begin{center}
\subfloat[Task 4]{
\includegraphics[width=0.62\columnwidth]{figures/learn-curve/cifar100.pdf}}
\subfloat[Task 5]{
\includegraphics[width=0.62\columnwidth]{figures/learn-curve/imageclef.pdf}}
\subfloat[Task 6]{
\includegraphics[width=0.62\columnwidth]{figures/learn-curve/imagenet.pdf}}
\caption{Ineffective fine-tuning of difficult tasks.
\added{\rm{All available operation data (5000, 480, and 5000, respectively) were used. }}}
\label{fig:fine-tune1}
\end{center}
\end{figure*}

Fortunately, our operational calibration worked quite well in these difficult situations. 
In addition to the improvement in Brier scores reported in Table~\ref{tab:brier-score}, 
we can also see the saving of LCE for task~4 in Figure~\ref{fig:LCE-1} as an example. 
Our approach reduced about a half of the LCE when $\lambda > 0.8$, 
which indicates its capability in reducing high confidence errors.   

%
%For 
%\emph{fine-tune technique with \textbf{***xjw::limited dataset***} could not 
%increase the accuracy of model on the specific operation domain}.
%We confirm this point through the following experiments:
%we employ the whole operation set for calibration 
%to fine-tune the model previously trained on original domain.
%Due to the small size of operation data, 
%data augmentation, weight decay, and regularization 
%are all applied to avoid over-fitting.
%The experimental results are shown in Figure~\ref{fig:fine-tune1}.
%For task 4 and task 5, 
%that models quickly overfit to the the limited operation datasets.
%However, the accuracy of operation domain even decline slightly. 
%For the last task, in addition to the difficulty of the dataset (e.g.,~ImageNet), 
%the operation of down-sampling has lost much information from original image.
%Thus it is hard for the model to learn knowledge from such operational images.
%
%Although the fine-tuning technique does not work well in such tasks, 
%our calibration approach can still correct the corresponding confidence to 
%improve the decision quality of DNN. 
%The experimental results in Table~\ref{tab:brier-score} prove this claim. 
%The brier scores~\textbf{***xjw::add Equation number***} for these three tasks descend  
%from 0.216 to 0.158, 0.226 to 0.179, and 0.191 to 0.161, respectively.
%It is worth noting that even for the ImageNet dataset, which is the most difficult task, 
%the calibration still be effective 
%, but its benefit brought by calibration is small 
%due to the large number of classes. 
%To evaluate the profit from decreasing the brier score, 
%we compute the LCE with different $u/(1+u)$ for task 4.
%For details, we choose $u/(1+u)$ from 0.05 to 0.95 with interval 0.05 
%to calculate how much LCE can be reduced by our approach 
%under the different loss $u$. 
%The experimental results are provided in Figure~\ref{fig:LCE-1}.
%When the loss for false prediction is small 
%(e.g., $u = 1/9$), 
%our calibration approach could not save loss in this situation.
%However, when the loss for prediction is large
%(e.g., $u = 9$),  
%the calibration approach shows amazing effect:
%the calibration approach can nearly save 60\% loss per input. 
%\textbf{***xjw::add several sentences to discuss other compared methods***}




\begin{figure}[htbp]
\begin{center}
\includegraphics[width=0.70\columnwidth]{figures/LCE/cifar100.pdf}
\caption{loss due to confidence error}
\label{fig:LCE-1}
\end{center}
\end{figure}


%\begin{figure*}[htbp]
%\begin{center}
%\subfloat[Vgg19~(cifar-100 $\rightarrow$ affine transformation)]{
%\includegraphics[width=0.7\columnwidth]{figures/efficacy/cifar100.pdf}} 
%\subfloat[ResNet-50~(imageclef-c $\rightarrow$ imageclef-p)]{
%\includegraphics[width=0.7\columnwidth]{figures/efficacy/imageclef.pdf}}
%\subfloat[Inception-v3~(imagenet $\rightarrow$ down-sample)]{
%\includegraphics[width=0.7\columnwidth]{figures/efficacy/imagenet.pdf}} 
%\caption{loss due to confidence error}
%\label{fig::LCE-1}
%\end{center}
%\end{figure*}

%\begin{figure*}[htbp]
%\begin{center}
%\subfloat[LeNet-5~(mnist $\rightarrow$ usps)]{
%\includegraphics[width=1\columnwidth]{figures/efficacy/mnist.pdf}}
%\subfloat[RNN~(Polarity-v1.0 $\rightarrow$ Polarity-v2.0)]{
%\includegraphics[width=1\columnwidth]{figures/efficacy/polarity.pdf}} \\
%\subfloat[ResNet-18~(cifar-10 $\rightarrow$ stl-10)]{
%\includegraphics[width=1\columnwidth]{figures/efficacy/cifar10.pdf}}
%\caption{loss due to confidence error}
%\label{fig::LCE-2}
%\end{center}
%\end{figure*}


\subsubsection{Calibration when fine-tuning is effective}

In case of easier situations that fine-tuning works, 
we can still calibrate the model to give more accurate confidence. 
Note that effective fine-tuning does not necessarily provide accurate confidence. 
One can first apply fine-tuning until test accuracy does not increase, 
and then calibrate the fine-tuned model with the rest operation data.  


For example, we managed to fine-tune the models in our tasks 1, 2, and 3.~\footnote{%
Here we used some information of the training process, such as the learning rates, weight decays and training epochs. Fine-tuning could be more difficult because these information could be unavailable in real-world operation settings.  
} 
Task 1 was the easiest to fine-tune and its accuracy kept increasing 
and exhausted all the 900 operational examples.
Task 2 was binary classification, in this case our calibration was actual 
an effective fine-tuning technique. 
Figure~\ref{fig:ft-cali2} shows that our approach was 
more effective and efficient than conventional fine-tuning as it converged more quickly. 
For task 3 with fine-tuning the accuracy stopped increasing at about 79\%, 
with about 3,000 operational examples.  
Figure~\ref{fig:ft-cali3} show that, 
the Brier score would decrease more if we spent rest operation data on calibration 
than continuing on the fine-tuning. 


\begin{figure}[htbp]
\begin{center}
\subfloat[\added{Task 2}]{
\includegraphics[width=0.5\columnwidth]{figures/brier-score/polarity.pdf}
\label{fig:ft-cali2}}
\subfloat[\added{Task 3}]{
\includegraphics[width=0.5\columnwidth]{figures/brier-score/cifar10.pdf}
\label{fig:ft-cali3}}
\caption{Calibration when fine-tuning is effective}
\end{center}
\end{figure}

%\begin{figure}[htbp]
%\begin{center}
%\includegraphics[width=0.45\columnwidth]{figures/brier-score/polarity.pdf}
%\caption{Operational calibration vs. Fine-tuning: Task 2}
%\label{fig:ft-cali2}
%\end{center}
%\end{figure}
%
%\begin{figure}[htbp]
%\begin{center}
%\includegraphics[width=0.45\columnwidth]{figures/brier-score/cifar10.pdf}
%\caption{Operational calibration after fine-tuning: Task 3}
%\label{fig:ft-cali3}
%\end{center}
%\end{figure}


Based on the significant (16.1\%-78.6\%) reductions in Brier scores in all of the tasks reported in Table~\ref{tab:brier-score} and the above discussions,
we conclude that \emph{the Gaussian Process-based approach to operational calibration
is generally effective, 
and it is worthwhile no matter whether the fine-tuning works or not}.  


%\begin{figure*}[htbp]
%\begin{center}
%%\subfloat[Task-1]{
%%\includegraphics[width=0.7\columnwidth]{figures/brier-score/mnist.pdf}}
%\subfloat[Task-2]{
%\includegraphics[width=1.0\columnwidth]{figures/brier-score/polarity.pdf}}
%\subfloat[Task-3]{
%\includegraphics[width=1.0\columnwidth]{figures/brier-score/cifar10.pdf}}
%\caption{The calibrated brier score of fine-tuned model}
%\label{fig:ft-cali}
%\end{center}
%\end{figure*}
%
%
%
%
%
%\begin{figure*}[htbp]
%\begin{center}
%\subfloat[Task-1]{
%\includegraphics[width=0.7\columnwidth]{figures/learn-curve/mnist.pdf}}
%\subfloat[Task-2]{
%\includegraphics[width=0.7\columnwidth]{figures/learn-curve/polarity.pdf}}
%\subfloat[Task-3]{
%\includegraphics[width=0.7\columnwidth]{figures/learn-curve/cifar10.pdf}}
%\caption{The fine-tuning of simple tasks}
%\label{fig:fine-tune2}
%\end{center}
%\end{figure*}
%
%
%In addition, for the first three tasks where fine-tuning method could work well, 
%it is difficult to choose the parameters (e.g., learning rate, weight decay, etc.).
%If the user 
%lacks the prior knowledge of training process or 
%some understandings of fine-tuning technique, 
%the fine-tuning may still be useless 
%and even decrease the accuracy of model.
%Furthermore, 
%in some situation, 
%it is not permitted to modify the model, e.g., 
%the model my be provided as a web service, 
%we could only get the limited information (e.g., outputs from last and/or penultimate layers) returned from the service.
%When we target to operation domain, the only thing we can do is to calibrate these outputs.
%%they need to finish the ensemble learning tasks 
%%or they will reuse the model in the future.
%In this part, we apply calibration without fine-tuning for the first three relatively simple tasks.
%The experimental results are shown in Table~\ref{tab:brier-score}, 
%The brier scores decrease from 0.207, 0.203, and 0.474 to 0.114, 0.102, and 0.101, respectively.
%\textbf{***xjw::add several sentences to discuss other compared methods***}
%% Above all, 
%
%
%
%
%
%As we discussed earlier, for relatively simple tasks (i.e., task 1, task 2, and task3),
%\emph{fine-tuning method is able to increase the accuracy of model on operation domain}. 
%However, the increasing of accuracy does not mean that 
%the reliability of confidence is also improved.
%In other words, fine-tuning could not ensure the model well-calibrated.
%Thus, the confidence calibration is still needed in this situation.
%In order to calibrate confidence after fine-tuning,
%we hold out a small proportion of data for calibration.
%%For given sample size, instead of use the whole datasets for fine-tuning, 
%For details, we first run fine-tuning to make 
%the accuracy of the model nearly convergence, 
%and then start calibration to further reduce the brier score.
%Taking task 3 as an example,  
%we find that when the sample size exceeds 3,000, 
%there is no significant improvement for fine-tuning by further applying samples.
%Therefore, we use the remaining samples to calibrate the fine-tuned model.
%The brier score of calibration for fine-tuned model are plotted in Figure~\ref{fig:calibration+fine-tune}. 
%For task 2, we also should calibrate the model after fine-tuning, 
%but this task is a two-class classification problem, 
%thus calibration is equivalent to fine-tuning. 
%In this sense, we directly compare the calibration and fine-tuning, 
%From Figure~\ref{fig:calibration+fine-tune} we find that our gaussian process calibration 
%can converge faster to final brier score than fine-tuning does. 
%Using only 150 samples can achieve the same performance of fine-tuning with 1,000 samples.
%We think that the reason of such novel efficiency is 
%due to our calibration method makes full use of 
%the representative ability of the model 
%so that can use less samples but achieve same brier score.
%For task 1, we find that the accuracy is still increasing when adding more samples for fine-tuning. 
%In this situation, we recommend user continuing fine-tuning the model until the accuracy convergence.
%
%\begin{figure*}[htbp]
%\begin{center}
%%\subfloat[Task-1]{
%%\includegraphics[width=0.7\columnwidth]{figures/brier-score/mnist.pdf}}
%\subfloat[Task-2]{
%\includegraphics[width=1.0\columnwidth]{figures/brier-score/polarity.pdf}}
%\subfloat[Task-3]{
%\includegraphics[width=1.0\columnwidth]{figures/brier-score/cifar10.pdf}}
%\caption{The calibrated brier score of fine-tuned model}
%\label{fig:fine-tune3}
%\end{center}
%\end{figure*}
%

\subsection{Comparing with alternative methods}

\added{First, we applied three widely used calibration methods, \emph{viz.} Temperature Scaling (TS)~\cite{hinton2015distilling}, 
Platt Scaling (PS)~\cite{Platt1999probabilisticoutputs}, and Isotonic Regression (IR)~\cite{zadrozny2002transforming},
with the same operation data used in our approach.
%
TS defines the calibration function $R$ in Equation~\ref{equ:logitcali} as $R(\bm{h}) = \bm{h}/T$,  
where $T$ is a scalar parameter computed by minimizing the 
negative log likelihood~\cite{hastie2009elements}
on a validation dataset. 
PS and IR directly work on the confidence values. 
PS trains a one-dimensional logistic regression and calibrates confidence 
as $\hat{c} = 1/(1+e^{-a\cdot c_{\mathfrak{M}}+b})$, 
where $a, b$ are scalar parameters computed by minimizing the cross entropy on a validation dataset.
IR simply fits a monotonic confidence calibration function minimizing 
the Brier score on a validation dataset. 
Note that in our experiment, the operation data were used instead of the validated dataset. 
We implemented TS according to~\citet{guo2017calibration}. For PS and IR we used the
well-known machine learning library scikit-learn~\cite{scikit-learn}.
} 


%\footnote{\added{These two methods have been well developed in machine learning library scikit-learn~\cite{scikit-learn}, one can refer to sklearn.calibration.CalibratedClassifierCV.}}


% There exist different kinds of calibration methods, such as isotonic regression~\cite{zadrozny2002transforming}, 
% histogram binning~\cite{zadrozny2002transforming}, and Platt scaling~\cite{Platt1999probabilisticoutputs}. 
% \added{These methods all attempt to train a regression model whose input is confidence. 
% The first two methods are implemented based on isotonic regression and binning, and the last method define the calibration function as}
% \begin{equation}
% \added{R(c) = \frac{1}{1+e^{-(a \cdot c + b)}},}
% \end{equation}
% \added{where $c$ is the input of confidence value, and $a, b$ are parameter computed by minimizing the cross entropy on the validation dataset. }
% However, according to a recent study~\cite{guo2017calibration}, 
% the most effective choice is often a simple method called Temperatures Scaling~\cite{hinton2015distilling}.
% The idea is to define the calibration function as
%  \begin{equation}
%  R(\bm{h}) = \frac{\bm{h}}{T}, 
%  \end{equation}
% where $T$ is a scalar parameter computed by minimizing the 
% negative log likelihood~\cite{hastie2009elements}
% on the validation dataset. 
% \added{Moreover, Platt scaling can also be improved through taking logit as input~\cite{guo2017calibration}, i.e., define the calibration function as}
%  \begin{equation}
%  \added{R(\bm{h}) = \bm{W}^{\mathsf{T}}\bm{h}+\bm{b}, }
%  \end{equation}
%  \added{where $\bm{W}$ is a matrix parameter and $\bm{b}$ is a vector parameter. 
%  Both of these two parameters are computed by minimizing the cross entropy. }


%First, Temperature Scaling~\cite{hinton2015distilling}, which is reported to be the most effective conventional confidence calibration method~\cite{guo2017calibration}, was applied with the same operation data used in our approach.
As shown in Table~\ref{tab:brier-score}, TS, 
although reported to be usually the most effective conventional confidence calibration method~\cite{guo2017calibration},
was hardly effective in these cases. 
It even worsened the confidence in tasks 4 and 5. 
We observed that its bad performance  
came from the significantly lowered resolution part of the Brier score, 
which confirmed the analysis in Section~\ref{subsec:discussions}.
For example, in task 3, with Temperature Scaling the reliability decreased from 0.196 to 0.138, but the resolution dropped from 0.014 to 0.0. 
In fact, in this case the calibrated confidence values were all very closed to 0.5 after scaling. 
However, with our approach the reliability decreased to 0.107,
and the resolution also increased to 0.154. 
\added{The same reason also failed PS (col. PS-Conf.) and IR (col. IR).}

\added{We also included in our comparison an improved version of PS, which built 
a regression over the logit instead of the confidence~\cite{guo2017calibration}. 
Its calibration function $R$ for Equation~\ref{equ:logitcali} was
$R(\bm{h}) = \bm{W}^\mathsf{T} \bm{h} + \bm{b}$,
where $\bm{W}$  and $\bm{b}$ were 
computed by minimizing the cross entropy on the operation data. 
It performed much better than the original PS but 
still failed in tasks 4, 5 and 6.
}

% \added{, be ineffective in operation domain. 
% The details were shown in Table~\ref{tab:brier-score} (col. PS and col.IR). 
% Since the calibration effect is too poor, we tried to improve these two methods, i.e., taking logit as calibration input. 
% The experimental results are available in Table~\ref{tab:brier-score} (col. IPS and col.IIR) }

Second, we also tried to calibrate confidence based on the Surprise value 
that measured the difference in DL system's behavior 
between the input and the training data~\cite{kim2019guiding}.
We thought it could be effective because it also leveraged the distribution of examples 
in the representation space.
We made polynomial regression between the confidence adjustments and the likelihood-based Surprise values. 
Unfortunately, it did not work for most of the cases (col. SAR in Table~\ref{tab:brier-score} ). 
We believe the reason is that Surprise values are scalars 
and cannot provide enough information for operational calibration.  

Finally, to examine whether Gaussian Process Regression (GPR) is the right choice for our operational calibration framework, 
we also experimented with two standard regression methods, viz. 
Random Forest Regression (RFR) and Support Vector Regression (SVR). 
We used linear kernel for SVR and ten decision trees for RFR.
As shown in Table~\ref{tab:brier-score}, in most cases, the non-liner RFR performed better than the linear SVR, 
and both of them performed better than Temperature Scaling but worse than GPR.
The result indicates that (1) calibration based on the features extracted by the model 
rather than the logits computed by the model is crucial, 
(2) the confidence error is non-linear and unsystematic,   
and (3) the Gaussian Process as a Bayesian method can provide better estimation of the confidence. 


In summary, \replaced{our GPR approach achieved significant Brier Score reduction and outperformed 
conventional calibration methods and the Surprise value-base regression in all the tasks.}{
the Brier score reductions of our GPR approach were       
at least 3.87 times of that of Temperature Scaling and 2.24 times of Surprise value-base regression.} 
It also outperformed alternative implementations based on RFR and SVR. 
So we conclude that 
 \emph{our approach is more effective than Temperature Scaling and 
other alternative choices for operational calibration}.

%
%We also compared our approach with (1) 
%
%Here we compare our calibration approach with other DNN quality assurance methods.
%Following the temperature scaling which is the state-of-art calibration technique in machine learning,
%the surprise adequacy was applied to ensure the confidence accurate on operation domain.
%Finally, we explain the rationale of choosing gaussian process through comparing with other regression techniques.
%
%Researchers have proposed many methods to ensure the quality of models~\cite{XXX} in last years. 
%We want to know whether our method outperforms the other DNN quality assurance methods.  
%In this evaluation, we compare our calibration approach with two state-of-the-art methods, 
%i.e., temperature scaling and surprise adequacy.
%
%For surprise adequacy method, we choose 
%likelihood-based surprise adequacy (i.e., LSA)
%as the measurement for surprise value of operation data. 
%Notice that the original data must be available for computing the surprise value.
%Thus we provide the original data for this method.
%Because the output of LSA is scalar, 
%we use polynomial regression to calibrate the confidence: 
%the input of regression is surprise value 
%and the output of regression is the confidence difference.
%
%
%The experiments are conducted on all datasets except ImageNet due to the extremely large original dataset.
%As we can see, the results show that the LSA method is not able to 
%
%
%capture the confidence changes on the operation domain. 
%We think the reason for ineffectiveness is that
%the operation data are all surprises compared with original data.
%\textbf{***where is temperature scaling?***}
%
%Besides from the above methods, 
%we also conduct some experiments to show the rationality of gaussian process. 
%Specifically, 
%we apply Random Forest (RF) and Support Vector Regression (SVR) as the compared methods
%to calibrate the confidence. 
%In evaluation, we choose linear kernel for SVR and ten decision trees for RF.
%The experimental results are shown in Table~\ref{brier-score}. 
%We can see that linear regression methods (e.g., linear SVR) 
%cannot describe the changes of confidence on operation domain effectively. 
%The non-linear regression method can capture some changes, 
%but such tree model cannot learn the locality of inputs in representation space suitably\textbf{***stablely?***}. 
%Notice that
%the dimension of representation space is still too high 
%for such regression methods, 
%which leads training process very time-consuming
%compared to non-parametric gaussian process.

\subsection{Efficiency of operational calibration}

In the above we have already shown that our approach worked with 
small operation datasets that were insufficient for fine-tuning (Task 4, 5, and 6). 
In fact, the Gaussian Process-based approach has a nice property 
that it starts to work with very few labeled examples. 
We experimented the approach with the input selection method presented in Section~\ref{subsec:inputselection}.
We focused on the number of high-confidence false predictions, which 
was decreasing as more and more operational examples were labeled and used.  

We experimented with all the tasks but labeled only 10\% of the operation data. 
Table~\ref{tab:efficiency-results} shows the numbers of high-confidence false predictions 
before and after operational calibration. 
As a reference, we also include the numbers of high-confidence correct predictions. 
We can see that most of the high-confidence false predictions were eliminated. 
It is expected that there were less high-confidence correct predictions after calibration, 
because the actual accuracy of the models dropped. 
The much lowered LCE scores, which took into account 
both the loss in lowering the confidence of correct predictions and the gain in lowering the confidence of false predictions, 
 indicate that the overall improvements were significant.  

\begin{table}[htb]
\caption{Reducing high-confidence false predictions with 10\% operation data labeled}
\centering
\setlength{\tabcolsep}{.38em}
\begin{threeparttable}
\begin{tabular}{|p{0.4cm}<{\centering}|p{1.2cm}<{\centering}|c|c|c|c|c|}
\hline
No. & Model & $\lambda$ & Correct pred. & False pred. & LCE \\
\hhline{|======|}
\multirow{2}*{1} & \multirow{2}*{LeNet-5} & 0.8 & 473 $\rightarrow$ 309.1 & \textbf{126$\rightarrow$24.3} & 0.143$\rightarrow$0.089  \\
&  &  0.9  & 417 $\rightarrow$ 141.9 & \textbf{74 $\rightarrow$ 2.5} & 0.096$\rightarrow$0.055 \\
\hline
\multirow{2}*{2} & \multirow{2}*{RNN} & 0.8 & 512 $\rightarrow$ 552.9 & \textbf{118$\rightarrow$39.9} & 0.162$\rightarrow$0.091  \\
&  &  0.9  & 482 $\rightarrow$ 261.3 & \textbf{106 $\rightarrow$12.0} & 0.132$\rightarrow$0.070 \\
\hline
\multirow{2}*{3} & {ResNet} & 0.8 & 1350 $\rightarrow$ 839.2 & \textbf{1372$\rightarrow$59.7} & 0.370$\rightarrow$0.054  \\
& {-18}  &  0.9  & 1314 $\rightarrow$ 424.0 & \textbf{1263 $\rightarrow$9.4} & 0.358$\rightarrow$0.041 \\
\hline
\multirow{2}*{4} & \multirow{2}*{VGG-19} & 0.8 & 1105 $\rightarrow$ 392.5 & \textbf{583$\rightarrow$46.9} & 0.127$\rightarrow$0.070 \\
& &  0.9  & 772$\rightarrow$142.8  & \textbf{280$\rightarrow$9.3} & 0.074$\rightarrow$0.038 \\
\hline
\multirow{2}*{5} & {ResNet} & 0.8 & 53 $\rightarrow$ 26.9 & \textbf{16$\rightarrow$5.2} & 0.162$\rightarrow$0.136  \\
& {-50} &  0.9  & 46 $\rightarrow$ 26.9 &\textbf{10$\rightarrow$2.0} & 0.108$\rightarrow$0.064 \\
\hline
\multirow{2}*{6} & {Inception} & 0.8 & 1160$\rightarrow$692.0 & \textbf{265$\rightarrow$63.6} & 0.087$\rightarrow$0.073 \\
& {-v3} & 0.9 & 801$\rightarrow$554.1 & \textbf{137 $\rightarrow$ 40.2} & 0.054$\rightarrow$0.041 \\
\hline
\end{tabular}
 \begin{tablenotes}
        \footnotesize
        \item %To obtain the statistical results, 
        		We ran each experiment 10 times and computed the average numbers.% numbers of correct predictions and false 		          predictions.
  \end{tablenotes}
\end{threeparttable}
\label{tab:efficiency-results}

\end{table}


For a visual illustration of the efficiency of our approach, 
Figure~\ref{fig:efficiency-curve}  plots the change of proportions of 
high-confidence false and correct predictions as the size of data used in calibration increases. %Task 3.  
%Other tasks are similar and omitted here to save space. 
It is interesting to see that: 
(1) most of the high-confidence false predictions were identified very quickly, and
(2) the approach was conservative, 
but the conservativeness is gradually remedied with more labeled operation data used. 

\begin{figure}[htbp]
\begin{center}
\subfloat[Task 1]{
\includegraphics[width=0.5\columnwidth]{figures/efficiency/mnist/0dot9.pdf}}
\subfloat[Task 2]{
\includegraphics[width=0.5\columnwidth]{figures/efficiency/polarity/0dot9.pdf}}

\vspace{-2ex}
\subfloat[Task 3]{
\includegraphics[width=0.5\columnwidth]{figures/efficiency/cifar10/0dot9.pdf}}
\subfloat[Task 4]{
\includegraphics[width=0.5\columnwidth]{figures/efficiency/cifar100/0dot9.pdf}}

\vspace{-2ex}
\subfloat[Task 5]{
\includegraphics[width=0.5\columnwidth]{figures/efficiency/imageclef/0dot9.pdf}}
\subfloat[Task 6]{
\includegraphics[width=0.5\columnwidth]{figures/efficiency/imagenet/0dot9.pdf}}
\caption{The proportion curve of high confidence inputs.
\added{\rm{Sample size 0 means uncalibrated. The calibration started to take effect with very few data.}}}
\label{fig:efficiency-curve}
\end{center}
\end{figure}

Note that for tasks 4, 5 and 6, 
usual fine-tuning tricks did not work even with all the operation data labeled.
With our operational calibration, using only about 10\% of the data, 
we avoided about 97\%, 80\%, and 71\% high-confidence ($>$$0.9$) errors, respectively.

Based on the results, we can say that \emph{the Gaussian Process-based operational calibration 
is efficient in detecting most of the high-confidence errors with a small amount of labeled operation data}. 


%
%
%
%Here we evaluate our operational calibration method in terms of
%calibrating the high confident misclassifications.
%In evaluation, 
%we respectively set the confidence threshold as 0.8 and 0.9.
%In other words, we are more inclined to calibrate the inputs 
%whose confidences are greater than 0.8 and 0.9.
%We conduct the experiments for all tasks, 
%due to the page limitation, we only plot the experimental results of task 4 in Figure~\ref{fig:efficiency-curve}. 
%The blue line is the proportion of 
%inputs with high confidence to total inputs, 
%and the red line is the proportion of 
%misclassified inputs with high confidence to total inputs.
%The results show that our calibration approach
%nearly reduces 60\% of inputs with high confidence.
%We think it is an acceptable result,
%because the accuracy is dropped on operation domain.
%At the same time, the high confidence dropped nearly 90\%, 
%only a few inputs are misclassified with high confidence.
%
%
%
%In addition, we only use 10\% of the whole inputs for labeling 
%and build the gaussian process. 
%Then the number of high confidence false predictions 
%and high confidence correct predictions are counted respectively.
%The detailed results are provided in Table~\ref{tab:efficiency-results}.
%
%There is no exact specification for the optimal number of inputs with high confidences, 
%let alone the number of misclassified inputs with high confidences.
%Thus we could only use the LCE as the specification, which is also recorded in Table~\ref{tab:efficiency-results}. 
%
%As shown in Table~\ref{tab:efficiency-results}, we can conclude that our calibration method is very efficient. 
%With a few samples to building gaussian process, in relative simple tasks (i.e., task 1,2, and 3), 
%we can reduce about 90\% of misclassified inputs whose confideces are greater than 0.9, 
%and reduce at least 80\% of misclassified inputs whose confidences are greater than 0.8.
%In the rest complex tasks (i.e., 4,5 and 6), 




==> OptConfPaper/introduction.tex <==
% !TEX root = main.tex

\section{Introduction}
Deep learning (DL) has achieved human-level or even better performance in some difficult tasks, 
such as image classification and speech recognition~\cite{LeCun:2015aa, Goodfellow-et-al-2016}.
Deep Neural Network (DNN) models are increasingly adopted in high-stakes application scenarios such as medical diagnostics~\cite{obermeyer2016predicting} and self-driven cars~\cite{bojarski2016selfdriven}. 
However, it is not uncommon that DNN models perform poorly in practice~\cite{Riley2019nature}.
The interest in the quality assurance for DNN models as integral parts of software systems 
is surging in the community of software engineering~\cite{pei2017deepxplore, ma2018combinatorial, sun2018concolic, zhang2018deeproad, kim2019guiding, zhang2019surveyMLT}.


%one reason for machine learning misprediction bugs is no or poor calibration. This paper proposes an approach to debug this types of bugs via operational calibration. 

%Different from human written programs, a DNN model is intrinsically uncertain, 
%and it never promises to produce a definitely correct output (prediction) for an input.
%So individual incorrect outputs are not necessarily bugs. 
%However, besides the prediction for an input, 
%the model also provide a confidence value that 
%quantifies the likelihood of correctness for this prediction.   
%Accurate confidence information is important in real-wold decision making~\cite{guo2017calibration}.
%%A model with its confidence well calibrated for a given operation domain
%%knows when it works well and when not, and reduces the loss due to over- and under-confidence in decisions.
%For example, an over-confident benign prediction for a pathology image 
%could mislead a doctor into overlooking a malignant tumor, 
%while an under-confident benign prediction could result in unnecessary confirmatory testings. 
%\textcolor{red}{



\deleted{
While machine learning is primarily concerned with how well a model learns from its training data, 
software engineering must pay more attention to how well the trained model performs in the field.
This means that the quality assurance of DNN models used as software components needs to be \emph{operational}. 
In addition, it needs to be \emph{stochastic} to embrace the intrinsic uncertainty of the models 
and \emph{effective} to best utilize the effort in collecting and labeling operation data. 
}

A particular problem of using a previously \added{well-}trained DNN model in an operation domain is that 
the model may not only make more-than-expected mistakes in its predictions,  
but also give erroneous confidence values for these predictions. 
\deleted{Arguably the} \added{The} latter issue is \deleted{more harmful} \added{particularly problematic for decision making}, 
because if the confidence values were accurate, the model would be at least partially usable by accepting only high-confidence predictions.   
It needs to be emphasized that erroneous  predictions with high confidence are especially damaging 
because users will take high stakes in them. 
For example, an over-confident benign prediction for a pathology image 
could mislead a doctor into overlooking a malignant tumor.

The problem comes from the almost inevitable divergences between 
the original data on which a model is trained and the actual data in its operation domain,
which is often called \emph{domain shift} or \emph{dataset shift}~\cite{ng2016nuts}
 in the machine learning literature.
%The popular machine learning tricks (e.g., fine-tuning,  transfer learning~\cite{pan2009survey,wang14icml}, etc.) is difficult to solve this problem due to two practical restrictions in field:
It can be difficult and go beyond the stretch of usual machine learning tricks 
such as fine-tuning and transfer learning~\cite{pan2009survey,wang14icml}, 
because of two practical restrictions often encountered. 
First, %when a DNN model is provided by a third party, 
%its training data are sometimes 
the training data of a third-party DNN model are often
unavailable due to privacy and proprietary limitations~\cite{zhou2016learnware, Shokri2015CCS, konevcny2016federated}.
Second, one can only use a small number of labeled operation data 
because it could be very expensive to label the data collected in the field. 
For example, in an AI-assisted clinical medicine scenario, 
surgical biopsies may have to be involved in the labeling of radiology images.




%However, due to the fundamental difference between DNN models and human written programs,  
 
 
 
%Considering the inductive nature of deep learning~\cite{Goodfellow-et-al-2016}, 
%an essential problem %of adopting well trained DNN models as integral parts of practical software systems 
%is that DNN models might not work as well as expected under field conditions, 
%because the slight distribution divergences almost always exist between  
%the training data and the operation data in field. 
%The phenomena is usually called domain shift or dataset shift in the machine learning literature. 
%%
%The problem can be difficult and goes beyond the stretch of usual machine learning tricks 
%such as fine-tuning and transfer learning~\cite{pan2009survey,wang14icml} because of two practical 
%restrictions often encountered. First, the DNN model is provided by a third party, 
%and its training data are unavailable due to privacy and proprietary limitations~\cite{zhou2016learnware, Shokri2015CCS, konevcny2016federated}.
%Second, one can only use a small number of labeled operation data, 
%because it is expensive to label the data collected in field. 
%For example, in an AI-aided clinical medicine scenario, 
%surgical biopsies could be involved in the labeling of radiology or pathology images.

%Despite these stringent restrictions, 
%From a software engineering perspective, it is crucial  
%to know quantitatively \emph{how well} a DNN model will work in a given operation domain. 
%In this paper we focus on classifiers. 
%The ``how-well'' is characterized not only collectively with metrics such as model accuracy or precision, 
%but also individually with the \emph{confidence} for the prediction on each given input,  
%which estimates the likelihood of correctness for this prediction. 
% 
%Recently, Li et al proposed an efficient approach to the \emph{operational testing} of DNNs that significantly
%reduces the labeling cost in estimating a model's \emph{overall} operational accuracy~\cite{li2019boosting}. 
%Different from this operational testing, 


We consider \emph{operational calibration} 
that corrects the error in the confidence provided by a DNN model 
for its prediction on each input in a given operation domain. 
It does not change the predictions themselves  
%but fixes the erroneous confidence to the correct one.
but tells when the model works well and when not.
\added{As the quantification of the intrinsic uncertainty in the predictions made by a model, 
confidence values are integral parts of the model's outputs.
So operational calibration can be viewed as a kind of \emph{debugging} activity 
that identifies and fixes errors in these parts of model outputs. 
It improves the model's quality of service in the field 
with more accurate confidence for better decision making. } 
%
\replaced{As a quality assurance activity, operational calibration 
shall be carried out during the deployment of a previously trained DNN model 
in a new operation domain.
One can also incorporate it into the system and excise it from time to time to adapt 
the model to the evolving data distribution in the operation domain.
}{In this sense, operational calibration is a necessary debugging step 
%for fixing confidence errors
that should be incorporated in the engineering of the whole system. 
It fits a perviously trained DNN model to its operational domain with calibrated confidence for better decision making.  
Also, one can incorporate it into the system and excise it at runtime to continuously adapt to the evolutions in the operation domain.
} 
\deleted{We note that operational calibration is challenging because what it fixes is a function, not just a value.} 
%It also needs to be %effective, i.e., improving the accuracy of confidence values, and 
%efficient, i.e., reducing the effort in labeling operation data. 
%It is related to, but different from, the confidence calibration 
%extensively studied in the machine learning community~\cite{flach2016calibration, guo2017calibration}. 
%As to be discussed in Section~\ref{sec:problem} and evaluated in Section~\ref{sec:evaluation}, 
%existing confidence calibration methods are not targeted at specific operation domains 
%and ineffective for our purpose. 









It is natural to model operational calibration as a \added{case} \deleted{kind} of non-parametric Bayesian Inference 
and solve it with Gaussian Process Regression~\cite{rasmussen2005GPML}.  
We take the original confidence of a DNN model as the prior, 
and gradually calibrate the confidence with the evidence collected by selecting and labeling operation data. 
The key insight into effective and efficient regression comes from two observations:
First, the DNN model, although suffering from the domain shift, %the distribution divergence between operation and training data,
can be used as a feature extractor with which unlabeled operation data
can be nicely clustered~\cite{zhu2005semi, shu2018a}. 
In each cluster, the prediction correctness of an example is correlated with another one. 
The correlation can be effectively estimated with the distance of the two examples in the feature space.
Second, Gaussian Process is able to quantify the uncertainty after each step, 
%Notice that the advantage of Gaussian Process is to quantify the uncertainty after each step, 
which can be used to guide the selection of operation data to label efficiently. 
%and those examples that will reduce the highest uncertainty will be selected labeled for next step. 
%In this way the efficiency of approach is further improved. 

Systematic empirical evaluations showed that the approach was promising. 
It \deleted{significantly} outperformed existing calibration methods in both efficacy and efficiency
in all settings we tested. 
In some difficult tasks, it eliminated about 71\% to 97\% high-confidence errors 
with only about 10\% of the minimal amount of labeled operation data 
 needed for practical learning techniques to barely work.
\deleted{In practice, such few operation data can be collected as feedback during a system's runtime, 
and largely improve the system's reliability for its later decisions to make.} 
%
%  
%They are also  
%Therefore, how to assess and improve the reliability of DNN-based systems becomes a highly relevant problem and has attracted much research.  
%
%Recently, many works~\cite{ma2018deepgauge, pei2017deepxplore, ma2018combinatorial, sun2018concolic, zhang2018deeproad, kim2019guiding} based on structural coverage of DNN are proposed for searching adversarial inputs. 
%These testing methods are similar to \emph{debug testing}~\cite{frankl1998evaluating} in traditional software testing, 
%and they think that the adversarial examples are the bugs of the DNN model that needs to be fixed.  
%However, it is still questionable whether we could consider such adversarial examples as bugs. 
%\citeauthor{grosse2018statistical} found that the distributions between the original dataset and the adversarial dataset are different through the hypothetical test. 
%And lately, 
%\citeauthor{ilyas2019adversarial} proposed that the adversarial examples are features rather than the bugs of the model. 
%Besides, the effectiveness in searching adversarial inputs of these coverage-based testing methods needs exploration: 
%\citeauthor{li2019structural} pointed out that such testing methods could not transfer the wisdom of coverage in traditional software testing into debug DNN testing successfully, 
%and their preliminary study suggests that structural coverage criteria for neural networks can be misleading since there exists no correlation between coverage and fault-finding effectiveness. 
%
%Contrasting to these debug DNN testing aimed at generating artificial adversarial examples, 
%we focus on \emph{operational DNN testing},  
%i.e., testing a completely trained DNN model on a specific operational context. 
%This specific context is the actual application context that may differ from the original training/test context, 
%and the inputs of operational DNN testing are the data collected from it. 
%Particularly, when applying a completely trained DNN into practice, the discrepancy between original training context and application context may disturb the performance of the model.
%And the operational DNN testing is intent upon evaluating and ensuring the actual performance in the operational context.
%Consequently, An effective and efficient testing method for the DNN model under the operation environment is crucial.
%
%The main reasons that operational DNN testing worth researching are as follows:  
%\begin{itemize}[leftmargin=*]
%\item The \emph{statistical nature} of the DNN model. 
%The DNN model indeed is the inductive program that could not handle the arbitrary input correctly. 
%Therefore, an individual error-inducing input could not explain the performance of the model at all. 
%Moreover, the No-Free-Lunch theorem indicates that evaluating a model with the data independent of its operational context is pointless. 
%Therefore, we need to center on 
%the concrete application context rather than excessive attention to the arbitrarily test context with artificially generated inputs.
%\item The \emph{common situation} of the DNN application. 
%The performance of the DNN model depends upon the assumption that the test dataset should have the same distribution with the training dataset. 
%However, this assumption is often violated~\cite{darrell2015machine}, 
%and it occurs universally in visual recognition and computational biology. 
%For instance, an image-classification model can be learned from pictures on the internet, 
%but are often applied to real-world scenes. 
%Therefore, operational DNN testing are urgent needed in ensuring the quality of the model in the application context.
%\item The \emph{fundamental challenge} of the DNN testing. 
%Different from traditional operational testing that has been well studied~\cite{musa1993profiles, 2017bertolinoadaptive}, 
%operational DNN testing is in urgency for further researches. 
%\citeauthor{li2019boosting} proposed that the main challenge of operational DNN testing is that it is too expensive and even impractical to label all the operation data collected in the field. 
%For example, in medical diagnostics, 
%to decide whether a radiology or pathology image is really malignant or benign, 
%a surgical biopsy always is needed.  
%In this situation, each one more labeled sample means that there is a patient who will suffer more pain. 
%Therefore, it is critical to test the model with a limited budget for labeling data collected from this context. 
%Besides, for the sake of profit and safety, 
%the DNN model developer may only provide the DNN model and will not give the original training/test dataset. 
%Above all, the main challenge of the DNN testing is that we often need to evaluate and ensure the performance of the DNN model in an extremely demanding situation: 
%labeled operation data are limited, and the original data are not available.
%\end{itemize}
%

%In this paper, we try to calibrate the DNN confidence in the specific operational context. For details, the divergence between the original dataset and the operation dataset will cause the confidence to be misleading, i.e., there exist many high confidence error-inducing inputs so that we nearly could not determine whether the classification results can be trusted. To solve this problem, we exploit the feature representation capabilities of the DNN model, which are still valid under the operational context, to locate these miscalibrations in representation space.  Then try to calibrate them through building a reliable operational confidence distribution with Bayesian Inference~\cite{tipping2004bayesian}. 

In summary, the contributions of this paper are: 
\begin{itemize}
%\item Posing the problem of operational calibration 
%for DNN models in the field, 
%and casting it into a Bayesian inference framework. 
%
%\item Proposing a Gaussian Process-based approach to operational calibration, 
\item Examining quality assurance for  DNN models used as software components, 
and raising the problem of operational calibration as debugging for confidence errors of DNNs in the field.
\item Proposing a  Gaussian Process-based approach to operational calibration, 
which leverages the representation learned by the DNN model under calibration 
and the locality of confidence errors in this representation. 
\item Evaluating the approach systematically. Experiments with various datasets and models confirmed the general efficacy and efficiency of our approach.
\end{itemize}

The rest of this paper is organized as follows. 
We first discuss the general need for operational quality assurance for DNNs in Section~\ref{sec:operqa}, 
and then define the the problem of operational calibration in Section~\ref{sec:problem}. 
We detail our approach to operational calibration in Section~\ref{sec:method}
and evaluate it empirically in Section~\ref{sec:evaluation}. 
We overview related work and highlight their differences from ours in Section~\ref{sec:relatedwork}
before concluding the paper with Section~\ref{sec:conclusion}.



==> OptConfPaper/method.tex <==
% !TEX root = main.tex

\section{Solving Operational Calibration with Gaussian Process Regression}
\label{sec:method}

At first glance operational calibration seems a simple regression problem with BS as the loss function. 
However, a direct regression would not work because of the limited budget of labeled operation data. 
%  
It is helpful to view the problem in a Bayesian way. 
At the beginning, we have a prior belief about the correctness of a DNN model's predictions, 
which is the confidence outputs of the model.  
Once we observe some evidences that the model makes correct or incorrect predictions on some inputs, 
the belief should be adjusted accordingly.
The challenge here is to strike a balance between 
the priori that was learned from a huge training dataset but suffering from domain shift, 
and the evidence that is collected from the operation domain but limited in volume. 

%{\color{blue} In this section, we introduce technical details of the Gaussian Process, and then analyze why the Gaussian Process performs well in representation space.  
%Following that, we provide a complete algorithm for the operational calibration of DNN models. 
%Finally, we further discuss the difference between operational calibration and previous confidence calibration methods. 
%One can skip the section~\ref{subsec:modeling with Gaussian Process} if feeling afraid of a large number of mathematical formulas,
%but we strongly recommend interested reader can read the discussion in section~\ref{subsec:discussions}.}

\subsection{Modeling with Gaussian Process}
 \label{subsec:modeling with Gaussian Process}


%for a given input $\bm{x}$, 
%instead of taking $\bm{x}$ which is in original input space, 
%we take advantage of its corresponding vector $\bm{z}$ in representation space. 
%Hence, for inputs $\bm{x}_i, 1 \leq i \leq N$ of operation dataset $T$, 
%we denote their corresponding vector in representation space as $Z_0=(\bm{z}_1^T; \dots; \bm{z}_N^T)$ 
%and their corresponding original confidence can be easily derived from original model $\mathfrak{M}$, we denote them as $\bm{c}_0 = (c_1; \dots; c_n)$.
%Then, after labeling some operational inputs, we denote these labeling data as $\bm{Z}_1 = (\bm{z}_{1'}^T, \dots, \bm{z}_{m'}^T)$, and its corresponding original confidence and labels are $\bm{c}_1 = (c_{1'}, \dots, c_{m'})$ and $\bm{l}_1 = (l_{1'}, \dots, l_{m'})$, respectively. And we compute~\cite{wang14icml} the ratio $\bm{r}_1 = (r_{1'}; \dots; r_{m'})$ of original confidence and operational confidence, where
%\begin{equation}
%r_{i'} = \frac{l_{m'}}{c_{m'}}.
%\end{equation}

%Due to the difficulty in 
%directly transforming the locality of representation space 
%into mathematical probability relation between point and point in representation space, 
%we try to use a Log Gaussian Process (LGP)
%to model original confidence $c$ and confidence ratio $r$. 
%
%Therefore, for a given vector $\bm{z}$ in representation space, the probability distribution of its confidence $c$ follows:
%\begin{equation}
%P(c \mid \bm{z}) \sim \log-\mathcal{N}(\mu_0, \sigma_0), 
%\end{equation}
%where 
%\begin{equation}
%\begin{aligned}
%& \mu_0 = K_{\bm{z} \bm{Z}_0}(K_{\bm{Z}_0 \bm{Z}_0} + \lambda \bm{I})^{-1} \bm{c}_0, \\
%& \sigma_0 = K_{\bm{z} \bm{z}} - K_{\bm{z} \bm{Z}_0}(K_{\bm{Z}_0 \bm{Z}_0} + \lambda \bm{I})^{-1} K_{\bm{Z}_0\bm{z}}.
%\end{aligned}
%\end{equation}
%
%Similarly, the prior probability distribution of the ratio are:
%\begin{equation}
%P(r \mid \bm{z}) \sim \log-\mathcal{N}(0, k),
%\end{equation}
%after observing some labeled operation data, we have
%\begin{equation}
%P(r \mid \bm{z}, \bm{Z}_1, \bm{r}_1) \sim \log-\mathcal{N}(\mu_1, \sigma_1),
%\end{equation}
%where
%\begin{equation}
%\begin{aligned}
%& \mu_1 = K_{\bm{z} \bm{Z}_1}(K_{\bm{Z}_1 \bm{Z}_1} + \lambda \bm{I})^{-1} \bm{r}_1, \\
%& \sigma_1 = K_{\bm{z} \bm{z}} - K_{\bm{z} \bm{Z}_1}(K_{\bm{Z}_1 \bm{Z}_1} + \lambda \bm{I})^{-1} K_{\bm{Z}_1\bm{z}}.
%\end{aligned}
%\end{equation}
%
%Finally, since operational confidence $l = r \cdot c$, we have $l$ also submit to log normal distribution, i.e.,
%\begin{equation}
%P(l \mid \bm{z}) \sim \log- \mathcal{N}(\mu_0 + \mu_1, \sigma_0 + \sigma_1).
%\end{equation} 



%\subsection{Deep Neural Network}
%A deep neural network (DNN) classification is an artificial neural network (ANN) with multiple intermediate (hidden) layers between the input and output layers. 
%The input of the latter layer is obtained by linear and non-linear transformations of the output of the previous layer. 
%We also refer the output layer as softmax layer.
%For a \textit{K}-classification problem, the formulation of softmax function is as follows:
%\begin{equation}\nonumber
%\sigma(\mathbf{z})_{i}=\frac{e^{z_{i}}}{\sum_{j=1}^{K} e^{z_{j}}}, \quad i=1, \ldots, K, \quad \mathbf{z}=\left(z_{1}, \ldots, z_{K}\right) \in \mathbb{R}^{K},
%\end{equation}
%where the vector $\bm{z}$ is output of the logit layer (it is the previous layer of softmax layer. )
%In brief, softmax layer provides a probability distribution consisting of $K$ probabilities.
%
%Figure~\ref{fig:DNN} is a simple example of the neural network. The existence of activation functions $\phi$ makes the model non-linear. 
%
%\begin{figure}[h]
%\begin{center}
%\def\layersep{2cm}
%\begin{tikzpicture}[shorten >=1pt,->,draw=black!50, node distance=\layersep]
%    \tikzstyle{every pin edge}=[<-,shorten <=1pt]
%    \tikzstyle{neuron}=[circle,fill=black!25,minimum size=15pt,inner sep=0pt]
%    \tikzstyle{input neuron}=[neuron, fill=green!50];
%    \tikzstyle{output neuron}=[neuron, fill=red!50];
%    \tikzstyle{hidden neuron}=[neuron, fill=blue!50];
%    \tikzstyle{annot} = [text width=6em, text centered]
%
%    % Draw the input layer nodes
%    \foreach \name / \y in {1,...,2}
%    % This is the same as writing \foreach \name / \y in {1/1,2/2,3/3,4/4}
%        \node[input neuron] (I-\name) at (-1.5* \layersep,-\y) {$x_\y$};
%
%    % Draw the first hidden layer nodes
%    \foreach \name / \y in {1,...,3}
%        \path[yshift=0.5cm]
%            node[hidden neuron] (H1-\name) at (-0.75* \layersep,-\y cm) {$n_{\y}^{(2)}$};
%            
%    % Draw the second hidden layer nodes
%    \foreach \name / \y in {1,...,4}
%        \path[yshift=0.16cm]
%            node[hidden neuron] (H2-\name) at (0*\layersep,- 0.66* \y cm) {$n_{\y}^{(3)}$};
%
%    % Draw the output layer node
%    \foreach \name / \y in {1,...,2}
%    \node[output neuron] (L-\name) at (0.75*\layersep,-\y cm) {$l_\y$};
%
%    \foreach \name / \y in {1,...,2}
%    \node[output neuron] (S-\name) at (1.5*\layersep,-\y cm) {$s_\y$};
%    % Connect every node in the input layer with every node in the
%    % hidden layer.
%    \foreach \source in {1,...,1}
%        \foreach \dest  / \y in {1,...,3}
%            \path (I-\source) edge node[near start] {$w_{1{\y}}$} node[near end]{$b_1$} (H1-\dest);
%            
%    \foreach \source in {2,...,2}
%        \foreach \dest  in {1,...,3}
%            \path (I-\source) edge  (H1-\dest);
%
%    % Connect every node in the hidden layer 
%    \foreach \source in {1,...,3}
%            \foreach \dest in {1,...,4}
%             \path (H1-\source) edge (H2-\dest);
%             
%    % Connect every node in the hidden layer with the output layer
%    \foreach \source in {1,...,4}
%            \foreach \dest in {1,...,2}
%             \path (H2-\source) edge (L-\dest);
%    \foreach \source in {1,...,2}
%            \foreach \dest in {1,...,2}
%             \path (L-\source) edge (S-\dest);
%             
%    % Annotate the layers
%   \node[annot, above of=H2-1, node distance=0.7cm] (hl) {};
%   \node[annot, left of=hl, node distance=1cm] {Hidden Layers};
%    \node[annot, above of=I-1, node distance=1.2cm] {Input};
%    \node[annot, above of=L-1, node distance=1.2cm] {logit};
%    \node[annot, above of=S-1, node distance=1.2cm] {softmax};
%    %\draw[dashed, color=black, line width=0.5pt] (-0.3 * \layersep,-2.8cm) node[below]{$n_i=\phi(\sum_{j}w_{j,i}x_j + b_i)$} ->(-0.5 * \layersep,-2.8cm);
%    \node[below of=H1-3, node distance=0.6cm]{\small{$n_i=\phi(\sum_{j}w_{j,i}x_j + b_i)$}};
%
%\end{tikzpicture}
%\end{center}
%\caption{A simple neural network}
%\label{fig:DNN}
%\end{figure}
%
%Training a DNN model is trying to search the optimal parameters (weights $w_{i,j}$ and biases $b_i$)  
%for minimizing the averaged prediction error over the whole training dataset. 
%Actually, from the perspective of Bayesian, 
%the DNN model learned a posterior probability distribution~\cite{bishop2006prml}, denoted as $p(y \mid \bm{x})$.
%For the given input $\bm{x}$, DNN will give \textit{K} posterior probability functions $p(y = i \mid \bm{x}), i=1,2,\dots,K$ 
%The classification result for this input is 
%the category corresponding to the maximum posterior probability, 
%i.e., $f(\bm{x}) = \arg\max_i p(y = i \mid \bm{x})$, 
%and the confidence is the associate max value $\max_i p(y = i \mid \bm{x})$. 
%In real-world decision-making systems, 
%classification networks should not only be accurate enough in prediction
%but also could offer the precise confidence to indicate when they are likely to be incorrect. 
%For example, a self-driving car, 
%which uses a neural network to detect pedestrians and other obstructions~\cite{bojarski2016selfdriven}, 
%should rely more on other components of self-driven system to control the braking 
%if its detection network cannot confidently predict the presence or absence of immediate obstructions.
%
%In deep learning, 
%DNN testing often aimed to evaluate the generalization of the model. 
%The different evaluation metrics~\cite{seliya2009metrics} (e.g., precision, recall, and 0/1-loss) are set towards different contexts. 
%It always requires that the training data and test data are i.i.d, and in this sense, 
%the test set could adequately characterize the overall performance if test examples are sufficient. 

%In this paper, we assume that if the test set is large enough, the distribution of examples in the test set is consistent with that in the real task.
%However, when the size of test set is small, the inadequacy of test samples will bring unstablility of the accuracy.

%\subsection{The Problem Formulations}
%It can be seen that there exist apparent distinctions between DNN testing and conventional software testing. 
%We think that the fundamental cause is that the DNN is an inductive program and the conventional software is deductive: 
%An individual error-inducing input of the latter always can reveal some logistic error in the program, 
%but for the former, some error-inducing inputs are tolerable in statistics. 
%However, the final goal of 
%DNN testing and conventional software testing are the same, 
%i.e., improving the reliability of software system. 
%
%As has been stressed before, 
%the subject of our research is operational DNN testing. 
%Compared to previous debug DNN testing, 
%operational DNN testing emphasis on inputs 
%that may appear under a specific operational context 
%rather than arbitrary artificially generated inputs (e.g., adversarial inputs). 
%The essential reason is that the 
%distribution of operation data is not compatible with the generated misclassified data. 
%Hence, even finding out such error-inducing inputs, 
%we still can not utilize them to improve the practical performance of the model. 
%In fact, training the model with such adversarial inputs 
%may produce a negative impact 
%on the operational performance of the model~\cite{kurakin2016advtraining}.
%Therefore, we think operational DNN testing are worth deploying
%because testing a previously trained DNN model must depend on its associate application context.
%In other words, operational DNN testing aims to \emph{improve the reliability of software system in the specific operational context.}
%
%On the one hand, the most efficient method for improving the operational DNN reliability is increasing the accuracy of model (i.e., training) in this operational context. 
%However, two factors bring great difficulty in re-training or fine-tuning the model directly. 
%1) Models are often provided by software developers. 
%We can hardly obtain any information 
%about original training process and original data.
%2) The size of labeled operation data is very limited. 
%In this situation, it is reckless to modify the model directly based on operation data.
%Take the ImageCELF dataset
%\footnote{This is a dataset from ImageCLEF 2014 challenge, 
%it contains three similar datasets, 
%\emph{Caltech-256} (\textbf{C}), \emph{ImageNet ILSVRC 2012} (\textbf{I}), and \emph{Pascal VOC 2012} (\textbf{P}). 
%We choose \textbf{C} dataset as original data and \textbf{P} dataset as operation data.}
%~\cite{caputo2014imageclef} as an example. 
%A previously trained model can achieve 86\% accuracy on operational context. 
%When we fine-tuned the model based on the limited operation dataset, 
%the performance of the model did not rise as we expected. 
%The detailed results can are shown in Figure~\ref{fig:training-directly}, 
% the red line is the accuracy without any modification of the model, 
% and the blue line is the accuracy of the fine-tuning model at each training epoch. 
%These two accuracies are both tested on the operation dataset.
%\begin{figure}[htbp]
%\begin{center}
%\includegraphics[width=0.9\columnwidth]{figures/confidence/training-directly}
%\caption{The risk of fine-tuning model directly}
%\label{fig:training-directly}
%\end{center}
%\end{figure}
%
%On the other hand, even if we can fine-tune the model, it is nearly impossible for a DNN model to achieve 100\% accuracy on the given context~\cite{devroye2013probabilistic}. 
%Consequently, one often hopes the DNN can retain the reliable confidence to ensure the system is able to reject possible incorrect inputs. 
%However, the divergence between specific operational context and original context 
%may result in confidence miscalibrations of DNN. 
%For example, we firstly trained a model with the MNIST dataset~\cite{lecun1998gradient}, 
%and then applied it to classified another handwritten digits dataset USPS~\cite{transferlearning.xyz}. 
%We find that 74 inputs are misclassified with high confidence (confidence greater than 0.9) of all 288 misclassified inputs. 
%It means even we set the reject threshold as 0.9, 
%nearly 1/4 incorrect predictions still will be trusted by system.
%The detailed results can be seen in Figure~\ref{fig:conf-risk}.
%
%\begin{figure}[htbp]
%\begin{center}
%\includegraphics[width=0.9\columnwidth]{figures/confidence/conf-risk}
%\caption{The confidence distribution of misclassified inputs}
%\label{fig:conf-risk}
%\end{center}
%\end{figure}
%
%Therefore, we think a significant DNN testing approach should not only searching the misclassifications in the operational context, 
%but also detecting confidence miscalibrations. 
%In this paper, we set the goal of DNN testing as 
%detecting DNNs' confidence miscalibrations in their operational context. 
%In this sense, the problem of efficient DNN testing is: 
%\emph{How to use as few samples for labeling as possible 
%to find more confidence miscalibrations of DNN and to calibrate them.}
%
%
%%It is true that in many cases (e.g., AI-aided clinical medicine~\cite{obermeyer2016predicting}) 
%%the unlabeled data can be easily collected from the operational environment 
%%but labeling them is expensive because it needs high quality annotation (e.g.,labeling sample through expert queries).
%%However, only relying on accuracy estimation could not explain the reliability of DNN model: 
%%A reliable DNN model not only is able to achieve enough accuracy, 
%%but also indicates the correctness of classification results through confidence.


%\subsection{Confidence Calibration}

%\subsection{Bayesian Approach and Gaussian Process}
%Bayesian inference provides a general framework 
%that can derive the posterior probability as a consequence of two antecedents: 
%its corresponding prior probability 
%and the likelihood function for the observed data.  
%The posterior probability is computed by Bayes' theorem:
%\begin{equation}
%P(H \mid E)=\frac{P(E \mid H)}{P(E)} \cdot P(H),
%\end{equation}
%where 
%\begin{itemize}
%\item \emph{Hypothesis} $H$ is any hypothesis in the whole hypothesis space.
%\item \emph{Prior probability} $P(H)$ is the probability of the specific hypothesis. 
%\item \emph{Evidence} $E$ stands for the observed new data.
%\item \emph{Likelihood} $P(E \mid H)$ describes that for the given hypothesis $H$, 
%         the probability of the occurrence of evidence $E$.  
%\item \emph{Marginal likelihood} $P(E)$ is the probability of the occurrence of evidence $E$. 
%\item \emph{Posterior probability} $P(H \mid E)$ is the probability of the hypothesis $H$ given the observed evidence $E$.
%\end{itemize}


%\subsection{Gaussian Process for Regression}

It is natural to model the problem as a Gaussian Process~\cite{rasmussen2005GPML}, 
because what we need is actually a function $\hat{c}(\cdot)$. 
Gaussian Process is a non-parametric kind of Bayesian methods, 
which convert a prior over functions into a posterior over functions according to observed data.

For convenience, instead of estimating $\hat{c}(\cdot)$ directly,  
we consider  
\begin{equation}
h(\bm{x}) = \hat{c}(\bm{x}) - c_\mathfrak{M}(\bm{x}), 
\label{equ:deltaconf}
\end{equation}
where $c_\mathfrak{M}(\bm{x})$ is the original confidence output of $\mathfrak{M}$ for input $\bm{x}$.
At the beginning, without any evidence against $c_\mathfrak{M}(\bm{x})$, 
we assume that the prior distribution of $h(\cdot)$ is a zero-mean normal distribution
\begin{equation}
h \sim \mathcal{N}(\cdot \mid 0, k(\cdot, \cdot)),
\label{equ:normcov}
\end{equation}
where $k(\cdot, \cdot)$ is the covariance (kernel) function, which intuitively describes the ``smoothness'' of $h(\bm{x})$ from point to point. In other words, the covariance function ensures that $h$
produces close outputs when inputs are close in the input space.

Assume that we observe a set  of independent and identically distributed (i.i.d.) labeled operation data $\bm{I} = \{(\bm{x}_i, y_i) \mathop{|} 1\leq i \leq n\}$, in which   $y = h(\bm{x}) = \mathbb{I}(\bm{x}) - c_\mathfrak{M}(\bm{x})$. 
%where $\mathbb{I}(\bm{x})$ is the indicator function for whether the labeled input $\bm{x}$ 
%is misclassified or not.
%be observed data of from some unknown distribution. 
For notational convenience, let 
\begin{equation*}
\begin{aligned}
\bm{X} &= (\bm{x}_1^{\mathsf{T}}; \dots; \bm{x}_n^{\mathsf{T}})  \quad \text{and} \\
\bm{h} &= ({h(\bm{x}_1)}; {\dots}; {h(\bm{x}_n)})
\end{aligned}
\end{equation*}
be the observed data and their corresponding $y$-values, and let 
\begin{equation*}
\begin{aligned}
\bm{X}' &= (({\bm{x}'_{1}})^{\mathsf{T}}; \dots; ({\bm{x}'_{n}})^{\mathsf{T}}), \quad \text{and} \\
\bm{h}' &= ({h(\bm{x}'_{1})}; {\dots}; {h(\bm{x}'_{n})})
\end{aligned}
\end{equation*}
be those for a set $T=\{(\bm{x}'_i, y'_i), i=1,\dots,m\}$ of i.i.d.\ predictive points. 
We have
\begin{equation}
\left(\begin{array}{l}{\bm{h}} \\ {\bm{h'}}\end{array}\right) 
\mid \bm{X}, \bm{X}' \sim \mathcal{N}\left(\bm{0},
\left(
\begin{array}{cc}
{K_{\bm{X}\bm{X}}} & {K_{\bm{X}\bm{X}'}} \\ 
{K_{\bm{X}' \bm{X}}} & {K_{\bm{X}'\bm{X}'}}
\end{array}\right)\right)
\end{equation}
where $\bm{K}$ is the kernel matrix. 
Therefore, the conditional probability distribution is 
\begin{equation}
\bm{y'} \mid \bm{y}, \bm{X}, \bm{X}' \sim \mathcal{N}\left(\bm{\mu}', \bm{\Sigma}'\right)
\end{equation}
where
\begin{equation*}
\begin{aligned}
\bm{\mu}' &=\bm{K}_{\bm{X}' \bm{X}}\left(\bm{K}_{\bm{X} \bm{X}}\right)^{-1} \bm{y}, \\ 
\bm{\Sigma}' &=\bm{K}_{\bm{X}' \bm{X}'}-\bm{K}_{\bm{X}'\bm{X}} \left(\bm{K}_{\bm{X} \bm{X}}\right)^{-1} \bm{K}_{\bm{X} \bm{X}'}.
\end{aligned}
\end{equation*}
%To ensure the matrix invertible, we often add the regularization term:
%\begin{equation}
%\begin{aligned}
%\bm{\mu}' &=\bm{K}_{\bm{X}_{*} \bm{X}}\left(\bm{K}_{\bm{X} \bm{X}}+\sigma^{2} \bm{I}\right)^{-1} \bm{y}, \\ 
%\bm{\Sigma}' &=\bm{K}_{\bm{X}' \bm{X}'}-\bm{K}_{\bm{X}'\bm{X}} \left(\bm{K}_{\bm{X} \bm{X}}+\sigma^{2} \bm{I}\right)^{-1} \bm{K}_{\bm{X} \bm{X}'}.
%\end{aligned}
%\end{equation}


% in this group, 
%we denote the index set of labeled inputs as . 
%The labeled inputs can be written as $\bm{x}_i, $, 
%we can know whether these labeled inputs are misclassified, 
%i.e. the value of indicate function $\mathbb{I}(\bm{x}_i), i \in \mathcal{I}$.
%Therefore, we need to change confidence $c(\bm{x}_i), i \in \mathcal{I}$ 
%to $c'(\bm{x}_i) = \mathbb{I}(\bm{x}_i), i \in \mathcal{I}$.
%In this sense, we have 
%\begin{equation}
%\Delta c(\bm{x}_i) = c'(\bm{x}_i) - c(\bm{x}_i), \quad i \in \mathcal{I}.
%\end{equation}
%

With this Gaussian Process, we can estimate the probability distribution of the operational confidence for any input $\bm{x'}$ as follows
\begin{equation}
h(\bm{x'}) \mid \bm{x'}, \bm{X}, \bm{h} \sim \mathcal{N}(\mu, \sigma),
\end{equation}
where
\begin{equation*}
\begin{aligned}
& \mu = \bm{K}_{\bm{x'} \bm{X}}(\bm{K}_{\bm{X}\bm{X}})^{-1} \bm{h}, \\
& \sigma = \bm{K}_{\bm{x'} \bm{x'}} - \bm{K}_{\bm{x'}\bm{X}}(\bm{K}_{\bm{X} \bm{X}})^{-1} \bm{K}_{\bm{X}\bm{x'}}.
\end{aligned}
\end{equation*}
Then, with Equation~\ref{equ:deltaconf}, we have the distribution of $\hat{c}\left(\bm{x'}\right)$
\begin{equation}
P\left(\hat{c}\left(\bm{x'}\right) \mid \bm{x'}\right) \sim \mathcal{N}\left(c_\mathfrak{M}\left(\bm{x'}\right) + \mu, \sigma \right).
\end{equation} 

Finally, due to the value of confidence ranges from 0 to 1, 
we need to truncate the original normal distribution~\cite{burkardt2014truncated}, i.e.,
\begin{equation}
P\left(\hat{c}\left(\bm{x'}\right) \mid \bm{x'}\right) \sim \mathcal{TN}\left(\mu_{tn}, \sigma_{tn}; \alpha, \beta \right),
\end{equation} 
where
\begin{equation}\label{truncated normal distribution}
\begin{aligned}
& \mu_{tn} = c_\mathfrak{M}\left(\bm{x'}\right) + \mu + \frac{\phi(\alpha) - \phi(\beta)}{\Phi(\alpha) - \Phi(\beta)}\sigma,  \\
& \sigma_{tn}^2 = \sigma^2 \left[1 + \frac{\alpha \phi(\alpha) - \beta \phi(\beta)}{\Phi(\beta) - \Phi(\alpha)} - \left( \frac{\phi(\alpha) - \phi(\beta)}{\Phi(\beta) - \Phi(\alpha)} \right)^2 \right], \\
& \alpha = (0 - c_\mathfrak{M}\left(\bm{x'}\right) - \mu) / \sigma,   
\quad  \beta = (1 - c_\mathfrak{M}\left(\bm{x'}\right) - \mu) / \sigma.
\end{aligned}
\end{equation}
Here the $\phi(\cdot)$ and $\Phi(\cdot)$ are the probability density function and the cumulative distribution function of standard normal distribution, respectively.

With this Bayesian approach, 
we compute a distribution, rather than an exact value, 
for the confidence of each prediction. 
To compute the Brier score, % which only accepts a confidence value as input, 
we simply choose the maximum a posteriori (MAP), i.e., the mode of the distribution,
as the calibrated confidence value.
%In other word, the confidence value is computed by Maximum a Posteriori estimation .
Here it is the mean of the truncated normal distribution 
\begin{equation} 
	\hat{c}(\bm{x}) = \mu_{tn}.
\end{equation}

%Nevertheless, the Bayesian approach has its 
%advantage in providing more information about the 
%uncertainty of the estimated confidence. 
%As will be discussed later, this information is relevant in some cost-sensitive decisions,
%and can help in the selection of operation data to label.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




\subsection{Clustering in representation space}

%\subsection{Effective and Efficient Operational Calibration}

Directly applying the above Gaussian Process to estimate $\hat{c}(\cdot)$ would be 
ineffective and inefficient. 
It is difficult to specify a proper covariance function in Equation~\ref{equ:normcov}, 
because the correlation between the correctness of predictions on different examples 
in the very high-dimensional input space is difficult, if possible, to model.  

Fortunately, we have the DNN model $\mathfrak{M}$ on hand, 
which can be used as a feature extractor, %= f_\mathfrak{M}(\bm{x})  
although it may suffer from the problem of domain shift% and perform badly as a classifier
~\cite{bengio2012unsupervised}.
In this way we transform each input $\bm{x}$ from the input space to 
a corresponding point $\bm{z} $ in the representation space, 
which is defined by the output of the neurons in the last hidden layer. 
It turns out that the correctness of $\mathfrak{M}$'s predictions has 
an obvious locality, i.e., a prediction is more likely to be correct/incorrect 
if it is near to a correct/incorrect prediction in the representation space. 
%
%
%
%
%%There are a few works that attempted to increase the efficiency of operational DNN testing. 
%%\citeauthor{li2019boosting} proposed a test data reduction technique: 
%%Through the distribution approximation of the neurons in the last hidden layer of DNN, 
%%only using half of the test inputs for labeling can achieve a similar level of precision compared with the random sampling in whole test data.
%%However, we think they did not realize 
%%the real insight of their operation data reduction method. 
%Through the transformation of DNN, 
%the inputs are mapped into multiple clusters in representation space of last layer. 
%And the classification result derives from a linear classifier in this representation space. 
%Thus, in the representation space of last layer, 
%the correctness of inputs possesses locality. 
%For details, inputs which have similar outputs in this representation space 
%often are correct or incorrect at the same time.  
%We take datasets MNIST/USPS as a simple example.
%In particular, we previously train a model on MNIST dataset.
%When we applying this model on USPS dataset, 
%which is actually the operation domain,
%although the accuracy significantly drops from 97\% to 68\%, 
%the correctness and incorrectness in representation space still keep relevance.
%To visualize this property, 
%we reduce the representation space to two-dimensional plane, 
%and plot the the location in representation space of incorrect (red points) and correct (blue points) inputs
%See Figure~\ref{fig:locality} for an intuitive example.

%\begin{figure}[htbp]
%\begin{center}
%\includegraphics[width=0.85\columnwidth]{figures/confidence/locality}
%\caption{Locality of prediction correctness in the representation space. 
%\rm{A DNN model trained on the MNIST dataset is applied to an operation 
%domain of the USPS dataset. Despite the significant drop of accuracy from 97\% to 68\%,
%the model is still effective in grouping together examples with correct predictions (blue \textcolor{blue}{$+$}) 
%and those with incorrect ones (red \textcolor{red}{$\times$}). 
%The representation space is reduced to a two-dimensional plane to visualize the effect.}}
%
%\label{fig:locality}
%\end{center}
%\end{figure}

Another insight for improving the efficacy and efficiency of the Gaussian Process is that 
the distribution of operation data in the sparse representation space is far from even. 
They can be nicely grouped into a small number (usually tens) of clusters,
and the correlation of prediction correctness within a group is much stronger than that between groups. 
Consequently, instead of regression with a universal Gaussian Process, 
we carry out a Gaussian Process regression in each cluster.  

This clustering does not only reduce the computational cost of the Gaussian Processes, 
but also make it possible to use different covariance functions for different clusters. 
The flexibility makes our estimation more accurate. 
Elaborately, we use the RBF kernel 
\begin{equation}
k(\bm{z}_1,\bm{z}_2) = \exp\left(-\frac{{\| \bm{z}_1 - \bm{z}_2 \|}^2}{2 \ell^2} \right)
\end{equation} 
where the 
parameter $\ell$ (length scale) can be decided according to the distribution of the original confidence produced 
by $\mathfrak{M}$.   


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Considering costs in decision}
The cost of misclassification must be taken into account in real-world decision making. 
\replaced{We propose to}{One can} also measure how well a model is calibrated with the \emph{loss due to confidence error} (LCE) against a given cost model. 

For example, let us assume a simple cost model in which the gain for a correct prediction is 1 and the loss for a false prediction is $u$. The net gain if we take action on a prediction for input $\bm{x}$ will be
$ \mathbb{I}(\bm{x}) -  u \cdot (1-\mathbb{I}(\bm{x}))$. 
We further assume that there will be no cost to take no action 
when the expected net gain is negative. 
Then the actual gain for an input 
$\bm{x}$ with estimated confidence $\hat{c}(\bm{x})$ will be
\begin{equation}
g(\bm{x}) = 
\left\{
\begin{array}{cc}
{ \mathbb{I}(\bm{x}) -  u \cdot (1-\mathbb{I}(\bm{x}))} & {\text{if}~\hat{c}(\bm{x}) \ge \lambda,} \\
{0} & {\text{if}~\hat{c}(\bm{x}) < \lambda,}  
\end{array}\right.
\label{eqn:actgain}
\end{equation}
where $\lambda= \frac{u}{1+u}$ is the break-even threshold of confidence for taking action.
%
%In the perspective of frequentist, 
%confidence is an exact value 
%which indicates the probability of false prediction.
%In this sense, the break-even threshold of confidence will be $\lambda= \frac{u}{1+u}, \quad 0 < \lambda <1$. 
%We further assume that there is no cost to reject the prediction with confidence lower than $\lambda$.
%In the following we use $\lambda$ to characterize the cost model.  
%
On the other hand, if the confidence was perfect, 
i.e., $\hat{c}(\bm{x})=1$ if the prediction was correct, and 0 otherwise, 
the total gain for dataset $D$ would be 
a constant $G_D=\sum_{i=1}^N\mathbb{I}(\bm{x}_i)$. 
%But the actual gain for an input $\bm{x}$ with estimated confidence $\hat{c}(\bm{x})$ will be
%\begin{equation}
%g(\bm{x}) = 
%\left\{
%\begin{array}{cc}
%{ \mathbb{I}(\bm{x}) -  \frac{\lambda}{(1-\lambda)} \cdot (1-\mathbb{I}(\bm{x}))} & {\text{if}~\hat{c}(\bm{x}) \ge \lambda,} \\
%{0} & {\text{if}~\hat{c}(\bm{x}) < \lambda,}  
%\end{array}\right.
%\end{equation}
So the average LCE over a dataset $D$ with $N$ examples is
%\begin{equation}
$\ell(D) = \frac{1}{N}\left(G_D - \sum_{i=1}^N g(\bm{x}_i)\right)$.
%\end{equation}

%Therefore, the LCE problem is that how to set confidence threshold $\lambda$ and calibrate the confidence $\hat{c}(\cdot)$ to minimize loss due to confidence error $\ell(D)$.

With the Bayesian approach we do not have an exact $\hat{c}(\bm{x})$ 
but a truncated normal distribution of it. 
If we take $\mu_{tn}(\bm{x})$ as $\hat{c}(\bm{x})$,
the above equations still hold.%
%~\footnote{%
%This is because here $u$ is a constant. Things will be different if otherwise. %, for example, 
%%one puts higher stakes on higher confidence predictions. 
%The page limit does not allow us to elaborate on this issue, 
%but the Bayesian approach allows for the flexibility in dealing with different situations.  
%} 

%The expected net gain if we take action will be  
%%For loss due to confidence error, 
%%instead of choosing a single confidence threshold $\lambda$, 
%%the decision criteria for inputs acceptance will depend on the expected profit:
%%
%%In particular, in our simple problem setting 
%%(the gain for a correct prediction is 1 and the loss for a false prediction is $u$).
%%Base on the truncated normal distribution, the expected profit for input $\bm{x}$ is
%\begin{equation}
%\begin{aligned}
%%\mathbb{E}_u \left(\mu_{tn}, \sigma_{tn}\right) 
%g(\bm{x})  &= \int_{c \sim \mathcal{TN}} c \cdot 1 - (1-c) \cdot u \, dc  \\
%&= \mu_{tn}(\bm{x}) \cdot (1+u) - u,
%\end{aligned}
%\end{equation}
%which coincides with the first line of Equation~\ref{eqn:actgain} 
%if taking $\mu_{tn}(\bm{x})$ as $\hat{c}(\bm{x})$. 
%
%We should accept the input that its expected profit is greater than 0, 
%thus the criteria for input acceptance is 
%\begin{equation}
%\hat{c}(\bm{x}) = \mu_{tn}(\bm{x}) \ge \frac{1+u}{u}.
%\end{equation}
%
%It is worth mentioning that 
%although the final acceptance criterion is independent of variance $\sigma_{tn}$, 
%it is because we only consider a relative simple problem setting in this paper. 
%In the case of complex problems, 
%for example, the misclassifications with high confidence will lead to more loss, i.e., $u(\bm{c}) = t \cdot c$, 
%then the decision criteria is 
%\begin{equation}
%\begin{aligned}
%\mathbb{E}_u \left(\mu_{tn}, \sigma_{tn}\right) &= \int_{c \sim \mathcal{TN}} c \cdot 1 - (1-c) \cdot u \, dc  \\
%&= t(\sigma_{tn}^2 + \mu_{tn}^2) - (t-1) \mu_{tn}.
%\end{aligned}
%\end{equation}
%Therefore, the bayesian framework will provide a general method 
%that solve a family of cost-sensitive problem.
%We will further study this series of issues in the future.





Cost-sensitive calibration targets at minimizing the LCE instead of the Brier score. 
% used in the cost-insensitive case. 
%Operational The Brier score and LCE can be seen as cost-insensitive and cost-sensitive cases, respectively.
%Without a cost model, %value of $u$, 
%or we want to minimize LCE for any $u$, 
Notice that calibrating confidence with Brier score generally reduces LCE. 
However, with a cost model, the optimization toward minimizing LCE can be more effective and efficient. 
%For our example, if false prediction is very expensive ($u \gg 1$), 
%we shall spend more budget of labeling data on reducing high confidence misclassifications,
%rather than increasing the confidence of correct predictions. 
%it will be better to build a biased distribution for  $\hat{c}(\bm{x})$ 




\subsection{Selecting operation data to label}
\label{subsec:inputselection}
In case that the set of labeled operation data is given, 
we simply apply a Gaussian Process in each cluster in the representation space 
and get the posteriori distribution for confidence $\hat{c}(\cdot)$.
However, if we can decide which operation data to label, 
we shall spend the budget for labeling more wisely. 

Initially, we select the operational input at the center of each cluster to label, 
and apply a Gaussian Process in each cluster with this central input
to compute the posterior probability distribution of the confidence. 
Then we shall select the most ``helpful'' input to label and repeat the procedure. 
%
The insight for input selection is twofold. 
First, to reduce the uncertainty as much as possible, 
one should choose the input with maximal variance $\sigma_{tn}^2$.
Second, to reduce the LCE as much as possible, 
one should pay more attention to those input with confidence 
near to the break-even threshold $\lambda$. 
So we chose $\bm{x}^*$ as the next input to label:
\begin{equation} \label{equ:selection}
%\bm{x}^* = \arg\min_{\bm{x}} \frac{|\mu_{tn}(\bm{x}) - \frac{u}{u+1}|}{\sigma_{tn}(\bm{x})}.
\bm{x}^* = \arg\min_{\bm{x}} \frac{|\mu_{tn}(\bm{x}) - \lambda|}{\sigma_{tn}(\bm{x})}.
\end{equation}

\added{
With $\bm{x}^*$ and its label $y^*$, we update the corresponding Gaussian Process model and 
get better $\mu_{tn}(\cdot)$ and $\sigma_{tn}(\cdot)$. 
%The select-label-update procedure is repeated until the budget for labeling is used up. 
The select-label-update procedure is repeated until the labeling budget is used up. 
%Thus we should label iteratively such that we can keep the Gaussian Process model (i.e., $\mu_{tn}(\cdot)$ and $\sigma_{tn}(\cdot)$) updated for guiding the new input selection.
%Considering the limited size of labeled operation data and the non-parametric property of Gaussian Process,  the computational complexity of model updating is very low.
}

%Another requirement of operation calibration is 
%\emph{correcting high confidence misclassifications on operation domain with few samples}.
%As discussed earlier, inputs acceptance criteria in our setting are
%\begin{equation}
%\hat{c}(\bm{x}) = \mu_{tn}(\bm{x}) \ge \frac{u}{u+1},
%\end{equation}
%thus correcting high confidence misclassifications 
%is equivalent to minimizing LCE with large $u$.
%




\medskip 

Putting all the ideas together, we have Algorithm~\ref{alg:1} shown below. 
The algorithm is robust in that it does not rely on any hyperparameters 
except for the number of clusters.
It is also conservative in that it does not change the predictions made by 
the model. As a result, it needs no extra validation data.

\begin{algorithm}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\caption{Operational confidence calibration}
\label{alg:1}
\begin{algorithmic}[1]
\REQUIRE A trained DNN model $\mathfrak{M}$,  
unlabeled dataset $S$ collected from operation domain $\mathbb{D}$, 
and the budget $n$ for labeling inputs.
\ENSURE Calibrated confidence function $\hat{c}(\bm{x})$ for $\bm{x}$ belongs to $\mathbb{D}$.
\newline\emph{Build Gaussian Process models:}
\STATE Divide dataset $S$ into $L$ clusters using the K-modroid method, 
and label the inputs $\bm{o}_1,\dots,\bm{o}_L$ 
that correspond to the centers of the $L$ clusters. 
\STATE Initialize the labeled set $T = \{\bm{o}_1,\dots,\bm{o}_L\}$.
\STATE For each of the clusters, build a Gaussian Process model $gp_i$, $i=1,\dots, L$.
\WHILE {$|T| < n$}
    \STATE Select a new input $\tilde{\bm{x}} \in S \setminus T$ for labeling, where $\tilde{\bm{x}}$ is searched by Equation~\ref{equ:selection}.
    \STATE Update the Gaussian Process corresponding to the cluster containing $\tilde{\bm{x}}$.
    \STATE Update the labeled set $T \leftarrow T \cup \{\tilde{\bm{x}}\}$.
\ENDWHILE
\newline\emph{Compute confidence value for input $\bm{x}$:}
\STATE Find the Gaussian Process model $\hat{gp}$ corresponding to the cluster containing input $\bm{x}$.
\STATE Compute $\mu_{tn}(\bm{x})$ according to Equation~\ref{truncated normal distribution}.
\STATE Output the estimated calibrated confidence $\hat{c}(\bm{x}) = \mu_{tn}(\bm{x})$.
\end{algorithmic}
\end{algorithm}

\subsection{Discussions}
\label{subsec:discussions}
To understand why our approach is more effective than conventional confidence calibration techniques,
one can consider the three-part decomposition of the Brier score~\cite{murphy1973BSPartition}
\begin{equation}
\begin{aligned}
BS = &\sum_{m=1}^{M} \frac{|D_{m}|}{N} \left(\text{conf}(D_m) -\text{acc}(D_m) \right)^{2} \\
&-\sum_{m=1}^{M} \frac{1}{N} \left(\text{acc}(D_m) - \text{acc}\right)^{2}+\text{acc}(1-\text{acc}),
\end{aligned}
\end{equation}
where $D_m$ is the set of inputs whose confidence falls into 
the interval $I_{m}=\left(\frac{m-1}{M}, \frac{m}{M}\right]$, 
and the $\text{acc}(D_m)$ and $\text{conf}(D_m)$ 
are the expected accuracy and confidence in $D_m$, respectively.
The $\text{acc}$ is the accuracy of dataset $D$.

In this decomposition, the first term is called \emph{reliability}, 
which measures the distance between the confidence and the true posterior probabilities. 
The second term is \emph{resolution}, which measures the distinctions of the predictive probabilities.
The final term is \emph{uncertainty}, which is only determined by the accuracy.

In conventional confidence calibration,
the model is assumed to be well trained and work well with the accuracies.
In addition, the grouping of $D_m$ is acceptable because the confidence error is regarded as \emph{systematic error.} 
So one only cares about minimizing the reliability. 
This is exactly what conventional calibration techniques such as Temperature Scaling are designed for. 

However, in operational calibration, the model itself suffers from the domain shift, 
and thus may be less accurate than expected. 
Even worse, the grouping of $D_m$ is problematic because the confidence error is \emph{unsystematic} and 
the inputs in $D_m$ are not homogeneous anymore. 
Consequently, we need to maximize the resolution and minimize the reliability at the same time. 
Our approach achieves these two goals with  
 more discriminative calibration that is based on the features of individual inputs rather than their logits or confidence values. 
 


%According to the decomposition, 
%the goal of calibration, minimizing the Brier score, 
%is equivalent to minimizing the reliability and maximizing the the resolution at the same time.
%However, for temperature scaling method, 
%it assumes that the DNN's confidence error is a kind of systematic error.
%In other words, the goal of temperature scaling is to minimize the reliability.
%Thus, when applying the DNN model on operation domain, 
%the shift between origin domain and operation domain will bring some non-systematic error, i.e., the resolution needs to be maximized in further.
%In this situation, compared with our calibration method, 
%the temperature scaling method is not effective enough.

This observation also indicates that the benefit of our approach over Temperature Scaling 
will diminish if the confidence error happens to be systematic. 
For example, in case that the only divergence of the data in the operation domain 
is that some part of an image is missing, our approach will perform similarly to 
or even slightly worse than Temperature Scaling. 
%On the contrary, if the error of confidence is only a systematic decline or increase, 
%for example, 
%in case that , 
%temperature scaling will still be effective 
%and our method is relatively more complex, 
%so its efficacy may not be better than the former.
However, as can be seen from later experiments, most operational situations have more or less 
domain shifts that Temperature Ccaling cannot handle well.

In addition, when the loss for false prediction $u$ is very small ($u \leq 0.11$, as observed from experiments in the next section), our approach will be ineffective in reducing LCE.
It is expected because in this situation one should accept almost all predictions, 
even when their confidence values are low.



==> OptConfPaper/relatedwork.tex <==
% !TEX root = main.tex
\section{Related work}
\label{sec:relatedwork}
Operational calibration is %proposed as a software quality assurance activityoperation data
%for adopting a previously trained DNN model in an operation domain. 
%It is 
generally related to the \added{quality assurance for} \deleted{testing of} deep learning systems 
in the software engineering community, and the confidence calibration, 
transfer learning, and active learning in the machine learning community.   
We briefly overview related work in these directions 
and highlight the connections and differences between our work and them. 

\subsection{Software \added{quality assurance} \deleted{testing} for deep learning systems}
The research in this area can be roughly classified into four categories according to 
the kind of defects targeted: 
%There are many researches on seeking an effective and efficient technique 
%to assure the DNN quality. 
%Their ideas of DL testing can be divided into three classes.
\begin{itemize}[leftmargin=*]
\item \emph{Defects in DL programs}. This line of work focuses on 
the bugs in the code of DL frameworks. 
For example, \citeauthor{pham2019cradle} proposed to test the implementation 
of deep learning libraries (TensorFlow, CNTK and Theano) through differential testing~\cite{pham2019cradle}.
\citeauthor{odena2019tensorfuzz} used fuzzing techniques to expose 
numerical errors in matrix multiplication operations~\cite{odena2019tensorfuzz}. 
%They implemented the same model on different libraries, and then detected the differences of output on one identical input. 
%The different outputs always show the inconsistencies and bugs among libraries.
%(2) \citeauthor{odena2019tensorfuzz} used fuzzing to capture the numerical errors in matrix multiplication operations of networks. 
%They computed coverage metric by approximate nearest neighbor (ANN) algorithms, 
%and generated coverage-based test inputs to reveal disagreements between neural networks and their quantized versions. 
%\citeauthor{} 
\item \emph{Defects in DL models}. 
Regarding trained DNN models as pieces of software artifact, 
and borrowing the idea of structural coverage in conventional software testing, 
a series of coverage criteria have been proposed for the testing of DNNs, 
for example, 
%
%These bugs indicate the correctness of DNN model. 
%The main challenge of testing the model is how to effectively and efficiently search 
%the input which can reveal the incorrect prediction for given model.
%Therefore, many neuron coverage based testing methods are proposed (e.g. 
DeepXplore~\cite{pei2017deepxplore}, DeepGauge~\cite{ma2018deepgauge}, 
DeepConcolic~\cite{sun2018concolic}, and Surprise Adequacy~\cite{kim2019guiding},
to name but a few. 
%All of them tried to generate adversarial input 
%(which may not belong to normal data distribution~\cite{grosse2018statistical})
%through increasing the coverage. 
%However, the relation of 
%DNN quality assurance and training/testing the model based on adversarial inputs 
%still need further investigation.
%And recent research found that the adversarial inputs are features rather than bugs~\cite{ilyas2019adversarial}.

%In addition, some researchers focus on a particular problem of machine learning: overfitting and underfitting. 
%For example, \citeauthor{} detected underfitting/overfitting by observing the difference between training accuracy and test accuracy. 
%And fixed the underfitting/overfitting through selecting inputs to retrain the model.

\item \emph{Defects in training  datasets}.
Another critical element in machine learning is the dataset. 
There exist research aiming at debugging and fixing errors in the polluted training dataset. 
For example, PSI identifies root causes (e.g., incorrect labels) of data errors 
by efficiently computing the Probability of Sufficiency scores through 
probabilistic programming~\cite{chakarov2016debugging}.
\item \emph{Defects due to improper inputs}. A DNN model cannot well handle inputs 
out of the distribution for which it is trained. 
Thus a defensive approach is to detect such inputs. 
For example, \citeauthor{wang2019adversarial}'s approach checked whether an input is normal or adversarial 
by integrating statistical hypothesis testing and model mutation testing~\cite{wang2019adversarial}. 
\citeauthor{wang2020DISSECTOR} proposed DISSECTOR, which effectively distinguished unexpected inputs from normal inputs by verifying progressive relationship between layers~\cite{wang2020DISSECTOR}.
More work in this line can be found in the machine learning literature 
under the name of out-of-distribution detection~\cite{shalev2018out}.
\end{itemize}
For a more comprehensive survey on the testing of machine learning systems, one can consult 
 \citeauthor{zhang2019surveyMLT}~\cite{zhang2019surveyMLT}.


The main difference of our work, compared with these pieces of research, 
is that it is \emph{operational}, i.e., focusing on how well a DNN model will work 
in a given operation domain. As discussed in Section~\ref{sec:operqa}, 
without considering the operation domain, 
it is often difficult to tell whether a phenomena of a DNN model is a bug or a feature~\cite{ilyas2019adversarial,li2019structural}.

An exception is the recent proposal of \emph{operational testing}  
 for the efficient estimation of the accuracy of a DNN model 
in the field~\cite{li2019boosting}. 
Arguably operational calibration is more challenging and more rewarding than 
operational testing, because the latter only tells the overall performance 
of a model in an operation domain, but the former tells when it works well and when not. 
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{DNN confidence calibration}
Confidence calibration is important for training high quality classifiers. 
There is a plethora of proposals on this topic in the machine learning literature~\cite{niculescu2005predicting,naeini2015obtaining,zadrozny2002transforming, flach2016calibration, guo2017calibration}. Apart from the Temperature Scaling discussed in 
Section~\ref{subsec:dnnconfidence}, 
Isotonic regression~\cite{zadrozny2002transforming}, Histogram binning~\cite{zadrozny2001obtaining}, and Platt scaling~\cite{Platt1999probabilisticoutputs} 
are also often used. 
Isotonic regression is a non-parametric approach that employs the least square method with a non-decreasing and piecewise constant fitted function.
Histogram binning divides confidences into mutually exclusive bins 
and assigns the calibrated confidences by minimizing the bin-wise squared loss.
Platt scaling is a generalized version of Temperature Scaling.
It adds a linear transformation between the logit layer and the softmax layer, 
and optimizes the parameters with the NLL loss.
However, according to \citeauthor{guo2017calibration}, 
Temperature Scaling is often the most effective approach~\cite{guo2017calibration}.  

As discussed earlier in Section~\ref{subsec:discussions},
the problem of these calibration methods is that they regard 
confidence errors as systematic errors, 
which is usually not the case in the operation domain. 
Technically, these calibration methods are effective in 
minimize the reliability part of the Brier score, 
but ineffective in dealing with the problem in the resolution part. 

In addition, \citeauthor{flach2016calibration} discussed the problem of confidence calibration 
from a decision-theoretic perspective~\cite{flach2016calibration}. 
However, the confidence error caused by domain shift was not explicitly addressed. 

% Different from the above methods that calibrate the model without disturbing accuracy, 

%The Bayesian calibration is also considered due to its inherent uncertainty.  
%One such proposal is to use dropout, which was originally introduced as a regularization technique for training deep neural networks. 
%\citeauthor{gal2016dropout} instead proposed to use dropout at prediction time and cast it as approximate Bayesian inference~\cite{gal2016dropout}. 
%Because dropout can be seen as an ensemble method, 
%and the variance of predictive results can guide the confidence calibration. 
%However, though the mathematical results are very elegant, 
%this method still cannot be directly applied to large-scale tasks due to the considerable time consumption.
%
%Besides, conformal prediction, which determines precise levels of confidence in new predictions based on past experience, is also a related topic. 
%Recently, \citeauthor{papernot2018deep} introduce Deep k-Nearest Neighbors~\cite{papernot2018deep}. 
%They build k-Nearest Neighbors (kNN) models respectively for the output of each DNN immediate layer and estimate the confidence by the conformity of these kNNs' predictions.
%Unfortunately, the kNN model depends on the original training dataset and is not suitable for high dimensional situations. 

Previous research efforts on confidence calibration at prediction time instead of training time are uncommon, but do exist. 
\citeauthor{gal2016dropout} proposed to build a temporary ensemble model by using dropout at prediction time~\cite{gal2016dropout}. % and cast it as approximate Bayesian inference. 
% They calibrated the confidence based on the variance of this ensemble predictive results. 
Despite its elegant Bayesian inference framework, the method is computationally too expensive to handle 
%cannot be directly applied to 
large-scale tasks. % due to the considerable time consumption.
Recently, based on the insight of conformal prediction~\cite{shafer2008tutorial}, \citeauthor{papernot2018deep} %introduced Deep k-Nearest Neighbors~\cite{papernot2018deep}. 
%They 
proposed to build a k-Nearest Neighbors (kNN) model for the output of each DNN immediate layer~\cite{papernot2018deep}.   
The confidence of a prediction was estimated by the conformity of these kNNs' outputs.
Unfortunately, this method is  not applicable to non-trivial tasks either because of its incapability in handling high-dimensional examples. 
Note that these methods did not explicitly consider confidence errors caused by domain shifts.

\added{Another related line of work is under the name of uncertainty estimation~\cite{sensoy2018evidential, kuleshov2018accurate, schulam2019can}. 
For example, Evidential Deep Learning qualitatively evaluates the uncertainty of DNN predictions 
with a Dirichlet distribution placed on the class probabilities~\cite{sensoy2018evidential}. 
% Besides, there is quite a few work of uncertainty estimation, which is closely related to confidence calibration~\cite{sensoy2018evidential, kuleshov2018accurate, schulam2019can}. 
%For example, through putting a Dirichlet distribution on the class probabilities, \citeauthor{sensoy2018evidential} proposed Evidential Deep learning method that qualitatively evaluated the uncertainty of DNN predictions~\cite{sensoy2018evidential}. 
However, these methods mainly aim at out-of-distribution detection, which is considered easier than confidence calibration~\cite{flach2016calibration}. 
Identifying out-of-distribution inputs is useful in defending against adversarial attacks, 
but not directly helpful in adapting a model to a new operation domain. 
%In addition, these methods %also lack the scalability to work with large datasets such as ImageNet.
% do not explicitly consider domain shift either.% and may report most of the inputs in a new operation domain as ``out-of-distribution''.
%Apart from the worrying scalability of these methods, they also 
}


%Many experiments were conducted to analyze the reason for confidence errors. 
%Recent research showed that, 
%without the dataset shift,
%the confidence error is mainly caused by over-optimized on the surrogate loss (cross-entropy loss). 
%In other words, when operation data and origin data are i.i.d,
%the confidence error is actually a kind of systematic error.
%To calibration the confidence influenced by this error, 
%some simple regression methods can be very effective.
%In addition to temperature scaling which is discussed in Section~\ref{subsec:dnnconfidence}, 
%Isotonic regression, Histogram binning and Platt scaling~\cite{flach2016calibration, guo2017calibration}, 
%were also proposed to calibrate DNN confidence.
%
%
%However, in many situations, especially for deep learning tasks, 
%the i.i.d assumption may not be hold any more. 
%For example, an image-classification model 
%can be learned from pictures on the internet, 
%but is finally applied to real-world scenes. 
%Due to the existence of dataset shift, 
%confidence error are more than just systematic error 
%and these calibration methods are not effective. 
%Therefore, debug the confidence errors and calibrate DNN confidence 
%should be operational. 
%
%In addition to brier score as a measure of confidence calibration.
%Expected calibration error (ECE), negative log likelihood (NLL), 
%and many other measures are also used for evaluate the efficacy of calibration~\cite{guo2017calibration}.
%In decision theory, the brier score is a proper score function that measures the accuracy of probabilistic predictions. 
%The ECE is actually the first term (reliability) in composition of brier score, 
%The NLL pay more attention to inputs with higher confidence error 
%and Brier score is more uniform.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Transfer learning and active learning}
Our approach to operational calibration borrowed ideas from 
transfer learning~\cite{pan2009survey}
and active learning~\cite{settles2009active}. 
Transfer learning (or domain adaptation) aims at training a model from a source domain (origin domain in our terms)
that can be generalized to a target domain (operation domain), 
despite the dataset shift~\cite{ng2016nuts} between the domains. 
The key is to learn features that are transferable between the domains. 

However, transfer learning techniques usually require 
data from both of the source and target domains. 
Contrastingly, operational calibration often has to work 
with limited data from the operation domain and no data from the origin domain. 
%It does not aim at improving prediction accuracy in the operation domain,  
%but it may leverage the existing transferability of features 
%learned by the DNN model.   
%Both of them leverage the transferability of features learned by the DNN model, but while 
%The former aims at better prediction accuracy, the latter at more accurate confidence.  
%In addition, 
Transfer learning usually fails to work under this constraint. 
Even in case it works, it does not necessarily produce well calibrated models, 
and operational calibration is  needed to correct confidence errors~(cf. Figure~\ref{fig:ft-cali3}). 

Active learning aims at reducing the cost of labeling training data by 
deliberately selecting and labeling inputs from a large set of unlabeled data.  
For the Gaussian Process Regression, 
there exist different input selection strategies~\cite{seo2000gaussian, kapoor2007active, pasolli2011gaussian}.
We tried many of them, such as those based on uncertainty~\cite{seo2000gaussian}, on density~\cite{zhu2009active}, 
and on disagreement~\cite{pasolli2011gaussian}, but failed to find a reliable strategy 
that can further improve the data efficiency of our approach.
They were very sensitive to the choices of the initial inputs, the models, 
and the distribution of examples~\cite{settles2009active}.
However, we found that the combination of cost-sensitive sampling bias and uncertainty 
can help in reducing high-confidence false predictions, especially in a cost-sensitive setting. 




%is a kind of semi-supervised learning 
%whose goal is to get the best possible model performance 
%with as few queries as possible.
%
%the main challenge of employing transfer learning techniques to 
%assure operational DNN quality is the limitations of datasets and models.
%The 
%If this condition can be satisfied, the state-of-art transfer learning techniques 
%obviously can be used to assure operational DNN quality.
%However, in software development, 
%we nearly could not know the exact application context. 
%In other words, it is unavailable to operation data in the training process.  
%Besides, the number of operation data is also limited 
%and the original model may not be completely designed for operation data. 
%Thus the well-known technique, fine-tuning, also may not work in some situations.
%Due to these practical conditions, we think the operational calibration is 
%the most effective and efficient method for operational DNN quality assurance 
%and our experiments also valid this point.





==> zip/conclusions.tex <==
% !TEX root = main.tex
\section{conclusion}
\label{sec:conclusion}

Software quality assurance for systems incorporating DNN models 
is urgently needed. 
This paper focuses on the problem of operational calibration that 
detects and fixes the errors in the confidence given by a DNN model 
for its predictions in a given operation domain.
A Bayesian approach to operational calibration 
is given. It solves the problem with Gaussian Process Regression, 
which leverages the locality of the operation data, 
and also of their prediction correctness, in the representation space. 
\replaced{Experiments with representative datasets and DNN models
confirmed that the approach can significantly reduce the risk of 
high-confidence false prediction with a small number of  labeled data,
and thus efficiently improve the models' quality of service in operational settings.
}{The approach achieved impressive efficacy and efficiency 
in experiments with representative datasets and DNN models.} 


While with empirical evidence, we consider conducting more theoretical analysis on aspects
%Theoretical analysis on aspects 
such as the data efficiency and 
the convergence of our algorithm as future work. %is left for future work. 
In addition, we plan to investigate operational calibration methods 
for real-world decisions with more complicated cost models. 



==> zip/confidence.tex <==
% !TEX root = main.tex

\section{Operational calibration Problem}
\label{sec:problem}

Now we focus on the problem of operational calibration. % as a specific quality assurance task for engineering DNN-based systems in the field. 
We first briefly introduce DNN classifiers and their prediction confidence to pave the way for 
the formal definition of the problem. 

\subsection{DNN classifier and prediction confidence}
\label{subsec:dnnconfidence}

A deep neural network classifier contains multiple hidden layers between its input and output layers. 
A popular understanding~\cite{Goodfellow-et-al-2016} of the role of these hidden layers is that 
they progressively extract abstract features (e.g., a wheel, human skin, etc.) 
from a high-dimensional low-level input (e.g., the pixels of an image). 
These features provide a relatively low-dimensional high-level \emph{representation} $\bm{z}$ for the input $\bm{x}$, which makes the classification much easier, e.g., the image is more likely to be a car if wheels are present. 

What a DNN classifier tries to learn from the training data is a posterior probability distribution, 
denoted as $p(y \mid \bm{x})$~\cite{bishop2006prml}.
For a \textit{K}-classification problem, the distribution can be written as 
$p_i(\bm{x}) = p(y = i \mid \bm{x})$, where $i=1,2,\dots,K$. 
For each input $\bm{x}$ whose representation is $\bm{z}$, 
the output layer first computes the non-normalized prediction  
$\bm{h} =\bm{W}^{\top} \bm{z} + \bm{b}$, 
whose element $h_i$  is often called the \emph{logit} for the $i$-th class. 
The classifier then normalizes $\bm{h}$ with a softmax function to approximate the posterior probabilities
\begin{equation}
\hat{p}_i(\bm{x}) = \text{softmax}(\bm{h})_i=\frac{e^{h_i} }{\sum_{j=1}^{K} e^{h_j}}, \quad i=1, \ldots, K.
\end{equation}
%where $h_i$ is the logit value for the $i$th class.   
%(aslo called logit layer). 
%logit layer precede the softmax (output) layer. 
%and then classify inputs according to the features with a softmax function implemented in the output layer.
%%Therefore, we also refer the output layer as softmax layer.
%The purpose of training a DNN model with a data set 
%
%For a DNN model, it actually learned a posterior probability distribution~\cite{bishop2006prml} from training data, 
%denoted as $p(y \mid \bm{x})$.
%Particularly, for the given input $\bm{x}$, DNN will provided \textit{K} posterior probability values $p_i = p(y = i \mid \bm{x}), i=1,2,\dots,K$ 
%
Finally, to classify $\bm{x}$, one just chooses the 
%he classification result for this input is 
the category corresponding to the maximum posterior probability, 
i.e.,  
 \begin{equation}
 \hat{y}(\bm{x}) = \mathop{\arg\max}_i \hat{p}_i(\bm{x}).
 \end{equation}


Obviously, this prediction is intrinsically uncertain.  
%$\hat{y}(\bm{x}) = \arg\max_i p(y = i \mid \bm{x})$, 
The \emph{confidence} for this prediction, which quantifies the  
likelihood of correctness, can be naturally measured as 
the estimated posterior class probability 
% $$\hat{c}(\bm{x}) = \max_i \hat{p_i}(\bm{x}).$$ 
 \begin{equation}
 \hat{c}(\bm{x}) = \hat{p_i}(\bm{x}),  \quad i=\hat{y}(\bm{x}).
 \end{equation}
%
Confidence takes an important role in decision-making. 
For example, if the loss due to an incorrect prediction % $u_1$
is four times of the gain of a correct prediction, % $u_2$, 
one should not invest on predictions with confidence less than 0.8. 
%Inaccurate confidence could cause significant loss. 
%For example, an over-confident benign prediction for a pathology image 
%could mislead a doctor into overlooking a malignant tumor, 
%while an under-confident benign prediction could result in unnecessary confirmatory testings. 

Modern DNN classifiers are often inaccurate in confidence~\cite{szegedy2016rethinking}, 
because they overfit to the surrogate loss used in training~\cite{guo2017calibration, tewari2007consistency}. 
Simply put, they are over optimized toward the accuracy of classification, 
but not the accuracy of estimation for posterior probabilities. 
To avoid the potential loss caused by inaccurate confidence, 
\emph{confidence calibration} can be employed in the learning process~~\cite{flach2016calibration,guo2017calibration,tewari2007consistency}. 
\added{Early calibration methods such as isotonic regression~\cite{zadrozny2002transforming}, 
histogram binning~\cite{zadrozny2002transforming}, and Platt scaling~\cite{Platt1999probabilisticoutputs} simply 
train a regression model taking the uncalibrated confidence as input with the validation dataset.
More flexible methods, e.g., Temperature Scaling~\cite{hinton2015distilling}, 
find} a function $R$
to correct the logit $\bm{h}$ such that 
 \begin{equation}
 \hat{c}(\bm{x}) = \hat{p_i}(\bm{x})=\text{softmax}(R(\bm{h}))_i,  \quad i=\hat{y}(\bm{x})
 \label{equ:logitcali}
 \end{equation}
matches the real posterior probability $p_i(\bm{x})$. 
%   
Notice that, in this setting the inaccuracy of confidence is viewed as a kind of 
systematic error or bias, not associated with particular inputs or domains.
That is, \added{the calibration does not distinguish between different inputs with the same uncalibrated confidence.} \deleted{$R$ does not take $\bm{x}$ or $\bm{z}$ as input}. 




%which means 
%
%The fundamental goal of confidence calibration 
%is to make the confidence for a given input 
%equal to the true posterior probability of predictions.
%One often assume that confidence error 
%is caused by some systematic error of $\bm{h}$.
%For details, for each input, 
%there produces some consistent shifts between $\bm{h}$ 
%and the logit $\bm{h}'$ corresponding to true posterior probability.
%Thus, what we need to do is to learn a function
%that maps original logit $\bm{h}$ to the true logit $\bm{h}'$.

%There exist different kinds of calibration methods, such as isotonic regression~\cite{zadrozny2002transforming}, 
%histogram binning~\cite{zadrozny2002transforming}, and Platt scaling~\cite{Platt1999probabilisticoutputs}. 
%\added{These methods all attempt to train a regression model whose input is confidence. 
%For example, 
%The isotonic regression attempt to find a one-dimensional monotonic calibration function such that minimizing the Brier score.
%and the Platt scaling define the calibration function as}
%\begin{equation}
%\added{R(c) = \frac{1}{1+e^{-(a \cdot c + b)}},}
%\end{equation}
%\added{where $c$ is the input of confidence value, and $a, b$ are parameter computed by minimizing the cross entropy on the validation dataset. }
%However, according to a recent study~\cite{guo2017calibration}, 
%the most effective choice is often a simple method called Temperature Scaling~\cite{hinton2015distilling}.
%The idea is to define the calibration function as
% \begin{equation}
% R(\bm{h}) = \frac{\bm{h}}{T}, 
% \end{equation}
%where $T$ is a scalar parameter computed by minimizing the 
%negative log likelihood~\cite{hastie2009elements}
%on the validation dataset. 
%\added{Moreover, Platt scaling can also be improved through taking logit as input~\cite{guo2017calibration}, i.e., define the calibration function as}
% \begin{equation}
% \added{R(\bm{h}) = \bm{W}^{\mathsf{T}}\bm{h}+\bm{b}, }
% \end{equation}
% \added{where $\bm{W}$ is a matrix parameter and $\bm{b}$ is a vector parameter. 
% Both of these two parameters are computed by minimizing the cross entropy. }
 
%\begin{equation}
%\text{NLL}=- \sum_{i=1}^{n} \log \hat{c}(\bm{x}_i).
%\end{equation} 

%\emph{Expected Calibration Error}:
%\begin{equation}
%\mathrm{ECE}=\sum_{m=1}^{M} \frac{\left|D_{m}\right|}{n}\left|\operatorname{acc}\left(D_{m}\right)-\operatorname{conf}\left(D_{m}\right)\right|,
%\end{equation}
%where $D_m$ is the set of inputs whose confidence falls into 
%the interval $I_{m}=\left(\frac{m-1}{M}, \frac{m}{M}\right]$, 
%and the $acc(D_m)$ and $conf(D_m)$ are the expected accuracy and confidence in $D_m$, respectively.

%
%The experimental results show that the most fruitful method for calibration are \emph{temperature scaling} (TS):
%\begin{equation}
%\hat{q}(\bm{x}) = \max_{i} \frac{e^{(h_i/T)}}{\sum_{j=1}^{K} e^{(h_j/T)}}, \quad i=1, \ldots, K.
%\end{equation}
%where the temperature $T$ is chosen by minimizing the ECE.



%We first define the problem, and then present our method based on Gaussian Process. 

\subsection{Operational confidence calibration}



Given a domain where a previously trained DNN model is deployed, 
operational calibration 
identifies and fixes the model's errors in the confidence of predictions on individual inputs
in the domain.  
%against a set of operation data collected from 
%for a given domain in which the model actually operates.
%
%Viewing confidence as part of model output, operational calibration is not only testing, 
%but also a kind of debugging.  
%
Operational calibration is conservative in that it does not change the predictions made by the model, 
but tries to give accurate estimations on the likelihood of the predictions being correct. 
With this information, a DNN model will be useful even though its prediction accuracy 
is severely affected by the domain shift. 
One may take only its predictions on inputs with high confidence, 
but switch to other models or other backup measures if unconfident.  
 
 

%\subsection{Operational calibration}



%What operational calibration addresses is more an engineering problem than a machine learning problem.
%The essential task of machine learning is to induce from training data, 
%and it emphasizes the generalizability of the trained model, 
%although unfortunately the scope of generalization cannot be explicitly specified. 
%In dealing with domain shift, machine learning techniques such as transfer learning or domain adaptation 
%tend to \emph{generalize} the scope of the model to include the new operation context. 
%As a consequence these techniques heavily relies on the data from the original domain, 
%besides the new data from the operation context. 

%Contrastingly, operational calibration tries to make the most of a DNN model in a given operation context. 
%The model may be trained by a third party and provided \emph{as is}. 
%In operational calibration  
%the generalization to any domain other than the current one is not necessary.
%This more focused duty relieves us of the dependence to the original data. 
%The decoupling of DNN models from their training data and process is crucial to 
%promote the reuse of these models and to reduce privacy and proprietary risks~\cite{zhou2016learnware}. 
%Operational calibration also prioritize the saving of efforts in labeling data collected in operation context.   
%
%Besides these methodological considerations, 
%as to be shown later in Section~\ref{sec:evaluation},
%practically it would be imprudent and ineffective 
%to fine-tune or adapt a DNN model to fit an operational context 
%without access to the original training data, 
%unless we could afford a large number of labeled operation data.
%The trap here is that 
%%the performance of the model could be worsen because it 
%the model is very likely to be overfitting to the limited labeled operation data, 
%but not the entire operation domain without the balance from the original training data. 


 
%
%technique or fine-tuning  
%
%However, when applying DNN into application, 
%the specific operation context bring two tremendous difficulties. 
%First, the domain shift
%between original context and operation context 
%leads to some non-systematic error. 
%Therefore, the TS and other similar methods, which only rely on the logit, 
%is not effective in calibrating the operational confidence.
%Second, the information of original context, which includes original dataset and detailed training process of DNN, may be unavailable, 
%and operation dataset is not large enough. 
%Thus the transfer learning technique even fine-tuning could not effectively increasing the accuracy of model.
%%In this situation, it is reckless to modify the model directly based on operation data.

%Fortunately, the ability in extracting features is still useful. 
%In other words, the representation $\bm{z}$ in last hidden layer is still reliable.
%In this situation, instead of learning the parameters of function which map $\bm{z}$ to the true logit, we choose a bayesian method to estimate the operation confidence.

To quantify the accuracy of the confidence of a DNN model on a dataset 
%$D = \{(\bm{x}_i, \mathbb{I}(\bm{x}_i)), i=1,\dots,N\}$, 
$D = \{(\bm{x}_i, y_i), i=1,\dots,N\}$, 
one can use the  
%Generally, the confidence of a machine learning model can be viewed as a prediction operation datafor 
%the likelihood of the model giving correct prediction on a given input. 
%It can be measured by 
Brier score (BS)~\cite{brier1950verification}, which is actually the mean squared error of the estimation:
\begin{equation}
BS(D) = \frac{1}{N}\sum_{i=1}^N (\mathbb{I}(\bm{x}_i) - \hat{c}(\bm{x}_i))^2, 
\end{equation}
where $\mathbb{I}(\bm{x})$ 
is the indicator function for whether the labeled input $\bm{x}$ 
is misclassified or not, i.e., 
$\mathbb{I}(\bm{x}) = 1$ if $\hat{y}(\bm{x})=y(\bm{x})$, and $0$ otherwise.  
%is indicator function for whether the classification result is correct.



Now we formally define the problem of operation calibration:
\begin{problem} 	
%Given $\mathfrak{M}$ a previously trained DNN classifier, 
%%with its original confidence estimation $\hat{c}(\cdot)$
%$S$ a set of $N$ unlabeled examples collected from an operational domain, 
%and a budget $n \ll N$ for labeling the examples in $S$, 
%the task of operation calibration is try to find a confidence estimation function 
%$\hat{c}(\cdot)$ for $\mathfrak{M}$ 
%to minimize $BS(S)$ the Brier score in the cost-insensitive case, 
%or $\ell(S)$ for given $\lambda$ the loss due to confidence error in the cost-sensitive case.  
Given $\mathfrak{M}$ a previously trained DNN classifier, 
%with its original confidence estimation $\hat{c}(\cdot)$
$S$ a set of $N$ unlabeled examples collected from an operation domain, 
and a budget $n \ll N$ for labeling the examples in $S$, 
the task of operational calibration is to find a confidence estimation function 
$\hat{c}(\cdot)$ for $\mathfrak{M}$ with minimal Brier score $BS(S)$.
%to minimize  the .
%in the cost-insensitive case, 
%or $\ell(S)$ for given $\lambda$ the loss due to confidence error in the cost-sensitive case.  
\end{problem}

Notice that operational calibration is different from the confidence calibration discussed in 
Section~\ref{subsec:dnnconfidence}.
The latter is domain-independent and usually included as a step in the training process of a DNN model (one of machine learning's focuses), 
but the former is needed when the model is deployed as a software component by a third party in a specific operation domain (what software engineering cares about). 
Technically, operational calibration cannot take the confidence error as a systematic error of the learning process, 
%as the latter does, 
because the error is caused by the domain shift 
from the training data to the operation data, and it may \added{assign different confidence values to inputs with the same uncalibrated confidence value.} \deleted{depend on specific inputs from the operation domain.}


==> zip/dnnqa.tex <==
% !TEX root = main.tex

\section{Quality assurance for DNN models used as software artifacts}
\label{sec:operqa}

%Deep learning is intrinsically inductive~\cite{Goodfellow-et-al-2016}.
%However, conventional software engineering is mostly deductive, as evidenced by 
%its fundamental principle of specification-implementation consistency. 
%Adopting DNN models as integral parts of software systems poses 
%new challenges for quality assurance. 
%We first discuss the quality assurance problem for DNN models used in 
%given operation domains from a software engineering perspective, 
%and then briefly introduce DNN and its prediction confidence
%to provide the background for the work on operational calibration.  

%Different from human written programs, a DNN model is intrinsically uncertain about its predictions, 
%which is quantified by the corresponding confidence values. 
%Confidence takes an important role in practical decisions. 
%In this section we briefly introduce DNN and prediction confidence, 
%formally define the problem of confidence calibration for DNN in operation context, 
%and discuss its connection and difference with the calibration step usually included in the model training process.  

%\subsection{Operational quality assurance}

Well trained DNN models can provide marvelous capabilities, 
but unfortunately their failures in applications are also very common~\cite{Riley2019nature}.
When using a trained model as an integral part of a high-stakes software system, 
it is crucial to know quantitatively \emph{how well} the model will work \added{and to adapt it to the application conditions}.
The quality assurance combining the viewpoints from software engineering and machine learning is needed, but largely missing. 
\added{In what follows, we first discuss the non-conventional requirements for such quality assurance, 
and then give an application scenario to highlight the software engineering concerns. 
}




Deep learning is intrinsically inductive~\cite{Goodfellow-et-al-2016, zhou2019abductive}.
However, conventional software engineering is mostly deductive, 
as evidenced by its fundamental principle of specification-implementation consistency. 
%The principle of software quality assurance is founded on the specifications for software artifacts 
%and the deductive reasonings based on them. 
A specification defines the assumptions and guarantees of a software artifact.
The artifact is expected to meet its guarantees whenever its assumptions are satisfied.
Thus explicit specifications make software artifacts more or less domain independent.
However, statistical machine learning does not provide such kind of specifications. 
Essentially it tries to induce a model from its training data, 
which is intended to be general 
so that the model can give predictions on previously unseen inputs. 
Unfortunately the scope of generalization is unspecified. 
%Most transfer learning and domain adaptation techniques tries to 
%Thus the problem of domain shift is regarded as the lack of generalization 
As a result, a major problem comes from the divergence between the domain 
where the model was originally trained 
and the domain where it actually operates. 

So the first requirement for the quality assurance of a DNN model is to be \emph{operational}, i.e., to 
focus on the concrete domain where the model actually operates. 
Logically speaking, the quality of a trained DNN model will be pointless without considering its operation domain.
In practice, the performance of a model may drop significantly with domain shift~\cite{li2019boosting}.
%
On the other hand, focusing on the operation domain also relieves the DNN model 
from depending on its original training data. 
Apart from practical concerns such as protecting the privacy and property of the training data, 
decoupling a model from its training data and process will also be helpful for (re)using it 
as a commercial off-the-shelf (COTS) software product~\cite{zhou2016learnware}. 
This viewpoint from software engineering is in contrasting to machine learning techniques dealing with domain shift such as 
transfer learning or domain adaptation that heavily rely 
on the original training data and hyperparameters~\cite{pan2009survey,shu2018a,transferlearning.xyz}. 
They need original training data because they try to \emph{generalize} 
the scope of the model to include the new operation domain. 



The second requirement is to embrace the uncertainty that is intrinsic in DNN models. 
A defect, or a ``bug'', of a software artifact is a case that it does not deliver its promise. 
Different from conventional software artifacts, 
a DNN model never promises to be certainly correct on any given input, 
and thus individual incorrect predictions \emph{per se} should not be regarded as bugs, 
but to some extent features~\cite{ilyas2019adversarial}.   
Nevertheless, the model \emph{statistically} quantifies the uncertainty of their predictions. 
Collectively, it is measured with metrics such as accuracy or precision. 
Individually, it is stated by the confidence value about the prediction on each given input.  
These qualifications of uncertainty, as well as the predictions a model made, 
should be subject to quality assurance. 
For example, given a DNN model and its operation domain, 
operational testing~\cite{li2019boosting} examines 
to what degree the model's overall accuracy is degraded by the domain shift.
Furthermore, operational calibration, which is the topic of the current paper, 
identifies and fixes the misspecified confidence values on individual inputs.  
%Viewing confidence as part of model output, operational calibration is not only testing, 
%but also a kind of debugging.  

Finally, operational quality assurance should prioritize the saving of human efforts, 
which include the cost of collecting, and especially labeling, the data in the operation domain.  
The labeling of operation data often involves physical interactions, such as surgical biopsies  
and destructive testings, and thus can be expensive and time-consuming. 
%
Note that, as exemplified by the EU GDPR~\cite{eu-269-2014}, there are 
increasing concerns about the privacy and property rights in the data used to train DNN models. 
So when adopting a DNN model trained by a third party, 
one should not assume the availability of its original training data~\cite{zhou2016learnware, Shokri2015CCS, konevcny2016federated}. 
Without the access to the original training data, 
re-training or fine-tuning a DNN model to an operation domain can be unaffordable 
because it typically requires a large amount of labeled examples to work. 
Quality assurance activities often have to work under a much tighter budget for labeling data. 



\begin{figure}[htbp]
\begin{center}
\includegraphics[width=.95\columnwidth]{figures/OpQA}
\caption{Operational quality assurance}
\label{fig:opqa}
\end{center}
\end{figure}

Figure~\ref{fig:opqa} depicts the overall idea for operational quality assurance, 
which generalizes the process of operational testing proposed in~\cite{li2019boosting}. 
A DNN model, which is trained by a third party with the data from the origin domain, 
is to be deployed in an operation domain. It needs to be evaluated, and possibly adapted, 
with the data from the current operation domain. To reduce the effort of labeling, 
data selection can be incorporated in the procedure with the guidance of the information generated by  
the DNN model and the quality assurance activity.
Only the DNN models that pass the assessments and are possibly equipped 
with the adaptations will be put into operation. 





\added{
\medskip
For example, consider a scenario that a hospital decides to equip its radiology 
department with automated medical image analysis enabled by Deep Learning~\cite{obermeyer2016predicting}. 
While the system may involve many functionalities such as clinical workflow management, 
computer-aided diagnosis, and computer-assisted reporting, the key component is a DNN model or an ensemble of DNN models 
acting as a radiologist to classify images~\cite{MCM20DLRadiology}. 
It is too expensive and technically demanding for the hospital to collect enough high quality data and 
train the model in-house. 
So the hospital purchases the model from a third-party provider, and uses it as a COTS software component. 
However, the training conditions of the model are likely to be different from the operation conditions,
and the model performance reported by the provider is unreliable due to potential issues 
such as data mismatch, selection bias, and non-stationary environments~\cite{WMD18DLbiomedicine,Zech18VarGenDLRadiograph}. 
%In such a scenario re-training the model for the operation domain is usually infeasible, 
%due to the unavailability of the original training data and the limited availability of the labeled operation data~\cite{kemker2018measuring, kirkpatrick2017overcoming}.
To assure the system's quality of service, the model must be tested and calibrated against the current operation domain. 
The hospital first assesses the real accuracy of the model through operational testing~\cite{li2019boosting}, 
and decides to adopt it or not accordingly. 
Once the model is adopted and deployed, operational calibration steps in to adapt the model to the current operation domain, 
by fixing the errors in the confidence values and avoiding high-confidence false predictions. }

\added{
As a software quality assurance task, operational calibration tries to achieve best efficacy 
with a limited budget. The cost here, however, is mainly spent on the labeling of 
operation data. For sophisticated DNN models used for medical imaging classification such as Inception-V3, ResNet-50 and DenseNet-121~\cite{liu2017detecting, Zech18VarGenDLRadiograph}, 
even thousands of labeled data 	could be too less 
for model retraining or fine-tuning to work properly (c.f. Figure~\ref{fig:fine-tune1}). 
Nevertheless, as will be shown later, a deliberately designed calibration method 
can identify and fix most of the erroneous high confidence values associated to false predictions 
with only tens to small hundreds of labeled data (c.f. Figure~\ref{fig:efficiency-curve}).  
A model well calibrated for its operation domain, 
although still suffering from some loss in prediction accuracy, 
becomes more reliable in that broken promises are far less likely.   
%
%We give an example to explain the problem of operational confidence calibration more clearly.
%The hospital developed a medical image detection system to assist doctors in checking up patients. 
%The DNN model deployed in the system is well-trained based on original training data. 
%However, the performance (e.g., accuracy of prediction) drops significantly when using this system as the application on operation domain.
%Many factors may cause this problem, such as 
%mislabeling the training data, 
%damage to the image acquisition camera,
%and the emergence of new kinds of diseases.
%Actually, differences between origin domain and operation domain are almost inevitable~\cite{pooch2019can}. 
%In this situation, it is impossible to re-train a new model towards operation domain since labeling cost is too expensive and the size of operation data is too limited to support effective training~\cite{kemker2018measuring, kirkpatrick2017overcoming}.
%Thus, one may instead try to ``fix'' the current model to make full use of this system, 
%and the most practicable method is to calibrate the confidence on operation domain such that minimizing the loss caused by the low accuracy of DNN model.
}

  


==> zip/evaluation.tex <==
% !TEX root = main.tex
\section{Empirical evaluation}
\label{sec:evaluation}

We conducted a series of experiments to answer the following questions:
\begin{enumerate}
\item Is our approach to operational calibration generally effective in different tasks?
\item How effective it is, compared with alternative approaches?
\item How efficient it is, in the sense of saving labeling efforts? 
\end{enumerate}


We implemented our approach on top of the PyTorch 1.1.0 DL framework.
The code, together with the experimental data, are available at \url{https://github.com/Lizn-zn/Op-QA}. 
The experiments were conducted on a GPU server 
with two Intel Xeon Gold 5118 CPU @ 2.30GHz,
400GB RAM, and 10 GeForce RTX 2080 Ti GPUs.
The server ran Ubuntu 16.04 with GNU/Linux kernel 4.4.0. 

The execution time of our operational calibration 
depends on the size of the dataset used, and the architecture of the DNN model.  
For the tasks listed below, the execution time varied from about 3.5s to 50s, 
which we regard as totally acceptable. 

%\subsection{Evaluation setup}
\subsection{Experimental tasks}
To evaluate the general efficacy of our approach, 
we designed six tasks that were different in the application domains 
(image recognition and natural language processing), 
operation dataset size (from hundreds to thousands),
classification difficulty (from 2 to 1000 classes),
and model complexity (from $\sim$$10^3$ to $\sim$$10^7$ parameters).
To make our simulation of domain shifts realistic, 
in four tasks we adopted third-party operation datasets often used in the transfer learning research,
and the other two tasks we used mutations that are also frequented made in the machine learning community.  
Figure~\ref{fig:orig-and-opt} demonstrates some example images from the origin and operation domains 
\added{for tasks 3 and 5}.
%{\color{blue} Actually, a few factors may induce differences between origin domain and operation domain, such as the time of data collection (Task 2), the style of image background (Task 3), and the resolution of images (Task 6).
%}
%
%Considering different possible operation domains, 
%we choose various datasets to evaluate our approach. 
%In addition, DNN models with very different structures were used in these experiments.  
Table~\ref{tab:ExpDesign} lists the settings of the six tasks. %information of experimental design in details. 


%\begin{table}[htb]
%\caption{Dataset and model settings}
%\centering
%\setlength{\tabcolsep}{.38em}
%\begin{threeparttable}
%\begin{tabular}{|p{1.7cm}<{\centering}|c|p{1.1cm}<{\centering}|c|p{1.1cm}<{\centering}|}
%\hline
%\multirow{2}*{\textbf{Model}} & \multicolumn{2}{c|}{\textbf{Original}}  & \multicolumn{2}{c|}{\textbf{Operational}} \\
%\cline{2-5}
%& \textbf{Dataset} & \textbf{Acc. (\%)} & \textbf{Dataset} & \textbf{Acc. (\%)} 
%\\
%\hhline{|=====|}
%LeNet-5 & MNIST & 96.9 & USPS & 68.0 \\
%\hline %\hhline{|======|}
%RNN & Polarity v1.0 & 99.0 & Polarity v2.0 & 83.4 \\
%\hline
%VGG-19 & CIFAR-10 & 93.1 & Rotation & 71.1 \\
%\hline
%ResNet-50 & ImageCLEF-c & 99.2 & ImageCLEF-p & 73.2 \\
%\hline
%Inception-v3 & ImageNet & 77.5 & Down-sampling & 48.9 \\
%\hline
%\end{tabular}
%\end{threeparttable}
%\label{tab:ExpDesign}
%\end{table}

\begin{table}[htb]
\caption{Dataset and model settings of tasks}
\centering
\setlength{\tabcolsep}{.25em}
\begin{threeparttable}
\begin{tabular}{|c|c|c|c|c|p{0.4cm}<{\centering}|}
\hline
\multirow{2}*{\textbf{Task}} & \multirow{2}*{\textbf{Model}} & \multicolumn{3}{c|}{\textbf{Origin Domain} $\rightarrow$ \textbf{Operation Domain}} \\
\cline{3-5}
& & \textbf{Dataset} & \textbf{Acc. (\%)} & \textbf{Size$^*$} \\
\hhline{|=====|}
\multirow{2}*{1} & \multirow{2}*{LeNet-5} & Digit recognition & \multirow{2}*{96.9 $\rightarrow$ 68.0} & \multirow{2}*{900} \\
& & (MNIST $\rightarrow$ USPS) &  & \\
\hline %\hhline{|======|}
\multirow{2}*{2} & \multirow{2}*{RNN} & Polarity & \multirow{2}*{99.0 $\rightarrow$ 83.4} & \multirow{2}*{1,000} \\
& & (v1.0 $\rightarrow$ v2.0) & & \\
\hline
\multirow{2}*{3} & \multirow{2}*{ResNet-18} & Image classification & \multirow{2}*{93.2 $\rightarrow$ 47.1} & \multirow{2}*{5,000} \\
& & CIFAR-10 $\rightarrow$ STL-10 &  & \\
\hline
\multirow{2}*{4} & \multirow{2}*{VGG-19} & CIFAR-100 & \multirow{2}*{72.0 $\rightarrow$ 63.6} & \multirow{2}*{5,000} \\
& & (orig. $\rightarrow$ crop) &  & \\
\hline
\multirow{2}*{5} & \multirow{2}*{ResNet-50} & ImageCLEF & \multirow{2}*{99.2 $\rightarrow$ 73.2} & \multirow{2}*{480} \\
& & (c $\rightarrow$ p) &  & \\
\hline
\multirow{2}*{6} & \multirow{2}*{Inception-v3} & ImageNet & \multirow{2}*{77.5 $\rightarrow$ 45.3} & \multirow{2}*{5,000} \\
& & (orig. $\rightarrow$ down-sample) &  & \\
\hline
\end{tabular}
 \begin{tablenotes}
        \footnotesize
        \item[*] It refers to the maximum number of operation data available for labeling.
      \end{tablenotes}
\end{threeparttable}
\label{tab:ExpDesign}
\end{table}

% In our experiments, we set the number of clusters as 30, 
In Task 1 we applied a LeNet-5 model originally trained 
with the images from the \textbf{MNIST} dataset~\cite{lecun1998gradient} 
to classify images from the \textbf{USPS} dataset~\cite{friedman2001elements}. 
Both of them are popular handwritten digit recognition datasets consisting of 
single-channel images  of size 16$\times$16$\times$1, \added{but the latter is more difficult to read}.
%We will introduce each dataset in the following.
%\textbf{MNIST/USPS} are two ~\cite{lecun1998gradient, friedman2001elements}.
%Each image is single-channel of size 16$\times$16$\times$1.
%
%We randomly selected samples from MNIST and USPS 
%to constructed training and operation domains, respectively. 
The size of the training dataset was 2,000, and the size of the operation dataset was 1,800.
We reserved 900 of the 1,800 operation data for testing, and used the other 900 for operational calibration. 
%For the operation dataset, we divide it into two sets with the same size.
%We use the first set to do the tasks of input selection, input labeling, and building the gaussian process.
%The second set is held out as the test set for operation domain.


Task 2 was focused on natural language processing. 
\textbf{Polarity} is a dataset for sentiment-analysis~\cite{Pang2002sentiment}. 
It consists of sentences labeled with corresponding sentiment polarity (i.e., positive or negative). 
We chose Polarity-v1.0, which contained 1,400 movie reviews collected in 2002, as the training set.
The Polarity-v2.0, which contained 2,000 movie reviews collected in 2004, was used as the data from 
the operation domain. We also reserved half of the operation data for testing. 
%Similarly, for the operation dataset, 
%we divide it into two sets with the same size for calibration and testing.

In Task 3 we used two classic image classification datasets \textbf{CIFAR-10}~\cite{krizhevsky2009learning}
 and \textbf{STL-10}~\cite{coates2011analysis}.
The former consists of 60,000 32$\times$32$\times$3 images in 10 classes, 
and each class contains 6,000 images.
The latter has only 1,3000 images, 
but the size of each image is 96$\times$96$\times$3.
We used the whole CIFAR-10 dataset to train the model. 
The operation domain was represented by 8,000 images collected from STL-10, 
in which 5,000 were used for calibration, and the other 3,000 were reserved for testing.


Tasks 4 used the dataset \textbf{CIFAR-100}, which was more difficult than 
CIFAR-10 and contained 100 classes with 600 images in each.
We trained the model with the whole training dataset of 50,000 images.
To construct the operation domain, we randomly cropped the remaining 10,000 images. % as the operation dataset.
One half of these cropped images were used for calibration and the other half for testing.
%The examples of original domain and operation domain are shown in Figure~\ref{fig:orig-and-opt}.

Task 5 used the image classification dataset from the \textbf{ImageCLEF} 2014 challenge~\cite{Mller2010ImageCLEF}. 
It is organized with 12 common classes derived from three different domains: 
ImageNet ILSVRC 2012 (i), Caltech-256 (c), and Pascal VOC 2012 (p).
We chose the dataset (c) as the origin domain and dataset (p) as the operation domain.
Due to the extremely small size of the dataset, we divided the dataset (p) 
for calibration and testing by the ratio 4:1.
%The examples of original domain and operation domain are shown in Figure~\ref{fig:orig-and-opt}.
 
Finally, Task 6 dealt with an extremely difficult situation. 
\textbf{ImageNet} is a large-scale image classification dataset 
containing more than 1.2 million 224$\times$224$\times$3 images across 1,000 categories~\cite{Deng09imagenet}.
The pre-trained model Inception-v3 was adopted for evaluation.
The operation domain was constructed by down-sampling 10,000 images from the original test dataset.
Again, half of the images were reserved for testing.
%The examples of original domain and operation domain are shown in Figure~\ref{fig:orig-and-opt}.

\begin{figure}[htbp]
\begin{center}
\subfloat[CIFAR-10 (origin domain)]{
\includegraphics[width=.42\columnwidth]{figures/show/cifar10/orig1.png}}
%\includegraphics[width=.4\columnwidth]{figures/show/cifar10/orig2.png}}
\hspace{2em}
\subfloat[STL-10 (operation domain)]{
\includegraphics[width=.42\columnwidth]{figures/show/cifar10/opt1.png}}
%\includegraphics[width=.4\columnwidth]{figures/show/cifar10/opt2.png}} \\

\subfloat[ImageCLEF-(c) (origin domain)]{
\includegraphics[width=.21\columnwidth]{figures/show/imageclef/orig1.png}
\includegraphics[width=.21\columnwidth]{figures/show/imageclef/orig2.png}}
\hspace{2em}
\subfloat[ImageCLEF-(p) {\tiny (operation domain)}]{
\includegraphics[width=.21\columnwidth]{figures/show/imageclef/opt1.png}
\includegraphics[width=.21\columnwidth]{figures/show/imageclef/opt2.png}} \\
%\subfloat[ImageNet-origin]{
%\includegraphics[width=.4\columnwidth]{figures/show/imagenet/orig1.png}
%\includegraphics[width=.4\columnwidth]{figures/show/imagenet/orig2.png}}
%\hspace{2em}
%\subfloat[ImageNet-operation]{
%\includegraphics[width=.4\columnwidth]{figures/show/imagenet/opt1.png}
%\includegraphics[width=.4\columnwidth]{figures/show/imagenet/opt2.png}} 
\caption{Examples of origin and operation domains. 
\added{\rm{In task~3 a ResNet-18 model was trained with low-resolution images (a), but applied to high-resolution images (b). In task~5 a ResNet-50 model was applied to images (d) with backgrounds and styles different from training images (c). }}
%\rm{The left column is the images collected from CIFAR-10 and ImageCLEF-c, which are used as the original data. 
%The right column is the images collected from STL-10 and ImageCLEF-p, which are used as the operation data.}
}
\label{fig:orig-and-opt}
\end{center}
\end{figure}


\subsection{Efficacy of operational calibration}

Table~\ref{tab:brier-score} gives the Brier scores of the confidence before (col. Orig.) and after (col. GPR) operational calibration. 
In these experiments all operation data listed in Table~\ref{tab:ExpDesign} (not including the reserved test data) were labeled and used in the calibration.
The result unambiguously confirmed the general efficacy of our approach. 
%and its superiority over alternative approaches. 
In the following we elaborate on its relationship with the fine-tuning technique often employed in practice.  
%and how it was compared with other approaches.   

\begin{table*}[htb]
\caption{Brier scores of different calibration methods}
\centering
% \setlength{\tabcolsep}{.38em}
\begin{threeparttable}
\begin{tabular}{|p{0.6cm}<{\centering}|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}*{\textbf{Task}} & \multirow{2}*{\textbf{Model}} & \multirow{2}*{\textbf{Orig.}} & \multicolumn{3}{c|}{\textbf{Operational calibration}} & \multicolumn{4}{c|}{\textbf{Conventional calibration}} & \multirow{2}*{\textbf{SAR}}  \\
\cline{4-10} 
  & & & \textbf{GPR} & \textbf{RFR} & \textbf{SVR} & \textbf{TS} & \added{\textbf{PS-conf.}} & \added{\textbf{PS-logit}} & \added{\textbf{IR}} &   \\
\hhline{|===========|}
1  & LeNet-5 & 0.207 & \textbf{0.114} & 0.126 & 0.163 & 0.183 & \added{0.316}  & \added{0.182} & \added{0.320} & 0.320 \\
\hline
2  & RNN & 0.203 & \textbf{0.102} & 0.107 & 0.202 & 0.185 & \added{0.641} & \added{0.125} & \added{0.655} & 0.175 \\
\hline %\hhline{|======|}
3  & ResNet-18 & 0.474 & \textbf{0.101} & 0.121 & 0.115 & 0.387 & \added{0.471} & \added{0.254} & \added{0.529} & 0.308 \\
\hline
4  & VGG-19 & 0.216 & \textbf{0.158} & 0.162 & 0.170 & 0.217 & \added{0.359}  & \added{0.253} & \added{0.364}  & 0.529 \\
\hline
5  & ResNet-50 & 0.226 & \textbf{0.179} & 0.204 & 0.245 & 0.556 & \added{0.789}  & \added{0.319} & \added{0.925}  & 0.364 \\
\hline
6  & Inception-v3 & 0.192 & \textbf{0.161} & 0.167 & 0.217 & 0.191 & \added{0.546} & \added{0.427} &  \added{0.334} & - \\
\hline
\end{tabular}
 \begin{tablenotes}
        \footnotesize
        \item 	Orig.--Before calibration. 
        		GPR--Gaussian Process-based approach.
				RFR--Random Forest Regression in the representation space.
				SVR--Support Vector Regression in the representation space.
				TS--Temperature Scaling~\cite{guo2017calibration}.
				\added{PS--Platt Scaling~\cite{Platt1999probabilisticoutputs}.
				IR--Isotonic Regression Scaling~\cite{zadrozny2002transforming}.
				Conf./Logit indicates that the calibration took confidence value/logit as input. }
				SAR--Regression with Surprise values~\cite{kim2019guiding}.
				We failed to evaluate SAR on task 6 because it took too long to run on the huge dataset.
  \end{tablenotes}
\end{threeparttable}
\label{tab:brier-score}
\end{table*}


\subsubsection{Calibration when fine-tuning is ineffective}

A machine learning engineer might first consider to apply 
fine-tuning tricks to deal with the problem of domain shift. 
However, for non-trivial tasks, such as our tasks 4, 5, and 6,
it can be very difficult, if possible, to fine-tune the DNN model 
with small operation datasets. 
Figure~\ref{fig:fine-tune1} shows the vain effort in fine-tuning 
the models with all the operation data (excluding test data). 
We tried all tricks including data augmentation, weight decay, and regularization 
to avoid over-fitting but failed to improve the test accuracy.  

\begin{figure*}[htbp]
\begin{center}
\subfloat[Task 4]{
\includegraphics[width=0.62\columnwidth]{figures/learn-curve/cifar100.pdf}}
\subfloat[Task 5]{
\includegraphics[width=0.62\columnwidth]{figures/learn-curve/imageclef.pdf}}
\subfloat[Task 6]{
\includegraphics[width=0.62\columnwidth]{figures/learn-curve/imagenet.pdf}}
\caption{Ineffective fine-tuning of difficult tasks.
\added{\rm{All available operation data (5000, 480, and 5000, respectively) were used. }}}
\label{fig:fine-tune1}
\end{center}
\end{figure*}

Fortunately, our operational calibration worked quite well in these difficult situations. 
In addition to the improvement in Brier scores reported in Table~\ref{tab:brier-score}, 
we can also see the saving of LCE for task~4 in Figure~\ref{fig:LCE-1} as an example. 
Our approach reduced about a half of the LCE when $\lambda > 0.8$, 
which indicates its capability in reducing high confidence errors.   

%
%For 
%\emph{fine-tune technique with \textbf{***xjw::limited dataset***} could not 
%increase the accuracy of model on the specific operation domain}.
%We confirm this point through the following experiments:
%we employ the whole operation set for calibration 
%to fine-tune the model previously trained on original domain.
%Due to the small size of operation data, 
%data augmentation, weight decay, and regularization 
%are all applied to avoid over-fitting.
%The experimental results are shown in Figure~\ref{fig:fine-tune1}.
%For task 4 and task 5, 
%that models quickly overfit to the the limited operation datasets.
%However, the accuracy of operation domain even decline slightly. 
%For the last task, in addition to the difficulty of the dataset (e.g.,~ImageNet), 
%the operation of down-sampling has lost much information from original image.
%Thus it is hard for the model to learn knowledge from such operational images.
%
%Although the fine-tuning technique does not work well in such tasks, 
%our calibration approach can still correct the corresponding confidence to 
%improve the decision quality of DNN. 
%The experimental results in Table~\ref{tab:brier-score} prove this claim. 
%The brier scores~\textbf{***xjw::add Equation number***} for these three tasks descend  
%from 0.216 to 0.158, 0.226 to 0.179, and 0.191 to 0.161, respectively.
%It is worth noting that even for the ImageNet dataset, which is the most difficult task, 
%the calibration still be effective 
%, but its benefit brought by calibration is small 
%due to the large number of classes. 
%To evaluate the profit from decreasing the brier score, 
%we compute the LCE with different $u/(1+u)$ for task 4.
%For details, we choose $u/(1+u)$ from 0.05 to 0.95 with interval 0.05 
%to calculate how much LCE can be reduced by our approach 
%under the different loss $u$. 
%The experimental results are provided in Figure~\ref{fig:LCE-1}.
%When the loss for false prediction is small 
%(e.g., $u = 1/9$), 
%our calibration approach could not save loss in this situation.
%However, when the loss for prediction is large
%(e.g., $u = 9$),  
%the calibration approach shows amazing effect:
%the calibration approach can nearly save 60\% loss per input. 
%\textbf{***xjw::add several sentences to discuss other compared methods***}




\begin{figure}[htbp]
\begin{center}
\includegraphics[width=0.70\columnwidth]{figures/LCE/cifar100.pdf}
\caption{loss due to confidence error}
\label{fig:LCE-1}
\end{center}
\end{figure}


%\begin{figure*}[htbp]
%\begin{center}
%\subfloat[Vgg19~(cifar-100 $\rightarrow$ affine transformation)]{
%\includegraphics[width=0.7\columnwidth]{figures/efficacy/cifar100.pdf}} 
%\subfloat[ResNet-50~(imageclef-c $\rightarrow$ imageclef-p)]{
%\includegraphics[width=0.7\columnwidth]{figures/efficacy/imageclef.pdf}}
%\subfloat[Inception-v3~(imagenet $\rightarrow$ down-sample)]{
%\includegraphics[width=0.7\columnwidth]{figures/efficacy/imagenet.pdf}} 
%\caption{loss due to confidence error}
%\label{fig::LCE-1}
%\end{center}
%\end{figure*}

%\begin{figure*}[htbp]
%\begin{center}
%\subfloat[LeNet-5~(mnist $\rightarrow$ usps)]{
%\includegraphics[width=1\columnwidth]{figures/efficacy/mnist.pdf}}
%\subfloat[RNN~(Polarity-v1.0 $\rightarrow$ Polarity-v2.0)]{
%\includegraphics[width=1\columnwidth]{figures/efficacy/polarity.pdf}} \\
%\subfloat[ResNet-18~(cifar-10 $\rightarrow$ stl-10)]{
%\includegraphics[width=1\columnwidth]{figures/efficacy/cifar10.pdf}}
%\caption{loss due to confidence error}
%\label{fig::LCE-2}
%\end{center}
%\end{figure*}


\subsubsection{Calibration when fine-tuning is effective}

In case of easier situations that fine-tuning works, 
we can still calibrate the model to give more accurate confidence. 
Note that effective fine-tuning does not necessarily provide accurate confidence. 
One can first apply fine-tuning until test accuracy does not increase, 
and then calibrate the fine-tuned model with the rest operation data.  


For example, we managed to fine-tune the models in our tasks 1, 2, and 3.~\footnote{%
Here we used some information of the training process, such as the learning rates, weight decays and training epochs. Fine-tuning could be more difficult because these information could be unavailable in real-world operation settings.  
} 
Task 1 was the easiest to fine-tune and its accuracy kept increasing 
and exhausted all the 900 operational examples.
Task 2 was binary classification, in this case our calibration was actual 
an effective fine-tuning technique. 
Figure~\ref{fig:ft-cali2} shows that our approach was 
more effective and efficient than conventional fine-tuning as it converged more quickly. 
For task 3 with fine-tuning the accuracy stopped increasing at about 79\%, 
with about 3,000 operational examples.  
Figure~\ref{fig:ft-cali3} show that, 
the Brier score would decrease more if we spent rest operation data on calibration 
than continuing on the fine-tuning. 


\begin{figure}[htbp]
\begin{center}
\subfloat[\added{Task 2}]{
\includegraphics[width=0.5\columnwidth]{figures/brier-score/polarity.pdf}
\label{fig:ft-cali2}}
\subfloat[\added{Task 3}]{
\includegraphics[width=0.5\columnwidth]{figures/brier-score/cifar10.pdf}
\label{fig:ft-cali3}}
\caption{Calibration when fine-tuning is effective}
\end{center}
\end{figure}

%\begin{figure}[htbp]
%\begin{center}
%\includegraphics[width=0.45\columnwidth]{figures/brier-score/polarity.pdf}
%\caption{Operational calibration vs. Fine-tuning: Task 2}
%\label{fig:ft-cali2}
%\end{center}
%\end{figure}
%
%\begin{figure}[htbp]
%\begin{center}
%\includegraphics[width=0.45\columnwidth]{figures/brier-score/cifar10.pdf}
%\caption{Operational calibration after fine-tuning: Task 3}
%\label{fig:ft-cali3}
%\end{center}
%\end{figure}


Based on the significant (16.1\%-78.6\%) reductions in Brier scores in all of the tasks reported in Table~\ref{tab:brier-score} and the above discussions,
we conclude that \emph{the Gaussian Process-based approach to operational calibration
is generally effective, 
and it is worthwhile no matter whether the fine-tuning works or not}.  


%\begin{figure*}[htbp]
%\begin{center}
%%\subfloat[Task-1]{
%%\includegraphics[width=0.7\columnwidth]{figures/brier-score/mnist.pdf}}
%\subfloat[Task-2]{
%\includegraphics[width=1.0\columnwidth]{figures/brier-score/polarity.pdf}}
%\subfloat[Task-3]{
%\includegraphics[width=1.0\columnwidth]{figures/brier-score/cifar10.pdf}}
%\caption{The calibrated brier score of fine-tuned model}
%\label{fig:ft-cali}
%\end{center}
%\end{figure*}
%
%
%
%
%
%\begin{figure*}[htbp]
%\begin{center}
%\subfloat[Task-1]{
%\includegraphics[width=0.7\columnwidth]{figures/learn-curve/mnist.pdf}}
%\subfloat[Task-2]{
%\includegraphics[width=0.7\columnwidth]{figures/learn-curve/polarity.pdf}}
%\subfloat[Task-3]{
%\includegraphics[width=0.7\columnwidth]{figures/learn-curve/cifar10.pdf}}
%\caption{The fine-tuning of simple tasks}
%\label{fig:fine-tune2}
%\end{center}
%\end{figure*}
%
%
%In addition, for the first three tasks where fine-tuning method could work well, 
%it is difficult to choose the parameters (e.g., learning rate, weight decay, etc.).
%If the user 
%lacks the prior knowledge of training process or 
%some understandings of fine-tuning technique, 
%the fine-tuning may still be useless 
%and even decrease the accuracy of model.
%Furthermore, 
%in some situation, 
%it is not permitted to modify the model, e.g., 
%the model my be provided as a web service, 
%we could only get the limited information (e.g., outputs from last and/or penultimate layers) returned from the service.
%When we target to operation domain, the only thing we can do is to calibrate these outputs.
%%they need to finish the ensemble learning tasks 
%%or they will reuse the model in the future.
%In this part, we apply calibration without fine-tuning for the first three relatively simple tasks.
%The experimental results are shown in Table~\ref{tab:brier-score}, 
%The brier scores decrease from 0.207, 0.203, and 0.474 to 0.114, 0.102, and 0.101, respectively.
%\textbf{***xjw::add several sentences to discuss other compared methods***}
%% Above all, 
%
%
%
%
%
%As we discussed earlier, for relatively simple tasks (i.e., task 1, task 2, and task3),
%\emph{fine-tuning method is able to increase the accuracy of model on operation domain}. 
%However, the increasing of accuracy does not mean that 
%the reliability of confidence is also improved.
%In other words, fine-tuning could not ensure the model well-calibrated.
%Thus, the confidence calibration is still needed in this situation.
%In order to calibrate confidence after fine-tuning,
%we hold out a small proportion of data for calibration.
%%For given sample size, instead of use the whole datasets for fine-tuning, 
%For details, we first run fine-tuning to make 
%the accuracy of the model nearly convergence, 
%and then start calibration to further reduce the brier score.
%Taking task 3 as an example,  
%we find that when the sample size exceeds 3,000, 
%there is no significant improvement for fine-tuning by further applying samples.
%Therefore, we use the remaining samples to calibrate the fine-tuned model.
%The brier score of calibration for fine-tuned model are plotted in Figure~\ref{fig:calibration+fine-tune}. 
%For task 2, we also should calibrate the model after fine-tuning, 
%but this task is a two-class classification problem, 
%thus calibration is equivalent to fine-tuning. 
%In this sense, we directly compare the calibration and fine-tuning, 
%From Figure~\ref{fig:calibration+fine-tune} we find that our gaussian process calibration 
%can converge faster to final brier score than fine-tuning does. 
%Using only 150 samples can achieve the same performance of fine-tuning with 1,000 samples.
%We think that the reason of such novel efficiency is 
%due to our calibration method makes full use of 
%the representative ability of the model 
%so that can use less samples but achieve same brier score.
%For task 1, we find that the accuracy is still increasing when adding more samples for fine-tuning. 
%In this situation, we recommend user continuing fine-tuning the model until the accuracy convergence.
%
%\begin{figure*}[htbp]
%\begin{center}
%%\subfloat[Task-1]{
%%\includegraphics[width=0.7\columnwidth]{figures/brier-score/mnist.pdf}}
%\subfloat[Task-2]{
%\includegraphics[width=1.0\columnwidth]{figures/brier-score/polarity.pdf}}
%\subfloat[Task-3]{
%\includegraphics[width=1.0\columnwidth]{figures/brier-score/cifar10.pdf}}
%\caption{The calibrated brier score of fine-tuned model}
%\label{fig:fine-tune3}
%\end{center}
%\end{figure*}
%

\subsection{Comparing with alternative methods}

\added{First, we applied three widely used calibration methods, \emph{viz.} Temperature Scaling (TS)~\cite{hinton2015distilling}, 
Platt Scaling (PS)~\cite{Platt1999probabilisticoutputs}, and Isotonic Regression (IR)~\cite{zadrozny2002transforming},
with the same operation data used in our approach.
%
TS defines the calibration function $R$ in Equation~\ref{equ:logitcali} as $R(\bm{h}) = \bm{h}/T$,  
where $T$ is a scalar parameter computed by minimizing the 
negative log likelihood~\cite{hastie2009elements}
on a validation dataset. 
PS and IR directly work on the confidence values. 
PS trains a one-dimensional logistic regression and calibrates confidence 
as $\hat{c} = 1/(1+e^{-a\cdot c_{\mathfrak{M}}+b})$, 
where $a, b$ are scalar parameters computed by minimizing the cross entropy on a validation dataset.
IR simply fits a monotonic confidence calibration function minimizing 
the Brier score on a validation dataset. 
Note that in our experiment, the operation data were used instead of the validated dataset. 
We implemented TS according to~\citet{guo2017calibration}. For PS and IR we used the
well-known machine learning library scikit-learn~\cite{scikit-learn}.
} 


%\footnote{\added{These two methods have been well developed in machine learning library scikit-learn~\cite{scikit-learn}, one can refer to sklearn.calibration.CalibratedClassifierCV.}}


% There exist different kinds of calibration methods, such as isotonic regression~\cite{zadrozny2002transforming}, 
% histogram binning~\cite{zadrozny2002transforming}, and Platt scaling~\cite{Platt1999probabilisticoutputs}. 
% \added{These methods all attempt to train a regression model whose input is confidence. 
% The first two methods are implemented based on isotonic regression and binning, and the last method define the calibration function as}
% \begin{equation}
% \added{R(c) = \frac{1}{1+e^{-(a \cdot c + b)}},}
% \end{equation}
% \added{where $c$ is the input of confidence value, and $a, b$ are parameter computed by minimizing the cross entropy on the validation dataset. }
% However, according to a recent study~\cite{guo2017calibration}, 
% the most effective choice is often a simple method called Temperatures Scaling~\cite{hinton2015distilling}.
% The idea is to define the calibration function as
%  \begin{equation}
%  R(\bm{h}) = \frac{\bm{h}}{T}, 
%  \end{equation}
% where $T$ is a scalar parameter computed by minimizing the 
% negative log likelihood~\cite{hastie2009elements}
% on the validation dataset. 
% \added{Moreover, Platt scaling can also be improved through taking logit as input~\cite{guo2017calibration}, i.e., define the calibration function as}
%  \begin{equation}
%  \added{R(\bm{h}) = \bm{W}^{\mathsf{T}}\bm{h}+\bm{b}, }
%  \end{equation}
%  \added{where $\bm{W}$ is a matrix parameter and $\bm{b}$ is a vector parameter. 
%  Both of these two parameters are computed by minimizing the cross entropy. }


%First, Temperature Scaling~\cite{hinton2015distilling}, which is reported to be the most effective conventional confidence calibration method~\cite{guo2017calibration}, was applied with the same operation data used in our approach.
As shown in Table~\ref{tab:brier-score}, TS, 
although reported to be usually the most effective conventional confidence calibration method~\cite{guo2017calibration},
was hardly effective in these cases. 
It even worsened the confidence in tasks 4 and 5. 
We observed that its bad performance  
came from the significantly lowered resolution part of the Brier score, 
which confirmed the analysis in Section~\ref{subsec:discussions}.
For example, in task 3, with Temperature Scaling the reliability decreased from 0.196 to 0.138, but the resolution dropped from 0.014 to 0.0. 
In fact, in this case the calibrated confidence values were all very closed to 0.5 after scaling. 
However, with our approach the reliability decreased to 0.107,
and the resolution also increased to 0.154. 
\added{The same reason also failed PS (col. PS-Conf.) and IR (col. IR).}

\added{We also included in our comparison an improved version of PS, which built 
a regression over the logit instead of the confidence~\cite{guo2017calibration}. 
Its calibration function $R$ for Equation~\ref{equ:logitcali} was
$R(\bm{h}) = \bm{W}^\mathsf{T} \bm{h} + \bm{b}$,
where $\bm{W}$  and $\bm{b}$ were 
computed by minimizing the cross entropy on the operation data. 
It performed much better than the original PS but 
still failed in tasks 4, 5 and 6.
}

% \added{, be ineffective in operation domain. 
% The details were shown in Table~\ref{tab:brier-score} (col. PS and col.IR). 
% Since the calibration effect is too poor, we tried to improve these two methods, i.e., taking logit as calibration input. 
% The experimental results are available in Table~\ref{tab:brier-score} (col. IPS and col.IIR) }

Second, we also tried to calibrate confidence based on the Surprise value 
that measured the difference in DL system's behavior 
between the input and the training data~\cite{kim2019guiding}.
We thought it could be effective because it also leveraged the distribution of examples 
in the representation space.
We made polynomial regression between the confidence adjustments and the likelihood-based Surprise values. 
Unfortunately, it did not work for most of the cases (col. SAR in Table~\ref{tab:brier-score} ). 
We believe the reason is that Surprise values are scalars 
and cannot provide enough information for operational calibration.  

Finally, to examine whether Gaussian Process Regression (GPR) is the right choice for our operational calibration framework, 
we also experimented with two standard regression methods, viz. 
Random Forest Regression (RFR) and Support Vector Regression (SVR). 
We used linear kernel for SVR and ten decision trees for RFR.
As shown in Table~\ref{tab:brier-score}, in most cases, the non-liner RFR performed better than the linear SVR, 
and both of them performed better than Temperature Scaling but worse than GPR.
The result indicates that (1) calibration based on the features extracted by the model 
rather than the logits computed by the model is crucial, 
(2) the confidence error is non-linear and unsystematic,   
and (3) the Gaussian Process as a Bayesian method can provide better estimation of the confidence. 


In summary, \replaced{our GPR approach achieved significant Brier Score reduction and outperformed 
conventional calibration methods and the Surprise value-base regression in all the tasks.}{
the Brier score reductions of our GPR approach were       
at least 3.87 times of that of Temperature Scaling and 2.24 times of Surprise value-base regression.} 
It also outperformed alternative implementations based on RFR and SVR. 
So we conclude that 
 \emph{our approach is more effective than Temperature Scaling and 
other alternative choices for operational calibration}.

%
%We also compared our approach with (1) 
%
%Here we compare our calibration approach with other DNN quality assurance methods.
%Following the temperature scaling which is the state-of-art calibration technique in machine learning,
%the surprise adequacy was applied to ensure the confidence accurate on operation domain.
%Finally, we explain the rationale of choosing gaussian process through comparing with other regression techniques.
%
%Researchers have proposed many methods to ensure the quality of models~\cite{XXX} in last years. 
%We want to know whether our method outperforms the other DNN quality assurance methods.  
%In this evaluation, we compare our calibration approach with two state-of-the-art methods, 
%i.e., temperature scaling and surprise adequacy.
%
%For surprise adequacy method, we choose 
%likelihood-based surprise adequacy (i.e., LSA)
%as the measurement for surprise value of operation data. 
%Notice that the original data must be available for computing the surprise value.
%Thus we provide the original data for this method.
%Because the output of LSA is scalar, 
%we use polynomial regression to calibrate the confidence: 
%the input of regression is surprise value 
%and the output of regression is the confidence difference.
%
%
%The experiments are conducted on all datasets except ImageNet due to the extremely large original dataset.
%As we can see, the results show that the LSA method is not able to 
%
%
%capture the confidence changes on the operation domain. 
%We think the reason for ineffectiveness is that
%the operation data are all surprises compared with original data.
%\textbf{***where is temperature scaling?***}
%
%Besides from the above methods, 
%we also conduct some experiments to show the rationality of gaussian process. 
%Specifically, 
%we apply Random Forest (RF) and Support Vector Regression (SVR) as the compared methods
%to calibrate the confidence. 
%In evaluation, we choose linear kernel for SVR and ten decision trees for RF.
%The experimental results are shown in Table~\ref{brier-score}. 
%We can see that linear regression methods (e.g., linear SVR) 
%cannot describe the changes of confidence on operation domain effectively. 
%The non-linear regression method can capture some changes, 
%but such tree model cannot learn the locality of inputs in representation space suitably\textbf{***stablely?***}. 
%Notice that
%the dimension of representation space is still too high 
%for such regression methods, 
%which leads training process very time-consuming
%compared to non-parametric gaussian process.

\subsection{Efficiency of operational calibration}

In the above we have already shown that our approach worked with 
small operation datasets that were insufficient for fine-tuning (Task 4, 5, and 6). 
In fact, the Gaussian Process-based approach has a nice property 
that it starts to work with very few labeled examples. 
We experimented the approach with the input selection method presented in Section~\ref{subsec:inputselection}.
We focused on the number of high-confidence false predictions, which 
was decreasing as more and more operational examples were labeled and used.  

We experimented with all the tasks but labeled only 10\% of the operation data. 
Table~\ref{tab:efficiency-results} shows the numbers of high-confidence false predictions 
before and after operational calibration. 
As a reference, we also include the numbers of high-confidence correct predictions. 
We can see that most of the high-confidence false predictions were eliminated. 
It is expected that there were less high-confidence correct predictions after calibration, 
because the actual accuracy of the models dropped. 
The much lowered LCE scores, which took into account 
both the loss in lowering the confidence of correct predictions and the gain in lowering the confidence of false predictions, 
 indicate that the overall improvements were significant.  

\begin{table}[htb]
\caption{Reducing high-confidence false predictions with 10\% operation data labeled}
\centering
\setlength{\tabcolsep}{.38em}
\begin{threeparttable}
\begin{tabular}{|p{0.4cm}<{\centering}|p{1.2cm}<{\centering}|c|c|c|c|c|}
\hline
No. & Model & $\lambda$ & Correct pred. & False pred. & LCE \\
\hhline{|======|}
\multirow{2}*{1} & \multirow{2}*{LeNet-5} & 0.8 & 473 $\rightarrow$ 309.1 & \textbf{126$\rightarrow$24.3} & 0.143$\rightarrow$0.089  \\
&  &  0.9  & 417 $\rightarrow$ 141.9 & \textbf{74 $\rightarrow$ 2.5} & 0.096$\rightarrow$0.055 \\
\hline
\multirow{2}*{2} & \multirow{2}*{RNN} & 0.8 & 512 $\rightarrow$ 552.9 & \textbf{118$\rightarrow$39.9} & 0.162$\rightarrow$0.091  \\
&  &  0.9  & 482 $\rightarrow$ 261.3 & \textbf{106 $\rightarrow$12.0} & 0.132$\rightarrow$0.070 \\
\hline
\multirow{2}*{3} & {ResNet} & 0.8 & 1350 $\rightarrow$ 839.2 & \textbf{1372$\rightarrow$59.7} & 0.370$\rightarrow$0.054  \\
& {-18}  &  0.9  & 1314 $\rightarrow$ 424.0 & \textbf{1263 $\rightarrow$9.4} & 0.358$\rightarrow$0.041 \\
\hline
\multirow{2}*{4} & \multirow{2}*{VGG-19} & 0.8 & 1105 $\rightarrow$ 392.5 & \textbf{583$\rightarrow$46.9} & 0.127$\rightarrow$0.070 \\
& &  0.9  & 772$\rightarrow$142.8  & \textbf{280$\rightarrow$9.3} & 0.074$\rightarrow$0.038 \\
\hline
\multirow{2}*{5} & {ResNet} & 0.8 & 53 $\rightarrow$ 26.9 & \textbf{16$\rightarrow$5.2} & 0.162$\rightarrow$0.136  \\
& {-50} &  0.9  & 46 $\rightarrow$ 26.9 &\textbf{10$\rightarrow$2.0} & 0.108$\rightarrow$0.064 \\
\hline
\multirow{2}*{6} & {Inception} & 0.8 & 1160$\rightarrow$692.0 & \textbf{265$\rightarrow$63.6} & 0.087$\rightarrow$0.073 \\
& {-v3} & 0.9 & 801$\rightarrow$554.1 & \textbf{137 $\rightarrow$ 40.2} & 0.054$\rightarrow$0.041 \\
\hline
\end{tabular}
 \begin{tablenotes}
        \footnotesize
        \item %To obtain the statistical results, 
        		We ran each experiment 10 times and computed the average numbers.% numbers of correct predictions and false 		          predictions.
  \end{tablenotes}
\end{threeparttable}
\label{tab:efficiency-results}

\end{table}


For a visual illustration of the efficiency of our approach, 
Figure~\ref{fig:efficiency-curve}  plots the change of proportions of 
high-confidence false and correct predictions as the size of data used in calibration increases. %Task 3.  
%Other tasks are similar and omitted here to save space. 
It is interesting to see that: 
(1) most of the high-confidence false predictions were identified very quickly, and
(2) the approach was conservative, 
but the conservativeness is gradually remedied with more labeled operation data used. 

\begin{figure}[htbp]
\begin{center}
\subfloat[Task 1]{
\includegraphics[width=0.5\columnwidth]{figures/efficiency/mnist/0dot9.pdf}}
\subfloat[Task 2]{
\includegraphics[width=0.5\columnwidth]{figures/efficiency/polarity/0dot9.pdf}}

\vspace{-2ex}
\subfloat[Task 3]{
\includegraphics[width=0.5\columnwidth]{figures/efficiency/cifar10/0dot9.pdf}}
\subfloat[Task 4]{
\includegraphics[width=0.5\columnwidth]{figures/efficiency/cifar100/0dot9.pdf}}

\vspace{-2ex}
\subfloat[Task 5]{
\includegraphics[width=0.5\columnwidth]{figures/efficiency/imageclef/0dot9.pdf}}
\subfloat[Task 6]{
\includegraphics[width=0.5\columnwidth]{figures/efficiency/imagenet/0dot9.pdf}}
\caption{The proportion curve of high confidence inputs.
\added{\rm{Sample size 0 means uncalibrated. The calibration started to take effect with very few data.}}}
\label{fig:efficiency-curve}
\end{center}
\end{figure}

Note that for tasks 4, 5 and 6, 
usual fine-tuning tricks did not work even with all the operation data labeled.
With our operational calibration, using only about 10\% of the data, 
we avoided about 97\%, 80\%, and 71\% high-confidence ($>$$0.9$) errors, respectively.

Based on the results, we can say that \emph{the Gaussian Process-based operational calibration 
is efficient in detecting most of the high-confidence errors with a small amount of labeled operation data}. 


%
%
%
%Here we evaluate our operational calibration method in terms of
%calibrating the high confident misclassifications.
%In evaluation, 
%we respectively set the confidence threshold as 0.8 and 0.9.
%In other words, we are more inclined to calibrate the inputs 
%whose confidences are greater than 0.8 and 0.9.
%We conduct the experiments for all tasks, 
%due to the page limitation, we only plot the experimental results of task 4 in Figure~\ref{fig:efficiency-curve}. 
%The blue line is the proportion of 
%inputs with high confidence to total inputs, 
%and the red line is the proportion of 
%misclassified inputs with high confidence to total inputs.
%The results show that our calibration approach
%nearly reduces 60\% of inputs with high confidence.
%We think it is an acceptable result,
%because the accuracy is dropped on operation domain.
%At the same time, the high confidence dropped nearly 90\%, 
%only a few inputs are misclassified with high confidence.
%
%
%
%In addition, we only use 10\% of the whole inputs for labeling 
%and build the gaussian process. 
%Then the number of high confidence false predictions 
%and high confidence correct predictions are counted respectively.
%The detailed results are provided in Table~\ref{tab:efficiency-results}.
%
%There is no exact specification for the optimal number of inputs with high confidences, 
%let alone the number of misclassified inputs with high confidences.
%Thus we could only use the LCE as the specification, which is also recorded in Table~\ref{tab:efficiency-results}. 
%
%As shown in Table~\ref{tab:efficiency-results}, we can conclude that our calibration method is very efficient. 
%With a few samples to building gaussian process, in relative simple tasks (i.e., task 1,2, and 3), 
%we can reduce about 90\% of misclassified inputs whose confideces are greater than 0.9, 
%and reduce at least 80\% of misclassified inputs whose confidences are greater than 0.8.
%In the rest complex tasks (i.e., 4,5 and 6), 




==> zip/introduction.tex <==
% !TEX root = main.tex

\section{Introduction}
Deep learning (DL) has achieved human-level or even better performance in some difficult tasks, 
such as image classification and speech recognition~\cite{LeCun:2015aa, Goodfellow-et-al-2016}.
Deep Neural Network (DNN) models are increasingly adopted in high-stakes application scenarios such as medical diagnostics~\cite{obermeyer2016predicting} and self-driven cars~\cite{bojarski2016selfdriven}. 
However, it is not uncommon that DNN models perform poorly in practice~\cite{Riley2019nature}.
The interest in the quality assurance for DNN models as integral parts of software systems 
is surging in the community of software engineering~\cite{pei2017deepxplore, ma2018combinatorial, sun2018concolic, zhang2018deeproad, kim2019guiding, zhang2019surveyMLT}.


%one reason for machine learning misprediction bugs is no or poor calibration. This paper proposes an approach to debug this types of bugs via operational calibration. 

%Different from human written programs, a DNN model is intrinsically uncertain, 
%and it never promises to produce a definitely correct output (prediction) for an input.
%So individual incorrect outputs are not necessarily bugs. 
%However, besides the prediction for an input, 
%the model also provide a confidence value that 
%quantifies the likelihood of correctness for this prediction.   
%Accurate confidence information is important in real-wold decision making~\cite{guo2017calibration}.
%%A model with its confidence well calibrated for a given operation domain
%%knows when it works well and when not, and reduces the loss due to over- and under-confidence in decisions.
%For example, an over-confident benign prediction for a pathology image 
%could mislead a doctor into overlooking a malignant tumor, 
%while an under-confident benign prediction could result in unnecessary confirmatory testings. 
%\textcolor{red}{



\deleted{
While machine learning is primarily concerned with how well a model learns from its training data, 
software engineering must pay more attention to how well the trained model performs in the field.
This means that the quality assurance of DNN models used as software components needs to be \emph{operational}. 
In addition, it needs to be \emph{stochastic} to embrace the intrinsic uncertainty of the models 
and \emph{effective} to best utilize the effort in collecting and labeling operation data. 
}

A particular problem of using a previously \added{well-}trained DNN model in an operation domain is that 
the model may not only make more-than-expected mistakes in its predictions,  
but also give erroneous confidence values for these predictions. 
\deleted{Arguably the} \added{The} latter issue is \deleted{more harmful} \added{particularly problematic for decision making}, 
because if the confidence values were accurate, the model would be at least partially usable by accepting only high-confidence predictions.   
It needs to be emphasized that erroneous  predictions with high confidence are especially damaging 
because users will take high stakes in them. 
For example, an over-confident benign prediction for a pathology image 
could mislead a doctor into overlooking a malignant tumor.

The problem comes from the almost inevitable divergences between 
the original data on which a model is trained and the actual data in its operation domain,
which is often called \emph{domain shift} or \emph{dataset shift}~\cite{ng2016nuts}
 in the machine learning literature.
%The popular machine learning tricks (e.g., fine-tuning,  transfer learning~\cite{pan2009survey,wang14icml}, etc.) is difficult to solve this problem due to two practical restrictions in field:
It can be difficult and go beyond the stretch of usual machine learning tricks 
such as fine-tuning and transfer learning~\cite{pan2009survey,wang14icml}, 
because of two practical restrictions often encountered. 
First, %when a DNN model is provided by a third party, 
%its training data are sometimes 
the training data of a third-party DNN model are often
unavailable due to privacy and proprietary limitations~\cite{zhou2016learnware, Shokri2015CCS, konevcny2016federated}.
Second, one can only use a small number of labeled operation data 
because it could be very expensive to label the data collected in the field. 
For example, in an AI-assisted clinical medicine scenario, 
surgical biopsies may have to be involved in the labeling of radiology images.




%However, due to the fundamental difference between DNN models and human written programs,  
 
 
 
%Considering the inductive nature of deep learning~\cite{Goodfellow-et-al-2016}, 
%an essential problem %of adopting well trained DNN models as integral parts of practical software systems 
%is that DNN models might not work as well as expected under field conditions, 
%because the slight distribution divergences almost always exist between  
%the training data and the operation data in field. 
%The phenomena is usually called domain shift or dataset shift in the machine learning literature. 
%%
%The problem can be difficult and goes beyond the stretch of usual machine learning tricks 
%such as fine-tuning and transfer learning~\cite{pan2009survey,wang14icml} because of two practical 
%restrictions often encountered. First, the DNN model is provided by a third party, 
%and its training data are unavailable due to privacy and proprietary limitations~\cite{zhou2016learnware, Shokri2015CCS, konevcny2016federated}.
%Second, one can only use a small number of labeled operation data, 
%because it is expensive to label the data collected in field. 
%For example, in an AI-aided clinical medicine scenario, 
%surgical biopsies could be involved in the labeling of radiology or pathology images.

%Despite these stringent restrictions, 
%From a software engineering perspective, it is crucial  
%to know quantitatively \emph{how well} a DNN model will work in a given operation domain. 
%In this paper we focus on classifiers. 
%The ``how-well'' is characterized not only collectively with metrics such as model accuracy or precision, 
%but also individually with the \emph{confidence} for the prediction on each given input,  
%which estimates the likelihood of correctness for this prediction. 
% 
%Recently, Li et al proposed an efficient approach to the \emph{operational testing} of DNNs that significantly
%reduces the labeling cost in estimating a model's \emph{overall} operational accuracy~\cite{li2019boosting}. 
%Different from this operational testing, 


We consider \emph{operational calibration} 
that corrects the error in the confidence provided by a DNN model 
for its prediction on each input in a given operation domain. 
It does not change the predictions themselves  
%but fixes the erroneous confidence to the correct one.
but tells when the model works well and when not.
\added{As the quantification of the intrinsic uncertainty in the predictions made by a model, 
confidence values are integral parts of the model's outputs.
So operational calibration can be viewed as a kind of \emph{debugging} activity 
that identifies and fixes errors in these parts of model outputs. 
It improves the model's quality of service in the field 
with more accurate confidence for better decision making. } 
%
\replaced{As a quality assurance activity, operational calibration 
shall be carried out during the deployment of a previously trained DNN model 
in a new operation domain.
One can also incorporate it into the system and excise it from time to time to adapt 
the model to the evolving data distribution in the operation domain.
}{In this sense, operational calibration is a necessary debugging step 
%for fixing confidence errors
that should be incorporated in the engineering of the whole system. 
It fits a perviously trained DNN model to its operational domain with calibrated confidence for better decision making.  
Also, one can incorporate it into the system and excise it at runtime to continuously adapt to the evolutions in the operation domain.
} 
\deleted{We note that operational calibration is challenging because what it fixes is a function, not just a value.} 
%It also needs to be %effective, i.e., improving the accuracy of confidence values, and 
%efficient, i.e., reducing the effort in labeling operation data. 
%It is related to, but different from, the confidence calibration 
%extensively studied in the machine learning community~\cite{flach2016calibration, guo2017calibration}. 
%As to be discussed in Section~\ref{sec:problem} and evaluated in Section~\ref{sec:evaluation}, 
%existing confidence calibration methods are not targeted at specific operation domains 
%and ineffective for our purpose. 









It is natural to model operational calibration as a \added{case} \deleted{kind} of non-parametric Bayesian Inference 
and solve it with Gaussian Process Regression~\cite{rasmussen2005GPML}.  
We take the original confidence of a DNN model as the prior, 
and gradually calibrate the confidence with the evidence collected by selecting and labeling operation data. 
The key insight into effective and efficient regression comes from two observations:
First, the DNN model, although suffering from the domain shift, %the distribution divergence between operation and training data,
can be used as a feature extractor with which unlabeled operation data
can be nicely clustered~\cite{zhu2005semi, shu2018a}. 
In each cluster, the prediction correctness of an example is correlated with another one. 
The correlation can be effectively estimated with the distance of the two examples in the feature space.
Second, Gaussian Process is able to quantify the uncertainty after each step, 
%Notice that the advantage of Gaussian Process is to quantify the uncertainty after each step, 
which can be used to guide the selection of operation data to label efficiently. 
%and those examples that will reduce the highest uncertainty will be selected labeled for next step. 
%In this way the efficiency of approach is further improved. 

Systematic empirical evaluations showed that the approach was promising. 
It \deleted{significantly} outperformed existing calibration methods in both efficacy and efficiency
in all settings we tested. 
In some difficult tasks, it eliminated about 71\% to 97\% high-confidence errors 
with only about 10\% of the minimal amount of labeled operation data 
 needed for practical learning techniques to barely work.
\deleted{In practice, such few operation data can be collected as feedback during a system's runtime, 
and largely improve the system's reliability for its later decisions to make.} 
%
%  
%They are also  
%Therefore, how to assess and improve the reliability of DNN-based systems becomes a highly relevant problem and has attracted much research.  
%
%Recently, many works~\cite{ma2018deepgauge, pei2017deepxplore, ma2018combinatorial, sun2018concolic, zhang2018deeproad, kim2019guiding} based on structural coverage of DNN are proposed for searching adversarial inputs. 
%These testing methods are similar to \emph{debug testing}~\cite{frankl1998evaluating} in traditional software testing, 
%and they think that the adversarial examples are the bugs of the DNN model that needs to be fixed.  
%However, it is still questionable whether we could consider such adversarial examples as bugs. 
%\citeauthor{grosse2018statistical} found that the distributions between the original dataset and the adversarial dataset are different through the hypothetical test. 
%And lately, 
%\citeauthor{ilyas2019adversarial} proposed that the adversarial examples are features rather than the bugs of the model. 
%Besides, the effectiveness in searching adversarial inputs of these coverage-based testing methods needs exploration: 
%\citeauthor{li2019structural} pointed out that such testing methods could not transfer the wisdom of coverage in traditional software testing into debug DNN testing successfully, 
%and their preliminary study suggests that structural coverage criteria for neural networks can be misleading since there exists no correlation between coverage and fault-finding effectiveness. 
%
%Contrasting to these debug DNN testing aimed at generating artificial adversarial examples, 
%we focus on \emph{operational DNN testing},  
%i.e., testing a completely trained DNN model on a specific operational context. 
%This specific context is the actual application context that may differ from the original training/test context, 
%and the inputs of operational DNN testing are the data collected from it. 
%Particularly, when applying a completely trained DNN into practice, the discrepancy between original training context and application context may disturb the performance of the model.
%And the operational DNN testing is intent upon evaluating and ensuring the actual performance in the operational context.
%Consequently, An effective and efficient testing method for the DNN model under the operation environment is crucial.
%
%The main reasons that operational DNN testing worth researching are as follows:  
%\begin{itemize}[leftmargin=*]
%\item The \emph{statistical nature} of the DNN model. 
%The DNN model indeed is the inductive program that could not handle the arbitrary input correctly. 
%Therefore, an individual error-inducing input could not explain the performance of the model at all. 
%Moreover, the No-Free-Lunch theorem indicates that evaluating a model with the data independent of its operational context is pointless. 
%Therefore, we need to center on 
%the concrete application context rather than excessive attention to the arbitrarily test context with artificially generated inputs.
%\item The \emph{common situation} of the DNN application. 
%The performance of the DNN model depends upon the assumption that the test dataset should have the same distribution with the training dataset. 
%However, this assumption is often violated~\cite{darrell2015machine}, 
%and it occurs universally in visual recognition and computational biology. 
%For instance, an image-classification model can be learned from pictures on the internet, 
%but are often applied to real-world scenes. 
%Therefore, operational DNN testing are urgent needed in ensuring the quality of the model in the application context.
%\item The \emph{fundamental challenge} of the DNN testing. 
%Different from traditional operational testing that has been well studied~\cite{musa1993profiles, 2017bertolinoadaptive}, 
%operational DNN testing is in urgency for further researches. 
%\citeauthor{li2019boosting} proposed that the main challenge of operational DNN testing is that it is too expensive and even impractical to label all the operation data collected in the field. 
%For example, in medical diagnostics, 
%to decide whether a radiology or pathology image is really malignant or benign, 
%a surgical biopsy always is needed.  
%In this situation, each one more labeled sample means that there is a patient who will suffer more pain. 
%Therefore, it is critical to test the model with a limited budget for labeling data collected from this context. 
%Besides, for the sake of profit and safety, 
%the DNN model developer may only provide the DNN model and will not give the original training/test dataset. 
%Above all, the main challenge of the DNN testing is that we often need to evaluate and ensure the performance of the DNN model in an extremely demanding situation: 
%labeled operation data are limited, and the original data are not available.
%\end{itemize}
%

%In this paper, we try to calibrate the DNN confidence in the specific operational context. For details, the divergence between the original dataset and the operation dataset will cause the confidence to be misleading, i.e., there exist many high confidence error-inducing inputs so that we nearly could not determine whether the classification results can be trusted. To solve this problem, we exploit the feature representation capabilities of the DNN model, which are still valid under the operational context, to locate these miscalibrations in representation space.  Then try to calibrate them through building a reliable operational confidence distribution with Bayesian Inference~\cite{tipping2004bayesian}. 

In summary, the contributions of this paper are: 
\begin{itemize}
%\item Posing the problem of operational calibration 
%for DNN models in the field, 
%and casting it into a Bayesian inference framework. 
%
%\item Proposing a Gaussian Process-based approach to operational calibration, 
\item Examining quality assurance for  DNN models used as software components, 
and raising the problem of operational calibration as debugging for confidence errors of DNNs in the field.
\item Proposing a  Gaussian Process-based approach to operational calibration, 
which leverages the representation learned by the DNN model under calibration 
and the locality of confidence errors in this representation. 
\item Evaluating the approach systematically. Experiments with various datasets and models confirmed the general efficacy and efficiency of our approach.
\end{itemize}

The rest of this paper is organized as follows. 
We first discuss the general need for operational quality assurance for DNNs in Section~\ref{sec:operqa}, 
and then define the the problem of operational calibration in Section~\ref{sec:problem}. 
We detail our approach to operational calibration in Section~\ref{sec:method}
and evaluate it empirically in Section~\ref{sec:evaluation}. 
We overview related work and highlight their differences from ours in Section~\ref{sec:relatedwork}
before concluding the paper with Section~\ref{sec:conclusion}.



==> zip/method.tex <==
% !TEX root = main.tex

\section{Solving Operational Calibration with Gaussian Process Regression}
\label{sec:method}

At first glance operational calibration seems a simple regression problem with BS as the loss function. 
However, a direct regression would not work because of the limited budget of labeled operation data. 
%  
It is helpful to view the problem in a Bayesian way. 
At the beginning, we have a prior belief about the correctness of a DNN model's predictions, 
which is the confidence outputs of the model.  
Once we observe some evidences that the model makes correct or incorrect predictions on some inputs, 
the belief should be adjusted accordingly.
The challenge here is to strike a balance between 
the priori that was learned from a huge training dataset but suffering from domain shift, 
and the evidence that is collected from the operation domain but limited in volume. 

%{\color{blue} In this section, we introduce technical details of the Gaussian Process, and then analyze why the Gaussian Process performs well in representation space.  
%Following that, we provide a complete algorithm for the operational calibration of DNN models. 
%Finally, we further discuss the difference between operational calibration and previous confidence calibration methods. 
%One can skip the section~\ref{subsec:modeling with Gaussian Process} if feeling afraid of a large number of mathematical formulas,
%but we strongly recommend interested reader can read the discussion in section~\ref{subsec:discussions}.}

\subsection{Modeling with Gaussian Process}
 \label{subsec:modeling with Gaussian Process}


%for a given input $\bm{x}$, 
%instead of taking $\bm{x}$ which is in original input space, 
%we take advantage of its corresponding vector $\bm{z}$ in representation space. 
%Hence, for inputs $\bm{x}_i, 1 \leq i \leq N$ of operation dataset $T$, 
%we denote their corresponding vector in representation space as $Z_0=(\bm{z}_1^T; \dots; \bm{z}_N^T)$ 
%and their corresponding original confidence can be easily derived from original model $\mathfrak{M}$, we denote them as $\bm{c}_0 = (c_1; \dots; c_n)$.
%Then, after labeling some operational inputs, we denote these labeling data as $\bm{Z}_1 = (\bm{z}_{1'}^T, \dots, \bm{z}_{m'}^T)$, and its corresponding original confidence and labels are $\bm{c}_1 = (c_{1'}, \dots, c_{m'})$ and $\bm{l}_1 = (l_{1'}, \dots, l_{m'})$, respectively. And we compute~\cite{wang14icml} the ratio $\bm{r}_1 = (r_{1'}; \dots; r_{m'})$ of original confidence and operational confidence, where
%\begin{equation}
%r_{i'} = \frac{l_{m'}}{c_{m'}}.
%\end{equation}

%Due to the difficulty in 
%directly transforming the locality of representation space 
%into mathematical probability relation between point and point in representation space, 
%we try to use a Log Gaussian Process (LGP)
%to model original confidence $c$ and confidence ratio $r$. 
%
%Therefore, for a given vector $\bm{z}$ in representation space, the probability distribution of its confidence $c$ follows:
%\begin{equation}
%P(c \mid \bm{z}) \sim \log-\mathcal{N}(\mu_0, \sigma_0), 
%\end{equation}
%where 
%\begin{equation}
%\begin{aligned}
%& \mu_0 = K_{\bm{z} \bm{Z}_0}(K_{\bm{Z}_0 \bm{Z}_0} + \lambda \bm{I})^{-1} \bm{c}_0, \\
%& \sigma_0 = K_{\bm{z} \bm{z}} - K_{\bm{z} \bm{Z}_0}(K_{\bm{Z}_0 \bm{Z}_0} + \lambda \bm{I})^{-1} K_{\bm{Z}_0\bm{z}}.
%\end{aligned}
%\end{equation}
%
%Similarly, the prior probability distribution of the ratio are:
%\begin{equation}
%P(r \mid \bm{z}) \sim \log-\mathcal{N}(0, k),
%\end{equation}
%after observing some labeled operation data, we have
%\begin{equation}
%P(r \mid \bm{z}, \bm{Z}_1, \bm{r}_1) \sim \log-\mathcal{N}(\mu_1, \sigma_1),
%\end{equation}
%where
%\begin{equation}
%\begin{aligned}
%& \mu_1 = K_{\bm{z} \bm{Z}_1}(K_{\bm{Z}_1 \bm{Z}_1} + \lambda \bm{I})^{-1} \bm{r}_1, \\
%& \sigma_1 = K_{\bm{z} \bm{z}} - K_{\bm{z} \bm{Z}_1}(K_{\bm{Z}_1 \bm{Z}_1} + \lambda \bm{I})^{-1} K_{\bm{Z}_1\bm{z}}.
%\end{aligned}
%\end{equation}
%
%Finally, since operational confidence $l = r \cdot c$, we have $l$ also submit to log normal distribution, i.e.,
%\begin{equation}
%P(l \mid \bm{z}) \sim \log- \mathcal{N}(\mu_0 + \mu_1, \sigma_0 + \sigma_1).
%\end{equation} 



%\subsection{Deep Neural Network}
%A deep neural network (DNN) classification is an artificial neural network (ANN) with multiple intermediate (hidden) layers between the input and output layers. 
%The input of the latter layer is obtained by linear and non-linear transformations of the output of the previous layer. 
%We also refer the output layer as softmax layer.
%For a \textit{K}-classification problem, the formulation of softmax function is as follows:
%\begin{equation}\nonumber
%\sigma(\mathbf{z})_{i}=\frac{e^{z_{i}}}{\sum_{j=1}^{K} e^{z_{j}}}, \quad i=1, \ldots, K, \quad \mathbf{z}=\left(z_{1}, \ldots, z_{K}\right) \in \mathbb{R}^{K},
%\end{equation}
%where the vector $\bm{z}$ is output of the logit layer (it is the previous layer of softmax layer. )
%In brief, softmax layer provides a probability distribution consisting of $K$ probabilities.
%
%Figure~\ref{fig:DNN} is a simple example of the neural network. The existence of activation functions $\phi$ makes the model non-linear. 
%
%\begin{figure}[h]
%\begin{center}
%\def\layersep{2cm}
%\begin{tikzpicture}[shorten >=1pt,->,draw=black!50, node distance=\layersep]
%    \tikzstyle{every pin edge}=[<-,shorten <=1pt]
%    \tikzstyle{neuron}=[circle,fill=black!25,minimum size=15pt,inner sep=0pt]
%    \tikzstyle{input neuron}=[neuron, fill=green!50];
%    \tikzstyle{output neuron}=[neuron, fill=red!50];
%    \tikzstyle{hidden neuron}=[neuron, fill=blue!50];
%    \tikzstyle{annot} = [text width=6em, text centered]
%
%    % Draw the input layer nodes
%    \foreach \name / \y in {1,...,2}
%    % This is the same as writing \foreach \name / \y in {1/1,2/2,3/3,4/4}
%        \node[input neuron] (I-\name) at (-1.5* \layersep,-\y) {$x_\y$};
%
%    % Draw the first hidden layer nodes
%    \foreach \name / \y in {1,...,3}
%        \path[yshift=0.5cm]
%            node[hidden neuron] (H1-\name) at (-0.75* \layersep,-\y cm) {$n_{\y}^{(2)}$};
%            
%    % Draw the second hidden layer nodes
%    \foreach \name / \y in {1,...,4}
%        \path[yshift=0.16cm]
%            node[hidden neuron] (H2-\name) at (0*\layersep,- 0.66* \y cm) {$n_{\y}^{(3)}$};
%
%    % Draw the output layer node
%    \foreach \name / \y in {1,...,2}
%    \node[output neuron] (L-\name) at (0.75*\layersep,-\y cm) {$l_\y$};
%
%    \foreach \name / \y in {1,...,2}
%    \node[output neuron] (S-\name) at (1.5*\layersep,-\y cm) {$s_\y$};
%    % Connect every node in the input layer with every node in the
%    % hidden layer.
%    \foreach \source in {1,...,1}
%        \foreach \dest  / \y in {1,...,3}
%            \path (I-\source) edge node[near start] {$w_{1{\y}}$} node[near end]{$b_1$} (H1-\dest);
%            
%    \foreach \source in {2,...,2}
%        \foreach \dest  in {1,...,3}
%            \path (I-\source) edge  (H1-\dest);
%
%    % Connect every node in the hidden layer 
%    \foreach \source in {1,...,3}
%            \foreach \dest in {1,...,4}
%             \path (H1-\source) edge (H2-\dest);
%             
%    % Connect every node in the hidden layer with the output layer
%    \foreach \source in {1,...,4}
%            \foreach \dest in {1,...,2}
%             \path (H2-\source) edge (L-\dest);
%    \foreach \source in {1,...,2}
%            \foreach \dest in {1,...,2}
%             \path (L-\source) edge (S-\dest);
%             
%    % Annotate the layers
%   \node[annot, above of=H2-1, node distance=0.7cm] (hl) {};
%   \node[annot, left of=hl, node distance=1cm] {Hidden Layers};
%    \node[annot, above of=I-1, node distance=1.2cm] {Input};
%    \node[annot, above of=L-1, node distance=1.2cm] {logit};
%    \node[annot, above of=S-1, node distance=1.2cm] {softmax};
%    %\draw[dashed, color=black, line width=0.5pt] (-0.3 * \layersep,-2.8cm) node[below]{$n_i=\phi(\sum_{j}w_{j,i}x_j + b_i)$} ->(-0.5 * \layersep,-2.8cm);
%    \node[below of=H1-3, node distance=0.6cm]{\small{$n_i=\phi(\sum_{j}w_{j,i}x_j + b_i)$}};
%
%\end{tikzpicture}
%\end{center}
%\caption{A simple neural network}
%\label{fig:DNN}
%\end{figure}
%
%Training a DNN model is trying to search the optimal parameters (weights $w_{i,j}$ and biases $b_i$)  
%for minimizing the averaged prediction error over the whole training dataset. 
%Actually, from the perspective of Bayesian, 
%the DNN model learned a posterior probability distribution~\cite{bishop2006prml}, denoted as $p(y \mid \bm{x})$.
%For the given input $\bm{x}$, DNN will give \textit{K} posterior probability functions $p(y = i \mid \bm{x}), i=1,2,\dots,K$ 
%The classification result for this input is 
%the category corresponding to the maximum posterior probability, 
%i.e., $f(\bm{x}) = \arg\max_i p(y = i \mid \bm{x})$, 
%and the confidence is the associate max value $\max_i p(y = i \mid \bm{x})$. 
%In real-world decision-making systems, 
%classification networks should not only be accurate enough in prediction
%but also could offer the precise confidence to indicate when they are likely to be incorrect. 
%For example, a self-driving car, 
%which uses a neural network to detect pedestrians and other obstructions~\cite{bojarski2016selfdriven}, 
%should rely more on other components of self-driven system to control the braking 
%if its detection network cannot confidently predict the presence or absence of immediate obstructions.
%
%In deep learning, 
%DNN testing often aimed to evaluate the generalization of the model. 
%The different evaluation metrics~\cite{seliya2009metrics} (e.g., precision, recall, and 0/1-loss) are set towards different contexts. 
%It always requires that the training data and test data are i.i.d, and in this sense, 
%the test set could adequately characterize the overall performance if test examples are sufficient. 

%In this paper, we assume that if the test set is large enough, the distribution of examples in the test set is consistent with that in the real task.
%However, when the size of test set is small, the inadequacy of test samples will bring unstablility of the accuracy.

%\subsection{The Problem Formulations}
%It can be seen that there exist apparent distinctions between DNN testing and conventional software testing. 
%We think that the fundamental cause is that the DNN is an inductive program and the conventional software is deductive: 
%An individual error-inducing input of the latter always can reveal some logistic error in the program, 
%but for the former, some error-inducing inputs are tolerable in statistics. 
%However, the final goal of 
%DNN testing and conventional software testing are the same, 
%i.e., improving the reliability of software system. 
%
%As has been stressed before, 
%the subject of our research is operational DNN testing. 
%Compared to previous debug DNN testing, 
%operational DNN testing emphasis on inputs 
%that may appear under a specific operational context 
%rather than arbitrary artificially generated inputs (e.g., adversarial inputs). 
%The essential reason is that the 
%distribution of operation data is not compatible with the generated misclassified data. 
%Hence, even finding out such error-inducing inputs, 
%we still can not utilize them to improve the practical performance of the model. 
%In fact, training the model with such adversarial inputs 
%may produce a negative impact 
%on the operational performance of the model~\cite{kurakin2016advtraining}.
%Therefore, we think operational DNN testing are worth deploying
%because testing a previously trained DNN model must depend on its associate application context.
%In other words, operational DNN testing aims to \emph{improve the reliability of software system in the specific operational context.}
%
%On the one hand, the most efficient method for improving the operational DNN reliability is increasing the accuracy of model (i.e., training) in this operational context. 
%However, two factors bring great difficulty in re-training or fine-tuning the model directly. 
%1) Models are often provided by software developers. 
%We can hardly obtain any information 
%about original training process and original data.
%2) The size of labeled operation data is very limited. 
%In this situation, it is reckless to modify the model directly based on operation data.
%Take the ImageCELF dataset
%\footnote{This is a dataset from ImageCLEF 2014 challenge, 
%it contains three similar datasets, 
%\emph{Caltech-256} (\textbf{C}), \emph{ImageNet ILSVRC 2012} (\textbf{I}), and \emph{Pascal VOC 2012} (\textbf{P}). 
%We choose \textbf{C} dataset as original data and \textbf{P} dataset as operation data.}
%~\cite{caputo2014imageclef} as an example. 
%A previously trained model can achieve 86\% accuracy on operational context. 
%When we fine-tuned the model based on the limited operation dataset, 
%the performance of the model did not rise as we expected. 
%The detailed results can are shown in Figure~\ref{fig:training-directly}, 
% the red line is the accuracy without any modification of the model, 
% and the blue line is the accuracy of the fine-tuning model at each training epoch. 
%These two accuracies are both tested on the operation dataset.
%\begin{figure}[htbp]
%\begin{center}
%\includegraphics[width=0.9\columnwidth]{figures/confidence/training-directly}
%\caption{The risk of fine-tuning model directly}
%\label{fig:training-directly}
%\end{center}
%\end{figure}
%
%On the other hand, even if we can fine-tune the model, it is nearly impossible for a DNN model to achieve 100\% accuracy on the given context~\cite{devroye2013probabilistic}. 
%Consequently, one often hopes the DNN can retain the reliable confidence to ensure the system is able to reject possible incorrect inputs. 
%However, the divergence between specific operational context and original context 
%may result in confidence miscalibrations of DNN. 
%For example, we firstly trained a model with the MNIST dataset~\cite{lecun1998gradient}, 
%and then applied it to classified another handwritten digits dataset USPS~\cite{transferlearning.xyz}. 
%We find that 74 inputs are misclassified with high confidence (confidence greater than 0.9) of all 288 misclassified inputs. 
%It means even we set the reject threshold as 0.9, 
%nearly 1/4 incorrect predictions still will be trusted by system.
%The detailed results can be seen in Figure~\ref{fig:conf-risk}.
%
%\begin{figure}[htbp]
%\begin{center}
%\includegraphics[width=0.9\columnwidth]{figures/confidence/conf-risk}
%\caption{The confidence distribution of misclassified inputs}
%\label{fig:conf-risk}
%\end{center}
%\end{figure}
%
%Therefore, we think a significant DNN testing approach should not only searching the misclassifications in the operational context, 
%but also detecting confidence miscalibrations. 
%In this paper, we set the goal of DNN testing as 
%detecting DNNs' confidence miscalibrations in their operational context. 
%In this sense, the problem of efficient DNN testing is: 
%\emph{How to use as few samples for labeling as possible 
%to find more confidence miscalibrations of DNN and to calibrate them.}
%
%
%%It is true that in many cases (e.g., AI-aided clinical medicine~\cite{obermeyer2016predicting}) 
%%the unlabeled data can be easily collected from the operational environment 
%%but labeling them is expensive because it needs high quality annotation (e.g.,labeling sample through expert queries).
%%However, only relying on accuracy estimation could not explain the reliability of DNN model: 
%%A reliable DNN model not only is able to achieve enough accuracy, 
%%but also indicates the correctness of classification results through confidence.


%\subsection{Confidence Calibration}

%\subsection{Bayesian Approach and Gaussian Process}
%Bayesian inference provides a general framework 
%that can derive the posterior probability as a consequence of two antecedents: 
%its corresponding prior probability 
%and the likelihood function for the observed data.  
%The posterior probability is computed by Bayes' theorem:
%\begin{equation}
%P(H \mid E)=\frac{P(E \mid H)}{P(E)} \cdot P(H),
%\end{equation}
%where 
%\begin{itemize}
%\item \emph{Hypothesis} $H$ is any hypothesis in the whole hypothesis space.
%\item \emph{Prior probability} $P(H)$ is the probability of the specific hypothesis. 
%\item \emph{Evidence} $E$ stands for the observed new data.
%\item \emph{Likelihood} $P(E \mid H)$ describes that for the given hypothesis $H$, 
%         the probability of the occurrence of evidence $E$.  
%\item \emph{Marginal likelihood} $P(E)$ is the probability of the occurrence of evidence $E$. 
%\item \emph{Posterior probability} $P(H \mid E)$ is the probability of the hypothesis $H$ given the observed evidence $E$.
%\end{itemize}


%\subsection{Gaussian Process for Regression}

It is natural to model the problem as a Gaussian Process~\cite{rasmussen2005GPML}, 
because what we need is actually a function $\hat{c}(\cdot)$. 
Gaussian Process is a non-parametric kind of Bayesian methods, 
which convert a prior over functions into a posterior over functions according to observed data.

For convenience, instead of estimating $\hat{c}(\cdot)$ directly,  
we consider  
\begin{equation}
h(\bm{x}) = \hat{c}(\bm{x}) - c_\mathfrak{M}(\bm{x}), 
\label{equ:deltaconf}
\end{equation}
where $c_\mathfrak{M}(\bm{x})$ is the original confidence output of $\mathfrak{M}$ for input $\bm{x}$.
At the beginning, without any evidence against $c_\mathfrak{M}(\bm{x})$, 
we assume that the prior distribution of $h(\cdot)$ is a zero-mean normal distribution
\begin{equation}
h \sim \mathcal{N}(\cdot \mid 0, k(\cdot, \cdot)),
\label{equ:normcov}
\end{equation}
where $k(\cdot, \cdot)$ is the covariance (kernel) function, which intuitively describes the ``smoothness'' of $h(\bm{x})$ from point to point. In other words, the covariance function ensures that $h$
produces close outputs when inputs are close in the input space.

Assume that we observe a set  of independent and identically distributed (i.i.d.) labeled operation data $\bm{I} = \{(\bm{x}_i, y_i) \mathop{|} 1\leq i \leq n\}$, in which   $y = h(\bm{x}) = \mathbb{I}(\bm{x}) - c_\mathfrak{M}(\bm{x})$. 
%where $\mathbb{I}(\bm{x})$ is the indicator function for whether the labeled input $\bm{x}$ 
%is misclassified or not.
%be observed data of from some unknown distribution. 
For notational convenience, let 
\begin{equation*}
\begin{aligned}
\bm{X} &= (\bm{x}_1^{\mathsf{T}}; \dots; \bm{x}_n^{\mathsf{T}})  \quad \text{and} \\
\bm{h} &= ({h(\bm{x}_1)}; {\dots}; {h(\bm{x}_n)})
\end{aligned}
\end{equation*}
be the observed data and their corresponding $y$-values, and let 
\begin{equation*}
\begin{aligned}
\bm{X}' &= (({\bm{x}'_{1}})^{\mathsf{T}}; \dots; ({\bm{x}'_{n}})^{\mathsf{T}}), \quad \text{and} \\
\bm{h}' &= ({h(\bm{x}'_{1})}; {\dots}; {h(\bm{x}'_{n})})
\end{aligned}
\end{equation*}
be those for a set $T=\{(\bm{x}'_i, y'_i), i=1,\dots,m\}$ of i.i.d.\ predictive points. 
We have
\begin{equation}
\left(\begin{array}{l}{\bm{h}} \\ {\bm{h'}}\end{array}\right) 
\mid \bm{X}, \bm{X}' \sim \mathcal{N}\left(\bm{0},
\left(
\begin{array}{cc}
{K_{\bm{X}\bm{X}}} & {K_{\bm{X}\bm{X}'}} \\ 
{K_{\bm{X}' \bm{X}}} & {K_{\bm{X}'\bm{X}'}}
\end{array}\right)\right)
\end{equation}
where $\bm{K}$ is the kernel matrix. 
Therefore, the conditional probability distribution is 
\begin{equation}
\bm{y'} \mid \bm{y}, \bm{X}, \bm{X}' \sim \mathcal{N}\left(\bm{\mu}', \bm{\Sigma}'\right)
\end{equation}
where
\begin{equation*}
\begin{aligned}
\bm{\mu}' &=\bm{K}_{\bm{X}' \bm{X}}\left(\bm{K}_{\bm{X} \bm{X}}\right)^{-1} \bm{y}, \\ 
\bm{\Sigma}' &=\bm{K}_{\bm{X}' \bm{X}'}-\bm{K}_{\bm{X}'\bm{X}} \left(\bm{K}_{\bm{X} \bm{X}}\right)^{-1} \bm{K}_{\bm{X} \bm{X}'}.
\end{aligned}
\end{equation*}
%To ensure the matrix invertible, we often add the regularization term:
%\begin{equation}
%\begin{aligned}
%\bm{\mu}' &=\bm{K}_{\bm{X}_{*} \bm{X}}\left(\bm{K}_{\bm{X} \bm{X}}+\sigma^{2} \bm{I}\right)^{-1} \bm{y}, \\ 
%\bm{\Sigma}' &=\bm{K}_{\bm{X}' \bm{X}'}-\bm{K}_{\bm{X}'\bm{X}} \left(\bm{K}_{\bm{X} \bm{X}}+\sigma^{2} \bm{I}\right)^{-1} \bm{K}_{\bm{X} \bm{X}'}.
%\end{aligned}
%\end{equation}


% in this group, 
%we denote the index set of labeled inputs as . 
%The labeled inputs can be written as $\bm{x}_i, $, 
%we can know whether these labeled inputs are misclassified, 
%i.e. the value of indicate function $\mathbb{I}(\bm{x}_i), i \in \mathcal{I}$.
%Therefore, we need to change confidence $c(\bm{x}_i), i \in \mathcal{I}$ 
%to $c'(\bm{x}_i) = \mathbb{I}(\bm{x}_i), i \in \mathcal{I}$.
%In this sense, we have 
%\begin{equation}
%\Delta c(\bm{x}_i) = c'(\bm{x}_i) - c(\bm{x}_i), \quad i \in \mathcal{I}.
%\end{equation}
%

With this Gaussian Process, we can estimate the probability distribution of the operational confidence for any input $\bm{x'}$ as follows
\begin{equation}
h(\bm{x'}) \mid \bm{x'}, \bm{X}, \bm{h} \sim \mathcal{N}(\mu, \sigma),
\end{equation}
where
\begin{equation*}
\begin{aligned}
& \mu = \bm{K}_{\bm{x'} \bm{X}}(\bm{K}_{\bm{X}\bm{X}})^{-1} \bm{h}, \\
& \sigma = \bm{K}_{\bm{x'} \bm{x'}} - \bm{K}_{\bm{x'}\bm{X}}(\bm{K}_{\bm{X} \bm{X}})^{-1} \bm{K}_{\bm{X}\bm{x'}}.
\end{aligned}
\end{equation*}
Then, with Equation~\ref{equ:deltaconf}, we have the distribution of $\hat{c}\left(\bm{x'}\right)$
\begin{equation}
P\left(\hat{c}\left(\bm{x'}\right) \mid \bm{x'}\right) \sim \mathcal{N}\left(c_\mathfrak{M}\left(\bm{x'}\right) + \mu, \sigma \right).
\end{equation} 

Finally, due to the value of confidence ranges from 0 to 1, 
we need to truncate the original normal distribution~\cite{burkardt2014truncated}, i.e.,
\begin{equation}
P\left(\hat{c}\left(\bm{x'}\right) \mid \bm{x'}\right) \sim \mathcal{TN}\left(\mu_{tn}, \sigma_{tn}; \alpha, \beta \right),
\end{equation} 
where
\begin{equation}\label{truncated normal distribution}
\begin{aligned}
& \mu_{tn} = c_\mathfrak{M}\left(\bm{x'}\right) + \mu + \frac{\phi(\alpha) - \phi(\beta)}{\Phi(\alpha) - \Phi(\beta)}\sigma,  \\
& \sigma_{tn}^2 = \sigma^2 \left[1 + \frac{\alpha \phi(\alpha) - \beta \phi(\beta)}{\Phi(\beta) - \Phi(\alpha)} - \left( \frac{\phi(\alpha) - \phi(\beta)}{\Phi(\beta) - \Phi(\alpha)} \right)^2 \right], \\
& \alpha = (0 - c_\mathfrak{M}\left(\bm{x'}\right) - \mu) / \sigma,   
\quad  \beta = (1 - c_\mathfrak{M}\left(\bm{x'}\right) - \mu) / \sigma.
\end{aligned}
\end{equation}
Here the $\phi(\cdot)$ and $\Phi(\cdot)$ are the probability density function and the cumulative distribution function of standard normal distribution, respectively.

With this Bayesian approach, 
we compute a distribution, rather than an exact value, 
for the confidence of each prediction. 
To compute the Brier score, % which only accepts a confidence value as input, 
we simply choose the maximum a posteriori (MAP), i.e., the mode of the distribution,
as the calibrated confidence value.
%In other word, the confidence value is computed by Maximum a Posteriori estimation .
Here it is the mean of the truncated normal distribution 
\begin{equation} 
	\hat{c}(\bm{x}) = \mu_{tn}.
\end{equation}

%Nevertheless, the Bayesian approach has its 
%advantage in providing more information about the 
%uncertainty of the estimated confidence. 
%As will be discussed later, this information is relevant in some cost-sensitive decisions,
%and can help in the selection of operation data to label.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




\subsection{Clustering in representation space}

%\subsection{Effective and Efficient Operational Calibration}

Directly applying the above Gaussian Process to estimate $\hat{c}(\cdot)$ would be 
ineffective and inefficient. 
It is difficult to specify a proper covariance function in Equation~\ref{equ:normcov}, 
because the correlation between the correctness of predictions on different examples 
in the very high-dimensional input space is difficult, if possible, to model.  

Fortunately, we have the DNN model $\mathfrak{M}$ on hand, 
which can be used as a feature extractor, %= f_\mathfrak{M}(\bm{x})  
although it may suffer from the problem of domain shift% and perform badly as a classifier
~\cite{bengio2012unsupervised}.
In this way we transform each input $\bm{x}$ from the input space to 
a corresponding point $\bm{z} $ in the representation space, 
which is defined by the output of the neurons in the last hidden layer. 
It turns out that the correctness of $\mathfrak{M}$'s predictions has 
an obvious locality, i.e., a prediction is more likely to be correct/incorrect 
if it is near to a correct/incorrect prediction in the representation space. 
%
%
%
%
%%There are a few works that attempted to increase the efficiency of operational DNN testing. 
%%\citeauthor{li2019boosting} proposed a test data reduction technique: 
%%Through the distribution approximation of the neurons in the last hidden layer of DNN, 
%%only using half of the test inputs for labeling can achieve a similar level of precision compared with the random sampling in whole test data.
%%However, we think they did not realize 
%%the real insight of their operation data reduction method. 
%Through the transformation of DNN, 
%the inputs are mapped into multiple clusters in representation space of last layer. 
%And the classification result derives from a linear classifier in this representation space. 
%Thus, in the representation space of last layer, 
%the correctness of inputs possesses locality. 
%For details, inputs which have similar outputs in this representation space 
%often are correct or incorrect at the same time.  
%We take datasets MNIST/USPS as a simple example.
%In particular, we previously train a model on MNIST dataset.
%When we applying this model on USPS dataset, 
%which is actually the operation domain,
%although the accuracy significantly drops from 97\% to 68\%, 
%the correctness and incorrectness in representation space still keep relevance.
%To visualize this property, 
%we reduce the representation space to two-dimensional plane, 
%and plot the the location in representation space of incorrect (red points) and correct (blue points) inputs
%See Figure~\ref{fig:locality} for an intuitive example.

%\begin{figure}[htbp]
%\begin{center}
%\includegraphics[width=0.85\columnwidth]{figures/confidence/locality}
%\caption{Locality of prediction correctness in the representation space. 
%\rm{A DNN model trained on the MNIST dataset is applied to an operation 
%domain of the USPS dataset. Despite the significant drop of accuracy from 97\% to 68\%,
%the model is still effective in grouping together examples with correct predictions (blue \textcolor{blue}{$+$}) 
%and those with incorrect ones (red \textcolor{red}{$\times$}). 
%The representation space is reduced to a two-dimensional plane to visualize the effect.}}
%
%\label{fig:locality}
%\end{center}
%\end{figure}

Another insight for improving the efficacy and efficiency of the Gaussian Process is that 
the distribution of operation data in the sparse representation space is far from even. 
They can be nicely grouped into a small number (usually tens) of clusters,
and the correlation of prediction correctness within a group is much stronger than that between groups. 
Consequently, instead of regression with a universal Gaussian Process, 
we carry out a Gaussian Process regression in each cluster.  

This clustering does not only reduce the computational cost of the Gaussian Processes, 
but also make it possible to use different covariance functions for different clusters. 
The flexibility makes our estimation more accurate. 
Elaborately, we use the RBF kernel 
\begin{equation}
k(\bm{z}_1,\bm{z}_2) = \exp\left(-\frac{{\| \bm{z}_1 - \bm{z}_2 \|}^2}{2 \ell^2} \right)
\end{equation} 
where the 
parameter $\ell$ (length scale) can be decided according to the distribution of the original confidence produced 
by $\mathfrak{M}$.   


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Considering costs in decision}
The cost of misclassification must be taken into account in real-world decision making. 
\replaced{We propose to}{One can} also measure how well a model is calibrated with the \emph{loss due to confidence error} (LCE) against a given cost model. 

For example, let us assume a simple cost model in which the gain for a correct prediction is 1 and the loss for a false prediction is $u$. The net gain if we take action on a prediction for input $\bm{x}$ will be
$ \mathbb{I}(\bm{x}) -  u \cdot (1-\mathbb{I}(\bm{x}))$. 
We further assume that there will be no cost to take no action 
when the expected net gain is negative. 
Then the actual gain for an input 
$\bm{x}$ with estimated confidence $\hat{c}(\bm{x})$ will be
\begin{equation}
g(\bm{x}) = 
\left\{
\begin{array}{cc}
{ \mathbb{I}(\bm{x}) -  u \cdot (1-\mathbb{I}(\bm{x}))} & {\text{if}~\hat{c}(\bm{x}) \ge \lambda,} \\
{0} & {\text{if}~\hat{c}(\bm{x}) < \lambda,}  
\end{array}\right.
\label{eqn:actgain}
\end{equation}
where $\lambda= \frac{u}{1+u}$ is the break-even threshold of confidence for taking action.
%
%In the perspective of frequentist, 
%confidence is an exact value 
%which indicates the probability of false prediction.
%In this sense, the break-even threshold of confidence will be $\lambda= \frac{u}{1+u}, \quad 0 < \lambda <1$. 
%We further assume that there is no cost to reject the prediction with confidence lower than $\lambda$.
%In the following we use $\lambda$ to characterize the cost model.  
%
On the other hand, if the confidence was perfect, 
i.e., $\hat{c}(\bm{x})=1$ if the prediction was correct, and 0 otherwise, 
the total gain for dataset $D$ would be 
a constant $G_D=\sum_{i=1}^N\mathbb{I}(\bm{x}_i)$. 
%But the actual gain for an input $\bm{x}$ with estimated confidence $\hat{c}(\bm{x})$ will be
%\begin{equation}
%g(\bm{x}) = 
%\left\{
%\begin{array}{cc}
%{ \mathbb{I}(\bm{x}) -  \frac{\lambda}{(1-\lambda)} \cdot (1-\mathbb{I}(\bm{x}))} & {\text{if}~\hat{c}(\bm{x}) \ge \lambda,} \\
%{0} & {\text{if}~\hat{c}(\bm{x}) < \lambda,}  
%\end{array}\right.
%\end{equation}
So the average LCE over a dataset $D$ with $N$ examples is
%\begin{equation}
$\ell(D) = \frac{1}{N}\left(G_D - \sum_{i=1}^N g(\bm{x}_i)\right)$.
%\end{equation}

%Therefore, the LCE problem is that how to set confidence threshold $\lambda$ and calibrate the confidence $\hat{c}(\cdot)$ to minimize loss due to confidence error $\ell(D)$.

With the Bayesian approach we do not have an exact $\hat{c}(\bm{x})$ 
but a truncated normal distribution of it. 
If we take $\mu_{tn}(\bm{x})$ as $\hat{c}(\bm{x})$,
the above equations still hold.%
%~\footnote{%
%This is because here $u$ is a constant. Things will be different if otherwise. %, for example, 
%%one puts higher stakes on higher confidence predictions. 
%The page limit does not allow us to elaborate on this issue, 
%but the Bayesian approach allows for the flexibility in dealing with different situations.  
%} 

%The expected net gain if we take action will be  
%%For loss due to confidence error, 
%%instead of choosing a single confidence threshold $\lambda$, 
%%the decision criteria for inputs acceptance will depend on the expected profit:
%%
%%In particular, in our simple problem setting 
%%(the gain for a correct prediction is 1 and the loss for a false prediction is $u$).
%%Base on the truncated normal distribution, the expected profit for input $\bm{x}$ is
%\begin{equation}
%\begin{aligned}
%%\mathbb{E}_u \left(\mu_{tn}, \sigma_{tn}\right) 
%g(\bm{x})  &= \int_{c \sim \mathcal{TN}} c \cdot 1 - (1-c) \cdot u \, dc  \\
%&= \mu_{tn}(\bm{x}) \cdot (1+u) - u,
%\end{aligned}
%\end{equation}
%which coincides with the first line of Equation~\ref{eqn:actgain} 
%if taking $\mu_{tn}(\bm{x})$ as $\hat{c}(\bm{x})$. 
%
%We should accept the input that its expected profit is greater than 0, 
%thus the criteria for input acceptance is 
%\begin{equation}
%\hat{c}(\bm{x}) = \mu_{tn}(\bm{x}) \ge \frac{1+u}{u}.
%\end{equation}
%
%It is worth mentioning that 
%although the final acceptance criterion is independent of variance $\sigma_{tn}$, 
%it is because we only consider a relative simple problem setting in this paper. 
%In the case of complex problems, 
%for example, the misclassifications with high confidence will lead to more loss, i.e., $u(\bm{c}) = t \cdot c$, 
%then the decision criteria is 
%\begin{equation}
%\begin{aligned}
%\mathbb{E}_u \left(\mu_{tn}, \sigma_{tn}\right) &= \int_{c \sim \mathcal{TN}} c \cdot 1 - (1-c) \cdot u \, dc  \\
%&= t(\sigma_{tn}^2 + \mu_{tn}^2) - (t-1) \mu_{tn}.
%\end{aligned}
%\end{equation}
%Therefore, the bayesian framework will provide a general method 
%that solve a family of cost-sensitive problem.
%We will further study this series of issues in the future.





Cost-sensitive calibration targets at minimizing the LCE instead of the Brier score. 
% used in the cost-insensitive case. 
%Operational The Brier score and LCE can be seen as cost-insensitive and cost-sensitive cases, respectively.
%Without a cost model, %value of $u$, 
%or we want to minimize LCE for any $u$, 
Notice that calibrating confidence with Brier score generally reduces LCE. 
However, with a cost model, the optimization toward minimizing LCE can be more effective and efficient. 
%For our example, if false prediction is very expensive ($u \gg 1$), 
%we shall spend more budget of labeling data on reducing high confidence misclassifications,
%rather than increasing the confidence of correct predictions. 
%it will be better to build a biased distribution for  $\hat{c}(\bm{x})$ 




\subsection{Selecting operation data to label}
\label{subsec:inputselection}
In case that the set of labeled operation data is given, 
we simply apply a Gaussian Process in each cluster in the representation space 
and get the posteriori distribution for confidence $\hat{c}(\cdot)$.
However, if we can decide which operation data to label, 
we shall spend the budget for labeling more wisely. 

Initially, we select the operational input at the center of each cluster to label, 
and apply a Gaussian Process in each cluster with this central input
to compute the posterior probability distribution of the confidence. 
Then we shall select the most ``helpful'' input to label and repeat the procedure. 
%
The insight for input selection is twofold. 
First, to reduce the uncertainty as much as possible, 
one should choose the input with maximal variance $\sigma_{tn}^2$.
Second, to reduce the LCE as much as possible, 
one should pay more attention to those input with confidence 
near to the break-even threshold $\lambda$. 
So we chose $\bm{x}^*$ as the next input to label:
\begin{equation} \label{equ:selection}
%\bm{x}^* = \arg\min_{\bm{x}} \frac{|\mu_{tn}(\bm{x}) - \frac{u}{u+1}|}{\sigma_{tn}(\bm{x})}.
\bm{x}^* = \arg\min_{\bm{x}} \frac{|\mu_{tn}(\bm{x}) - \lambda|}{\sigma_{tn}(\bm{x})}.
\end{equation}

\added{
With $\bm{x}^*$ and its label $y^*$, we update the corresponding Gaussian Process model and 
get better $\mu_{tn}(\cdot)$ and $\sigma_{tn}(\cdot)$. 
%The select-label-update procedure is repeated until the budget for labeling is used up. 
The select-label-update procedure is repeated until the labeling budget is used up. 
%Thus we should label iteratively such that we can keep the Gaussian Process model (i.e., $\mu_{tn}(\cdot)$ and $\sigma_{tn}(\cdot)$) updated for guiding the new input selection.
%Considering the limited size of labeled operation data and the non-parametric property of Gaussian Process,  the computational complexity of model updating is very low.
}

%Another requirement of operation calibration is 
%\emph{correcting high confidence misclassifications on operation domain with few samples}.
%As discussed earlier, inputs acceptance criteria in our setting are
%\begin{equation}
%\hat{c}(\bm{x}) = \mu_{tn}(\bm{x}) \ge \frac{u}{u+1},
%\end{equation}
%thus correcting high confidence misclassifications 
%is equivalent to minimizing LCE with large $u$.
%




\medskip 

Putting all the ideas together, we have Algorithm~\ref{alg:1} shown below. 
The algorithm is robust in that it does not rely on any hyperparameters 
except for the number of clusters.
It is also conservative in that it does not change the predictions made by 
the model. As a result, it needs no extra validation data.

\begin{algorithm}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\caption{Operational confidence calibration}
\label{alg:1}
\begin{algorithmic}[1]
\REQUIRE A trained DNN model $\mathfrak{M}$,  
unlabeled dataset $S$ collected from operation domain $\mathbb{D}$, 
and the budget $n$ for labeling inputs.
\ENSURE Calibrated confidence function $\hat{c}(\bm{x})$ for $\bm{x}$ belongs to $\mathbb{D}$.
\newline\emph{Build Gaussian Process models:}
\STATE Divide dataset $S$ into $L$ clusters using the K-modroid method, 
and label the inputs $\bm{o}_1,\dots,\bm{o}_L$ 
that correspond to the centers of the $L$ clusters. 
\STATE Initialize the labeled set $T = \{\bm{o}_1,\dots,\bm{o}_L\}$.
\STATE For each of the clusters, build a Gaussian Process model $gp_i$, $i=1,\dots, L$.
\WHILE {$|T| < n$}
    \STATE Select a new input $\tilde{\bm{x}} \in S \setminus T$ for labeling, where $\tilde{\bm{x}}$ is searched by Equation~\ref{equ:selection}.
    \STATE Update the Gaussian Process corresponding to the cluster containing $\tilde{\bm{x}}$.
    \STATE Update the labeled set $T \leftarrow T \cup \{\tilde{\bm{x}}\}$.
\ENDWHILE
\newline\emph{Compute confidence value for input $\bm{x}$:}
\STATE Find the Gaussian Process model $\hat{gp}$ corresponding to the cluster containing input $\bm{x}$.
\STATE Compute $\mu_{tn}(\bm{x})$ according to Equation~\ref{truncated normal distribution}.
\STATE Output the estimated calibrated confidence $\hat{c}(\bm{x}) = \mu_{tn}(\bm{x})$.
\end{algorithmic}
\end{algorithm}

\subsection{Discussions}
\label{subsec:discussions}
To understand why our approach is more effective than conventional confidence calibration techniques,
one can consider the three-part decomposition of the Brier score~\cite{murphy1973BSPartition}
\begin{equation}
\begin{aligned}
BS = &\sum_{m=1}^{M} \frac{|D_{m}|}{N} \left(\text{conf}(D_m) -\text{acc}(D_m) \right)^{2} \\
&-\sum_{m=1}^{M} \frac{1}{N} \left(\text{acc}(D_m) - \text{acc}\right)^{2}+\text{acc}(1-\text{acc}),
\end{aligned}
\end{equation}
where $D_m$ is the set of inputs whose confidence falls into 
the interval $I_{m}=\left(\frac{m-1}{M}, \frac{m}{M}\right]$, 
and the $\text{acc}(D_m)$ and $\text{conf}(D_m)$ 
are the expected accuracy and confidence in $D_m$, respectively.
The $\text{acc}$ is the accuracy of dataset $D$.

In this decomposition, the first term is called \emph{reliability}, 
which measures the distance between the confidence and the true posterior probabilities. 
The second term is \emph{resolution}, which measures the distinctions of the predictive probabilities.
The final term is \emph{uncertainty}, which is only determined by the accuracy.

In conventional confidence calibration,
the model is assumed to be well trained and work well with the accuracies.
In addition, the grouping of $D_m$ is acceptable because the confidence error is regarded as \emph{systematic error.} 
So one only cares about minimizing the reliability. 
This is exactly what conventional calibration techniques such as Temperature Scaling are designed for. 

However, in operational calibration, the model itself suffers from the domain shift, 
and thus may be less accurate than expected. 
Even worse, the grouping of $D_m$ is problematic because the confidence error is \emph{unsystematic} and 
the inputs in $D_m$ are not homogeneous anymore. 
Consequently, we need to maximize the resolution and minimize the reliability at the same time. 
Our approach achieves these two goals with  
 more discriminative calibration that is based on the features of individual inputs rather than their logits or confidence values. 
 


%According to the decomposition, 
%the goal of calibration, minimizing the Brier score, 
%is equivalent to minimizing the reliability and maximizing the the resolution at the same time.
%However, for temperature scaling method, 
%it assumes that the DNN's confidence error is a kind of systematic error.
%In other words, the goal of temperature scaling is to minimize the reliability.
%Thus, when applying the DNN model on operation domain, 
%the shift between origin domain and operation domain will bring some non-systematic error, i.e., the resolution needs to be maximized in further.
%In this situation, compared with our calibration method, 
%the temperature scaling method is not effective enough.

This observation also indicates that the benefit of our approach over Temperature Scaling 
will diminish if the confidence error happens to be systematic. 
For example, in case that the only divergence of the data in the operation domain 
is that some part of an image is missing, our approach will perform similarly to 
or even slightly worse than Temperature Scaling. 
%On the contrary, if the error of confidence is only a systematic decline or increase, 
%for example, 
%in case that , 
%temperature scaling will still be effective 
%and our method is relatively more complex, 
%so its efficacy may not be better than the former.
However, as can be seen from later experiments, most operational situations have more or less 
domain shifts that Temperature Ccaling cannot handle well.

In addition, when the loss for false prediction $u$ is very small ($u \leq 0.11$, as observed from experiments in the next section), our approach will be ineffective in reducing LCE.
It is expected because in this situation one should accept almost all predictions, 
even when their confidence values are low.



==> zip/relatedwork.tex <==
% !TEX root = main.tex
\section{Related work}
\label{sec:relatedwork}
Operational calibration is %proposed as a software quality assurance activityoperation data
%for adopting a previously trained DNN model in an operation domain. 
%It is 
generally related to the \added{quality assurance for} \deleted{testing of} deep learning systems 
in the software engineering community, and the confidence calibration, 
transfer learning, and active learning in the machine learning community.   
We briefly overview related work in these directions 
and highlight the connections and differences between our work and them. 

\subsection{Software \added{quality assurance} \deleted{testing} for deep learning systems}
The research in this area can be roughly classified into four categories according to 
the kind of defects targeted: 
%There are many researches on seeking an effective and efficient technique 
%to assure the DNN quality. 
%Their ideas of DL testing can be divided into three classes.
\begin{itemize}[leftmargin=*]
\item \emph{Defects in DL programs}. This line of work focuses on 
the bugs in the code of DL frameworks. 
For example, \citeauthor{pham2019cradle} proposed to test the implementation 
of deep learning libraries (TensorFlow, CNTK and Theano) through differential testing~\cite{pham2019cradle}.
\citeauthor{odena2019tensorfuzz} used fuzzing techniques to expose 
numerical errors in matrix multiplication operations~\cite{odena2019tensorfuzz}. 
%They implemented the same model on different libraries, and then detected the differences of output on one identical input. 
%The different outputs always show the inconsistencies and bugs among libraries.
%(2) \citeauthor{odena2019tensorfuzz} used fuzzing to capture the numerical errors in matrix multiplication operations of networks. 
%They computed coverage metric by approximate nearest neighbor (ANN) algorithms, 
%and generated coverage-based test inputs to reveal disagreements between neural networks and their quantized versions. 
%\citeauthor{} 
\item \emph{Defects in DL models}. 
Regarding trained DNN models as pieces of software artifact, 
and borrowing the idea of structural coverage in conventional software testing, 
a series of coverage criteria have been proposed for the testing of DNNs, 
for example, 
%
%These bugs indicate the correctness of DNN model. 
%The main challenge of testing the model is how to effectively and efficiently search 
%the input which can reveal the incorrect prediction for given model.
%Therefore, many neuron coverage based testing methods are proposed (e.g. 
DeepXplore~\cite{pei2017deepxplore}, DeepGauge~\cite{ma2018deepgauge}, 
DeepConcolic~\cite{sun2018concolic}, and Surprise Adequacy~\cite{kim2019guiding},
to name but a few. 
%All of them tried to generate adversarial input 
%(which may not belong to normal data distribution~\cite{grosse2018statistical})
%through increasing the coverage. 
%However, the relation of 
%DNN quality assurance and training/testing the model based on adversarial inputs 
%still need further investigation.
%And recent research found that the adversarial inputs are features rather than bugs~\cite{ilyas2019adversarial}.

%In addition, some researchers focus on a particular problem of machine learning: overfitting and underfitting. 
%For example, \citeauthor{} detected underfitting/overfitting by observing the difference between training accuracy and test accuracy. 
%And fixed the underfitting/overfitting through selecting inputs to retrain the model.

\item \emph{Defects in training  datasets}.
Another critical element in machine learning is the dataset. 
There exist research aiming at debugging and fixing errors in the polluted training dataset. 
For example, PSI identifies root causes (e.g., incorrect labels) of data errors 
by efficiently computing the Probability of Sufficiency scores through 
probabilistic programming~\cite{chakarov2016debugging}.
\item \emph{Defects due to improper inputs}. A DNN model cannot well handle inputs 
out of the distribution for which it is trained. 
Thus a defensive approach is to detect such inputs. 
For example, \citeauthor{wang2019adversarial}'s approach checked whether an input is normal or adversarial 
by integrating statistical hypothesis testing and model mutation testing~\cite{wang2019adversarial}. 
\citeauthor{wang2020DISSECTOR} proposed DISSECTOR, which effectively distinguished unexpected inputs from normal inputs by verifying progressive relationship between layers~\cite{wang2020DISSECTOR}.
More work in this line can be found in the machine learning literature 
under the name of out-of-distribution detection~\cite{shalev2018out}.
\end{itemize}
For a more comprehensive survey on the testing of machine learning systems, one can consult 
 \citeauthor{zhang2019surveyMLT}~\cite{zhang2019surveyMLT}.


The main difference of our work, compared with these pieces of research, 
is that it is \emph{operational}, i.e., focusing on how well a DNN model will work 
in a given operation domain. As discussed in Section~\ref{sec:operqa}, 
without considering the operation domain, 
it is often difficult to tell whether a phenomena of a DNN model is a bug or a feature~\cite{ilyas2019adversarial,li2019structural}.

An exception is the recent proposal of \emph{operational testing}  
 for the efficient estimation of the accuracy of a DNN model 
in the field~\cite{li2019boosting}. 
Arguably operational calibration is more challenging and more rewarding than 
operational testing, because the latter only tells the overall performance 
of a model in an operation domain, but the former tells when it works well and when not. 
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{DNN confidence calibration}
Confidence calibration is important for training high quality classifiers. 
There is a plethora of proposals on this topic in the machine learning literature~\cite{niculescu2005predicting,naeini2015obtaining,zadrozny2002transforming, flach2016calibration, guo2017calibration}. Apart from the Temperature Scaling discussed in 
Section~\ref{subsec:dnnconfidence}, 
Isotonic regression~\cite{zadrozny2002transforming}, Histogram binning~\cite{zadrozny2001obtaining}, and Platt scaling~\cite{Platt1999probabilisticoutputs} 
are also often used. 
Isotonic regression is a non-parametric approach that employs the least square method with a non-decreasing and piecewise constant fitted function.
Histogram binning divides confidences into mutually exclusive bins 
and assigns the calibrated confidences by minimizing the bin-wise squared loss.
Platt scaling is a generalized version of Temperature Scaling.
It adds a linear transformation between the logit layer and the softmax layer, 
and optimizes the parameters with the NLL loss.
However, according to \citeauthor{guo2017calibration}, 
Temperature Scaling is often the most effective approach~\cite{guo2017calibration}.  

As discussed earlier in Section~\ref{subsec:discussions},
the problem of these calibration methods is that they regard 
confidence errors as systematic errors, 
which is usually not the case in the operation domain. 
Technically, these calibration methods are effective in 
minimize the reliability part of the Brier score, 
but ineffective in dealing with the problem in the resolution part. 

In addition, \citeauthor{flach2016calibration} discussed the problem of confidence calibration 
from a decision-theoretic perspective~\cite{flach2016calibration}. 
However, the confidence error caused by domain shift was not explicitly addressed. 

% Different from the above methods that calibrate the model without disturbing accuracy, 

%The Bayesian calibration is also considered due to its inherent uncertainty.  
%One such proposal is to use dropout, which was originally introduced as a regularization technique for training deep neural networks. 
%\citeauthor{gal2016dropout} instead proposed to use dropout at prediction time and cast it as approximate Bayesian inference~\cite{gal2016dropout}. 
%Because dropout can be seen as an ensemble method, 
%and the variance of predictive results can guide the confidence calibration. 
%However, though the mathematical results are very elegant, 
%this method still cannot be directly applied to large-scale tasks due to the considerable time consumption.
%
%Besides, conformal prediction, which determines precise levels of confidence in new predictions based on past experience, is also a related topic. 
%Recently, \citeauthor{papernot2018deep} introduce Deep k-Nearest Neighbors~\cite{papernot2018deep}. 
%They build k-Nearest Neighbors (kNN) models respectively for the output of each DNN immediate layer and estimate the confidence by the conformity of these kNNs' predictions.
%Unfortunately, the kNN model depends on the original training dataset and is not suitable for high dimensional situations. 

Previous research efforts on confidence calibration at prediction time instead of training time are uncommon, but do exist. 
\citeauthor{gal2016dropout} proposed to build a temporary ensemble model by using dropout at prediction time~\cite{gal2016dropout}. % and cast it as approximate Bayesian inference. 
% They calibrated the confidence based on the variance of this ensemble predictive results. 
Despite its elegant Bayesian inference framework, the method is computationally too expensive to handle 
%cannot be directly applied to 
large-scale tasks. % due to the considerable time consumption.
Recently, based on the insight of conformal prediction~\cite{shafer2008tutorial}, \citeauthor{papernot2018deep} %introduced Deep k-Nearest Neighbors~\cite{papernot2018deep}. 
%They 
proposed to build a k-Nearest Neighbors (kNN) model for the output of each DNN immediate layer~\cite{papernot2018deep}.   
The confidence of a prediction was estimated by the conformity of these kNNs' outputs.
Unfortunately, this method is  not applicable to non-trivial tasks either because of its incapability in handling high-dimensional examples. 
Note that these methods did not explicitly consider confidence errors caused by domain shifts.

\added{Another related line of work is under the name of uncertainty estimation~\cite{sensoy2018evidential, kuleshov2018accurate, schulam2019can}. 
For example, Evidential Deep Learning qualitatively evaluates the uncertainty of DNN predictions 
with a Dirichlet distribution placed on the class probabilities~\cite{sensoy2018evidential}. 
% Besides, there is quite a few work of uncertainty estimation, which is closely related to confidence calibration~\cite{sensoy2018evidential, kuleshov2018accurate, schulam2019can}. 
%For example, through putting a Dirichlet distribution on the class probabilities, \citeauthor{sensoy2018evidential} proposed Evidential Deep learning method that qualitatively evaluated the uncertainty of DNN predictions~\cite{sensoy2018evidential}. 
However, these methods mainly aim at out-of-distribution detection, which is considered easier than confidence calibration~\cite{flach2016calibration}. 
Identifying out-of-distribution inputs is useful in defending against adversarial attacks, 
but not directly helpful in adapting a model to a new operation domain. 
%In addition, these methods %also lack the scalability to work with large datasets such as ImageNet.
% do not explicitly consider domain shift either.% and may report most of the inputs in a new operation domain as ``out-of-distribution''.
%Apart from the worrying scalability of these methods, they also 
}


%Many experiments were conducted to analyze the reason for confidence errors. 
%Recent research showed that, 
%without the dataset shift,
%the confidence error is mainly caused by over-optimized on the surrogate loss (cross-entropy loss). 
%In other words, when operation data and origin data are i.i.d,
%the confidence error is actually a kind of systematic error.
%To calibration the confidence influenced by this error, 
%some simple regression methods can be very effective.
%In addition to temperature scaling which is discussed in Section~\ref{subsec:dnnconfidence}, 
%Isotonic regression, Histogram binning and Platt scaling~\cite{flach2016calibration, guo2017calibration}, 
%were also proposed to calibrate DNN confidence.
%
%
%However, in many situations, especially for deep learning tasks, 
%the i.i.d assumption may not be hold any more. 
%For example, an image-classification model 
%can be learned from pictures on the internet, 
%but is finally applied to real-world scenes. 
%Due to the existence of dataset shift, 
%confidence error are more than just systematic error 
%and these calibration methods are not effective. 
%Therefore, debug the confidence errors and calibrate DNN confidence 
%should be operational. 
%
%In addition to brier score as a measure of confidence calibration.
%Expected calibration error (ECE), negative log likelihood (NLL), 
%and many other measures are also used for evaluate the efficacy of calibration~\cite{guo2017calibration}.
%In decision theory, the brier score is a proper score function that measures the accuracy of probabilistic predictions. 
%The ECE is actually the first term (reliability) in composition of brier score, 
%The NLL pay more attention to inputs with higher confidence error 
%and Brier score is more uniform.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Transfer learning and active learning}
Our approach to operational calibration borrowed ideas from 
transfer learning~\cite{pan2009survey}
and active learning~\cite{settles2009active}. 
Transfer learning (or domain adaptation) aims at training a model from a source domain (origin domain in our terms)
that can be generalized to a target domain (operation domain), 
despite the dataset shift~\cite{ng2016nuts} between the domains. 
The key is to learn features that are transferable between the domains. 

However, transfer learning techniques usually require 
data from both of the source and target domains. 
Contrastingly, operational calibration often has to work 
with limited data from the operation domain and no data from the origin domain. 
%It does not aim at improving prediction accuracy in the operation domain,  
%but it may leverage the existing transferability of features 
%learned by the DNN model.   
%Both of them leverage the transferability of features learned by the DNN model, but while 
%The former aims at better prediction accuracy, the latter at more accurate confidence.  
%In addition, 
Transfer learning usually fails to work under this constraint. 
Even in case it works, it does not necessarily produce well calibrated models, 
and operational calibration is  needed to correct confidence errors~(cf. Figure~\ref{fig:ft-cali3}). 

Active learning aims at reducing the cost of labeling training data by 
deliberately selecting and labeling inputs from a large set of unlabeled data.  
For the Gaussian Process Regression, 
there exist different input selection strategies~\cite{seo2000gaussian, kapoor2007active, pasolli2011gaussian}.
We tried many of them, such as those based on uncertainty~\cite{seo2000gaussian}, on density~\cite{zhu2009active}, 
and on disagreement~\cite{pasolli2011gaussian}, but failed to find a reliable strategy 
that can further improve the data efficiency of our approach.
They were very sensitive to the choices of the initial inputs, the models, 
and the distribution of examples~\cite{settles2009active}.
However, we found that the combination of cost-sensitive sampling bias and uncertainty 
can help in reducing high-confidence false predictions, especially in a cost-sensitive setting. 




%is a kind of semi-supervised learning 
%whose goal is to get the best possible model performance 
%with as few queries as possible.
%
%the main challenge of employing transfer learning techniques to 
%assure operational DNN quality is the limitations of datasets and models.
%The 
%If this condition can be satisfied, the state-of-art transfer learning techniques 
%obviously can be used to assure operational DNN quality.
%However, in software development, 
%we nearly could not know the exact application context. 
%In other words, it is unavailable to operation data in the training process.  
%Besides, the number of operation data is also limited 
%and the original model may not be completely designed for operation data. 
%Thus the well-known technique, fine-tuning, also may not work in some situations.
%Due to these practical conditions, we think the operational calibration is 
%the most effective and efficient method for operational DNN quality assurance 
%and our experiments also valid this point.




